A Comprehensive Review of Modern Object Segmentation Approaches

Image segmentation is the task of associating pixels in an image with their respective object class labels. It has a wide range of applications in many industries including healthcare, transportation, robotics, fashion, home improvement, and tourism. Many deep learning-based approaches have been developed for image-level object recognition and pixel-level scene understanding-with the latter requiring a much denser annotation of scenes with a large set of objects. Extensions of image segmentation tasks include 3D and video segmentation, where units of voxels, point clouds, and video frames are classified into different objects. We use "Object Segmentation" to refer to the union of these segmentation tasks. In this monograph, we investigate both traditional and modern object segmentation approaches, comparing their strengths, weaknesses, and utilities. We examine in detail the wide range of deep learning-based segmentation techniques developed in recent years, provide a review of the widely used datasets and evaluation metrics, and discuss potential future research directions.

==> CGV-097-Final Files 2/3D_segmentation.tex <==
%\begin{center}
\begin{scriptsize}
\begin{longtable}{|L{1cm}|L{4.2cm}|L{3.8cm}|L{1cm}|} 
\caption{Summary of Popular 3D Segmentation Methods.} \label{tab:threed} \\
\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances (default metric: mIoU (\%))} &                  \textbf{Categorization} \\
                               \hline
\endfirsthead

\caption* {\textbf{Table 5.1 Continued}}\\

\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances} &                  \textbf{Categorization} \\
                               \hline
\endhead

\hline \multicolumn{4}{|r|}{{Cont.}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

                                                               3DCNN-DQN-RNN &                                                                                  Combining CNN, RNN, and Deep Q-Network for 3D object recognition &            Stanford 3D semantic parsing (70.76), SUNCG (33.21) &       Voxel based \\ \hline
            V-Net &                                                        Loss function based on Dice coefficient for tackling background-foreground voxel imbalance &                                         PROMISE2012 (Dice score=82.39) &       Voxel based \\ \hline
           OctNet &                  Hierarchical and nonuniform division of 3D space using unbalanced octrees for efficient allocation of memory to important voxels &                                                RueMonge2014 (81.5) &       Voxel based \\ \hline
              SSC &                                                             Eliminating computations in empty spaces to efficiently process spatially-sparse data &                                              NYU Depth test (68.5) &       Voxel based \\ \hline
           3D-CNN &                                                                                     3D point cloud data segmentation through voxel transformation & Large Lidar point cloud dataset of the urban area of Ottawa (93.0) & Point cloud based \\ \hline
         PointNet &                                                              Raw point clouds segmentation with feature transformation and multi-layer-perceptron &                                                   ShapeNet part (83.7) & Point cloud based \\ \hline
            RSNet &                                                                              Extraction of feature dependencies with slice pooling and RNN layers &                   S3DIS (51.93),  ScanNet (39.35), ShapeNet (84.9) & Point cloud based \\ \hline
              SPG &                                                       Novel 3D point cloud representation capturing contextual relationships between object parts &                                       S3DIS (62.1),  Semantic3D (76.2) & Point cloud based \\ \hline
       RandLA-Net &                                                                                     Random sampling of point clouds and local feature aggregation &                                Semantic3D (77.4), SemanticKITTI (53.9) & Point cloud based \\ \hline
          SCF-Net &                                                                                 Spatial Contextual Feature learning from large-scale point clouds &                                       S3DIS (71.6),  Semantic3D (77.6) & Point cloud based \\ \hline
         BAAF-Net &                                                 Local context augmentation with bilateral block and adaptive fusion of multi-resolutional feature &                 S3DIS (72.2),  Semantic3D (76.2), SemanticKITTI (59.9) & Point cloud based \\ \hline
Point Transformer &                                                                                                     Vector self-attention based transformer layer &                            S3DIS (73.5), ShapeNetPart (ins. mIoU=86.6) & Point cloud based \\ \hline
       Cylinder3D &                                                                             Cylindrical partition of point clouds and asymmetrical 3D convolution &                                 SemanticKITTI (67.8), nuScenes (76.1)  & Point cloud based \\ \hline
          LSD-Net &                                                                                                              Boundary refinement and RGB-D fusion &                                                   NYU-Depth v2 (45.9) &       RGB-D based \\ \hline
          LSTM-CF & Capturing and fusion of contextual information from multiple channels of photometric and depth data with Long Short-Term Memorized Context Fusion &                                         SUN-RGBD (48.1), NYUDv2 (49.7) &       RGB-D based \\ \hline
           DA-RNN &                                                                   Injection of semantic labels into 3D scenes with Data Associated Recurrent Unit &                            Synthetic ShapeNet Scene dataset (85.9) &       RGB-D based \\ \hline
\end{longtable}
\end{scriptsize}
%\end{center}

==> CGV-097-Final Files 2/CGV-097-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-Final Files 2/CGV-097-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-Final Files 2/CGV-097-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-Final Files 2/CGV-097-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-Final Files 2/CGV-097-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-Final Files 2/CGV-097-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-Final Files 2/CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Aaron Hertzmann }{Adobe Research, USA}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Facebook}
\journaleditor{Brian Curless}{University of Washington}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{William T. Freeman}{MIT}
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Stanford}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Luc Van Gool}{KU Leuven and ETH Zurich}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Deep Learning for Multimedia Forensics}\\
Irene Amerini, Aris Anagnostopoulos, Luca Maiano and Lorenzo Ricciardi Celsi\\
ISBN: 978-1-68083-854-1\\
\\
\noindent \textit{Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art}\\
Joel Janai, Fatma Güney, Aseem Behl and Andreas Geiger\\
ISBN: 978-1-68083-688-2\\
\\
\noindent \textit{Discrete Graphical Models - An Optimization Perspective}\\
Bogdan Savchynskyy\\
ISBN: 978-1-68083-638-7\\
\\
\noindent \textit{Line Drawings from 3D Models: A Tutorial}\\
Pierre Bénard and Aaron Hertzmann\\
ISBN: 978-1-68083-590-8\\
\\
\noindent \textit{Publishing and Consuming 3D Content on the Web: A Survey}\\
Marco Potenziani, Marco Callieri, Matteo Dellepiane and Roberto Scopigno\\
ISBN: 978-1-68083-536-6\\
\\
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\


==> CGV-097-Final Files 2/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> CGV-097-Final Files 2/cleaned_dataset_tasks.tex <==
\begin{tabulary}{\linewidth}{LLLLLLL}
\toprule
Dataset Name & Object Detection & Semantic Segmentation & Instance Segmentation & Panoptic Segmentation & 3D segmentation & Video segmentation \\
\midrule
  Cityscapes &                  &             \checkmark &             \checkmark &             \checkmark &                 &          \checkmark \\
    ShapeNet &                  &             \checkmark &                       &                       &       \checkmark &                    \\
       S3DIS &                  &             \checkmark &                       &                       &       \checkmark &                    \\
       NYUv2 &                  &             \checkmark &             \checkmark &                       &                 &                    \\
     ScanNet &                  &             \checkmark &                       &             \checkmark &       \checkmark &                    \\
       DAVIS &                  &                       &                       &                       &                 &          \checkmark \\
      ADE20K &                  &             \checkmark &                       &                       &                 &                    \\
   Sun RGB-D &        \checkmark &             \checkmark &                       &                       &                 &                    \\
  Semantic3D &                  &             \checkmark &                       &                       &                 &                    \\
  PASCAL VOC &        \checkmark &             \checkmark &                       &                       &                 &                    \\
      CamVid &                  &             \checkmark &                       &                       &                 &          \checkmark \\
         LIP &                  &             \checkmark &                       &                       &                 &                    \\
        COCO &        \checkmark &             \checkmark &             \checkmark &             \checkmark &                 &                    \\
       KITTI &        \checkmark &             \checkmark &                       &             \checkmark &                 &                    \\
 YouTube-VOS &                  &                       &                       &                       &                 &          \checkmark \\
    nuScenes &        \checkmark &             \checkmark &             \checkmark &                       &       \checkmark &                    \\
    nuImages &        \checkmark &             \checkmark &             \checkmark &                       &                 &                    \\
        LVIS &        \checkmark &                       &             \checkmark &                       &                 &                    \\
     PartNet &                  &                       &                       &                       &       \checkmark &                    \\
       DRIVE &                  &             \checkmark &                       &                       &                 &                    \\
   PROMISE12 &                  &             \checkmark &                       &                       &                 &                    \\
\bottomrule
\end{tabulary}

==> CGV-097-Final Files 2/dataset_size.tex <==
\begin{scriptsize}
\begin{longtable}{|L{1.5cm}|L{2.7cm}|L{4.5cm}|L{1cm}|} 
\caption{Dataset Scene, Size, and Variety.} \label{tab:datasize} \\

\hline     \textbf{Dataset Name} &                                                                                                        \textbf{\# of object classes} &                                                                                                                        \textbf{Size} &   \textbf{Scene} \\ \hline
\endfirsthead

\caption* {\textbf{Table 7.2 Continued}}\\

\hline     \textbf{Dataset Name} &                                                                                                        \textbf{\# of object classes} &                                                                                                                        \textbf{Size} &   \textbf{Scene} \\ \hline
\endhead

\hline \multicolumn{4}{|r|}{{Cont.}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

  Cityscapes &                                                                                                                         30 &                                                                        5k fine annotated images, 20k coarse annotated images &  street \\ \hline
        ShapeNet &                                                                                                                       3135 &                                                                                            Over 300M models, 220k classified & variety \\ \hline
           S3DIS &                                                                                                                         12 &                                                                                    6 large-scale indoor areas with 271 rooms &  indoor \\ \hline
           NYUv2 &                                                                                                                         26 & 1,449 densely labeled pairs of aligned RGB and depth images, 464 new scenes taken from 3 cities 407,024 new unlabeled frames &  indoor \\ \hline
         ScanNet &                                                                                                                         20 &                                             1,513 annotated scans of labeled voxels with an approximate 90\% surface coverage &  indoor \\ \hline
           DAVIS &                                                                                                                            &                                                        50 video sequences with 3,455 densely annotated frames in pixel level & variety \\ \hline
          ADE20K &                                                                                                                        150 &                             20K scene-centric images exhaustively annotated with pixel-level objects and object parts labels & variety \\ \hline
       Sun RGB-D &                                                                                                                        700 &                      10,335 real RGB-D images of room scenes. Each RGB image has a corresponding depth and segmentation map &  indoor \\ \hline
      Semantic3D &                                                                                                                          8 &                                                                        Over 3 billion points, 15 training and 15 test scenes & outdoor \\ \hline
      PASCAL VOC &                                                                                                                         20 &                                             1,464 images for training, 1,449 images for validation and a private testing set & variety \\ \hline
          CamVid &                                                                                                                         32 &                                                                                                                   701 frames  &  street \\ \hline
             LIP &                                                                                                                         19 &                                                                            50k images with elaborated pixel-wise annotations &  people \\ \hline
            COCO & object detection: 80, keypoints detection: 17, stuff image segmentation: 91, panoptic: 80 thing and 3 stuff categories  &                                                                                                                  328K images & variety \\ \hline
           KITTI &                                                                                                                            &                                                                        180 GB sensor streams with images, OXTS, and Velodyne &  street \\ \hline
     YouTube-VOS &                                                                                                                       7800 & 4,453 videos, 340+ minutes, labeled with dense pixel-level annotations every 5th frame, has instance segmentaion annotations &         \\ \hline
        nuScenes &                                                                                                                         10 &                                                                                                28,130 samples from 1k scenes  &  street \\ \hline
        nuImages &                                                                                                                         10 &                                                                                                         93k annotated images  &  street \\ \hline
            LVIS &                                                                                                                        1k+ &                                                                                                                  164k images & variety \\ \hline
         PartNet &                                                                                                                         24 &                                                                                 573,585 part instances over 26,671 3D models &  indoor \\ \hline
           DRIVE &                                                                                                                            &                                                                                                                    40 images  & medical \\ \hline
Mapillary Vistas &                                                                             66 semantic categories and 37 instance classes &                                                                                                  25k high-resolution images  &  street \\ \hline
           VIPER &                                                                                                                         11 &                                                                                            250K high-resolution video frames & virtual \\ \hline
       PROMISE12 &                                                                                                                            &                                                                                                            50 training cases & medical \\ \hline
            Apolloscape &                                                                                35 semantic classes and 8 instance classes  &                                                                                                         140,000 video frames &  street \\ \hline
            A2D2 &                                                                                                                         38 &                                                                          41,277 annotated frames, 392,556 unannotated frames &  street \\ \hline
             BDD &                                                                                                                         40 &                                                                                                                  100k videos  &  street \\ \hline
             IDD &                                                                                                                         34 &                                                                                                                10,004 images  &  street \\ \hline
        WildDash &                                                                                 28 semantic classes and 9 instance classes &                                                                                                                 1,800 frames &  street \\ \hline
       DensePASS &                                                                                                                         19 &                                                                            100 labelled and 2,000 unlabeled panoramic images &  street \\ \hline
         SYNTHIA &                                                                                                                         13 &                                                                                                                  9,400 frames  & virtual \\ \hline
            GTA5 &                                                                                                                         19 &                                                                                                       24,966 synthetic images  & virtual \\ \hline
         2D-3D-S &                                                                                                                         13 &                                                                                                            70,496 RGB images  &  indoor \\ \hline
\end{longtable}
\end{scriptsize}

==> CGV-097-Final Files 2/dataset_table.tex <==
\begin{tabular}{llllllllllllllllllllllllllll}
\toprule
{} &                                       Dataset Name & Object Detection & Semantic Segmentation & Instance Segmentation & Panoptic Segmentation & 3D segmentation & Video segmentation &                                   Others (Specify) &                                # of object classes &                                               Size &    Scene &                                              Notes &                                        Unnamed: 12 & Unnamed: 13 & Unnamed: 14 & Unnamed: 15 & Unnamed: 16 & Unnamed: 17 & Unnamed: 18 & Unnamed: 19 & Unnamed: 20 & Unnamed: 21 & Unnamed: 22 & Unnamed: 23 & Unnamed: 24 & Unnamed: 25 & Unnamed: 26 \\
\midrule
0  &                                         Cityscapes &                  &            \checkmark &            \checkmark &            \checkmark &                 &         \checkmark &  Image-to-image Translation, Real-Time Semantic... &                                                 30 &  5000 fine annotated images, 20000 coarse annot... &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
1  &                                           ShapeNet &                  &            \checkmark &                       &                       &      \checkmark &                    &                                  3D Reconstruction &                                               3135 &                  over 300M models, 220k classified &  variety &  ShapeNet Parts subset contains 31,693 meshes c... &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
2  &           Stanford 3D Indoor Scene Dataset (S3DIS) &                  &            \checkmark &                       &                       &      \checkmark &                    &                                                    &                                                 12 &          6 large-scale indoor areas with 271 rooms &   indoor &  3D Instance Segmentation and 3D Semantic Segme... &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
3  &                               NYU-Depth V2 (NYUv2) &                  &            \checkmark &            \checkmark &                       &                 &                    &  3D Object Detection, Scene Segmentation, Monoc... &                                                 26 &  1449 densely labeled pairs of aligned RGB and ... &   indoor &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
4  &                                            ScanNet &                  &            \checkmark &                       &            \checkmark &      \checkmark &                    &  Scene Segmentation, 3D Object Detection, Depth... &                                                 20 &  1513 annotated scans of labeled voxels with an... &   indoor &                                       2D & 3D data &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
5  &  Densely Annotation Video Segmentation dataset ... &                  &                       &                       &                       &                 &         \checkmark &  Interactive Segmentation, Video Denoising, Vid... &                                                    &  50 video sequences with 3455 densely annotated... &  variety &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
6  &                                             ADE20K &                  &            \checkmark &                       &                       &                 &                    &  Image-to-Image Translation, Scene Recognition,... &                                                150 &  20K scene-centric images exhaustively annotate... &  variety &  Scene Parsing Benchmark (SceneParse150) is a s... &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
7  &                                          Sun RGB-D &       \checkmark &            \checkmark &                       &                       &                 &                    &  3D Object Detection, Monocular 3D Obeject Dete... &                                                700 &  10335 real RGB-D images of room scenes. Each R... &   indoor &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
8  &                                         Semantic3D &                  &            \checkmark &                       &                       &                 &                    &                                                    &                                                  8 &  over 3 billion points, 15 training and 15 test... &  outdoor &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
9  &  PASCAL Visual Object Classes Challenge (PASCAL... &       \checkmark &            \checkmark &                       &                       &                 &                    &  Weakly-supervised instance segmentation, Weakl... &                                                    &  1,464 images for training, 1,449 images for va... &  variety &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
10 &  Cambridge-driving Labeled Video Database (CamVid) &                  &            \checkmark &                       &                       &                 &         \checkmark &                    Real-Time Semantic Segmentation &                                                 32 &                                         701 frames &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
11 &                             Look into Person (LIP) &                  &            \checkmark &                       &                       &                 &                    &                                                    &  19 semantic human part labels and 2D human pos... &  50,000 images with elaborated pixel-wise annot... &   people &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
12 &         Microsoft Common Objects in Context (COCO) &       \checkmark &            \checkmark &            \checkmark &            \checkmark &                 &                    &  Real-Time Object Detection, Pose Estimation, K... &  object detection: 80, keypoints detection: 17,... &                                        328K images &  variety &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
13 &  Karlsruhe Institute of Technology and Toyota T... &       \checkmark &            \checkmark &                       &            \checkmark &                 &                    &  3D Object Detection, Vehicle Pose Estimation, ... &                                                    &  180 GB sensor streams with images, OXTS, and V... &   street &  Not all sequences are annotated, i.e. only the... &  http://www.cvlibs.net/publications/Geiger2013I... &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
14 &    YouTube-VOS (Youtube Video Object Segmentation) &                  &                       &                       &                       &                 &         \checkmark &  Visual Object Tracking, One-shot visual object... &                                               7800 &  4,453 videos, 340+ minutes, labeled with dense... &          &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
15 &                                           nuScenes &       \checkmark &            \checkmark &            \checkmark &                       &      \checkmark &                    &  3D Object Detection, 3D Multi-Object Tracking,... &                                                 10 &                    28130 samples from 1,000 scenes &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
16 &                                           nuImages &       \checkmark &            \checkmark &            \checkmark &                       &                 &                    &                                                    &                                                 10 &                            93,000 annotated images &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
17 &      Large Vocabulary Instance Segmentation (LVIS) &       \checkmark &                       &            \checkmark &                       &                 &                    &                                                    &                                                1k+ &                                        164k images &  variety &                    Has a long tail of rare objects &               https://arxiv.org/pdf/1908.03195.pdf &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
18 &                                            PartNet &                  &                       &                       &                       &      \checkmark &                    &                                                    &                                                 24 &       573,585 part instances over 26,671 3D models &          &  annotated with fine-grained, instance-level, a... &                   https://partnet.cs.stanford.edu/ &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
19 &  Digital Retinal Images for Vessel Extraction (... &                  &            \checkmark &                       &                       &                 &                    &                         Medical Image Segmentation &                                                    &                                          40 images &  medical &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
20 &                                          PROMISE12 &                  &            \checkmark &                       &                       &                 &                    &                         Medical Image Segmentation &                                                    &                                  50 training cases &  medical &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
\bottomrule
\end{tabular}


==> CGV-097-Final Files 2/dataset_task.tex <==
\begin{scriptsize}
\begin{longtable}{|L{1.6cm}|L{0.23cm}|L{0.23cm}|L{0.23cm}|L{0.23cm}|L{0.23cm}|L{0.23cm}|L{5.1cm}|} 
\caption{Summary of Dataset and Associated Tasks} \label{tab:datatask} \\

\hline Dataset Name & \rot{Object Detection} &  \rot{Semantic Segmentation} &  \rot{Instance Segmentation} &  \rot{Panoptic Segmentation} &  \rot{3D segmentation} &  \rot{Video segmentation} & Others \\ \hline
\endfirsthead

\caption* {\textbf{Table 7.1 Continued}}\\

\hline Dataset Name & \rot{Object Detection} &  \rot{Semantic Segmentation} &  \rot{Instance Segmentation} &  \rot{Panoptic Segmentation} &  \rot{3D segmentation} &  \rot{Video segmentation} & Others \\ \hline
\endhead

\hline \multicolumn{8}{|r|}{{Cont.}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

Cityscapes     &                  &  \checkmark &            \checkmark &            \checkmark &                 &         \checkmark &                                     Image-to-image Translation, Real-Time Semantic Segmentation \\ \hline

ShapeNet       &                  &            \checkmark &                       &                       &      \checkmark &                    &                                                                               3D Reconstruction \\ \hline

S3DIS             & &            \checkmark &                       &                       &      \checkmark &                    &                                                                                                 \\ \hline

 NYUv2           &       \checkmark &            \checkmark &            \checkmark &                       &                 &                    &                       Monocular Depth Estimation, Depth Completion, Surface Normals Estimation \\ \hline

ScanNet          &       \checkmark &            \checkmark &                       &            \checkmark &      \checkmark &                    &              Depth Estimation, Scene Recognition, 3D Reconsturction, Surface Normals Estimation \\ \hline

DAVIS 	  &       \checkmark &                       &                       &                       &                 &         \checkmark &                               Interactive Segmentation, Video Denoising, Video Object Detection \\ \hline

ADE20K           &                  &            \checkmark &                       &                       &                 &                    &                                                 Image-to-Image Translation, Scene Understanding \\ \hline

Sun RGB-D       &       \checkmark &            \checkmark &                       &                       &                 &                    &                                                                          Room Layout Estimation \\ \hline

Semantic3D      &                 &            \checkmark &                       &                       &                 &                    &                                                                                                 \\ \hline

PASCAL VOC    & \checkmark &            \checkmark &            \checkmark &            \checkmark &                 &                    &                                                                                  Graph Matching \\ \hline

CamVid             &                 &            \checkmark &                       &                       &                 &         \checkmark &                                                                                                 \\ \hline

LIP 		    &               &            \checkmark &                       &                       &                 &                    &                                                                                                 \\ \hline

COCO		    &       \checkmark &            \checkmark &            \checkmark &            \checkmark &                 &                    &        Pose Estimation, Keypoint Detection, Text-to-Image Generation, Visual Question Answering \\ \hline

KITTI 		    &       \checkmark &            \checkmark &                       &            \checkmark &                 &                    & Vehicle Pose Estimation, Monocular Depth Estimation, Multiple Object Tracking, Depth Completion \\ \hline

YouTube-VOS    &                  &                       &                       &                       &                 &         \checkmark &                                                        Visual Object Tracking, Video Inpainting \\ \hline

nuScenes           &       \checkmark &            \checkmark &            \checkmark &                       &      \checkmark &                    &                                                3D Multi-Object Tracking,  Trajectory Prediction \\ \hline

nuImages          &       \checkmark &            \checkmark &            \checkmark &                      &                 &                    &                                                                                                 \\ \hline

LVIS                   &       \checkmark &                       &            \checkmark &                       &                 &                    &                                                                                                 \\ \hline

PartNet             &                &                       &                       &                       &      \checkmark &                    &                                                                                                 \\ \hline

DRIVE               &                  &            \checkmark &                       &                       &                 &                    &                                                                                                 \\ \hline

Mapillary Vistas &       \checkmark &            \checkmark &            \checkmark &            \checkmark &                 &                    &                                                                                                 \\ \hline

VIPER                &       \checkmark &            \checkmark &            \checkmark &            \checkmark &      \checkmark &         \checkmark &  Optical Flow, Visual Odometry \\ \hline

PROMISE12      &                  &            \checkmark &                       &                       &                 &                    &                                                                                                 \\ \hline

Apolloscape      &                  &            \checkmark &            \checkmark &                       &                 &                    &                                                        Self-Localization, Lanemark Segmentation \\ \hline

A2D2                &       \checkmark &            \checkmark &            \checkmark &                      &      \checkmark &                    &                                                                                                 \\ \hline

BDD                  &       \checkmark &            \checkmark &            \checkmark &                       &                 &         \checkmark &                                        Multi-Object Tracking, Lane Detection, Domain Adaptation \\ \hline

IDD                  &       \checkmark &            \checkmark &                        &                       &                 &                    &                                                                                                 \\ \hline

WildDash         &                 &            \checkmark &            \checkmark &            \checkmark &                 &                    &                                                                                                 \\ \hline

DensePASS     &                  &            \checkmark &                       &                       &                 &                    &                                                       Panoramic Segmentation, Domain Adaptation \\ \hline

SYNTHIA         &                  &            \checkmark &                       &                       &                 &                    &                                                   Domain Adaptation, Image-to-Image Translation \\ \hline

GTA5               &                  &            \checkmark &                       &                       &                 &                    &                                                   Domain Adaptation, Image-to-Image Translation \\ \hline

2D-3D-S          &       \checkmark &            \checkmark &                       &                       &      \checkmark &                    &                              Depth Estimation, Surface Normals Estimation, Scene Reconstruction \\ \hline
\end{longtable}
\end{scriptsize}

==> CGV-097-Final Files 2/instance_segmentation.tex <==
\begin{center}
\begin{scriptsize}
\begin{longtable}{|L{1.2cm}|L{3.9cm}|L{3.6cm}|L{1.3cm}|} 
\caption{Summary of Popular Instance Segmentation Methods.} \label{tab:instance} \\

\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances} &                  \textbf{Categorization} \\
                               \hline
\endfirsthead

\caption* {\textbf{Table 4.1 Continued}}\\

\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances} &                  \textbf{Categorization} \\
                               \hline
\endhead

\hline \multicolumn{4}{|r|}{{Cont.}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

                                                               SDS &                                                                                                        Multiscale Combinatorial Grouping (MCN) algorithm for region proposals &                                                                          PASCAL VOC (Mask AP=52.6) &      Two-stage \\ \hline
                      DeepMask &                                                                                                                                    Region proposals and object classification &                                            MS COCO (AR= 36.6), PASCAL VOC 2007 (AR = 43.3) &      Two-stage \\ \hline
                     SharpMask &                                                                                 Augmenting feedforward nets for object segmentation with a novel top-down refinement approach &                                                                         MS COCO (AR= 39.3) &      Two-stage \\ \hline
                  MultiPathNet & Capturing multi-scale contexts with foveal structure; skip connections for recovering spatial information; novel loss function integrating metrics at multiple IOU thresholds &                                                                     MS COCO (Mask AP=25.0) &      Two-stage \\ \hline
                    Mask R-CNN &                                       Extends Faster R-CNN by adding a branch for predicting an object mask in parallel with the existing branch for bounding box recognition & Cityscapes (Mask AP=36.4), MS COCO (ResNeXt-101: Mask AP=37.1, SpineNet-190: Mask AP=46.1) &      Two-stage \\ \hline
            Mask Scoring R-CNN &                                                                                          MaskIoU head trained with simple regression for improving segmentation mask quality &                                                                     MS COCO (Mask AP=39.6) &      Two-stage \\ \hline
                         PANet &                                                                                                 Bottom-up path, adaptive feature pooling, and fully-connected layers that improve information propagation in Mask-R-CNN &                                          MS COCO (Mask AP=42.0), Cityscapes (Mask AP=41.4) &      Two-stage \\ \hline
                          MNCs &                                                                        Three-stage network consisting of instance differentiation, mask estimation, and object categorization &                                 PASCAL VOC (Mask AP=63.5), MS COCO (Mask AP=24.6) &      Two-stage \\ \hline
                   MaskX R-CNN &                                                     Weight transfer function that maps a category’s bounding box detection parameters to its instance segmentation parameters &                                                                     MS COCO (Mask AP=29.5) &      Two-stage \\ \hline
                       MaskLab &                                                                                   Three branches consisting of box detection, semantic segmentation, and direction prediction &                                                                     MS COCO (Mask AP=43.0) &      Two-stage \\ \hline
                           OMN &                                                                                               Inference of object segment representation based on distance to object boundary &                             PASCAL VOC (MASK AP=65.69), Cityscapes (Mask AP=17.4) &      Two-stage \\ \hline
            Cascade Mask R-CNN &                                                                         Progressively improves boudning box quality with sequential detectors with increasing IoU thresholds &                                                         MS COCO (2017 val)  (Mask AP=42.3) &      Two-stage \\ \hline
                          FCOS &                                                                                          Center-ness loss measuring how “centered” is the pixel location in its bounding box  &                                                                     MS COCO (Mask AP=44.7) &      One-stage \\ \hline
                    ExtremeNet &                                                                                                                 Extreme points used to approximate an instance segmentation mask &                                                                     MS COCO (Mask AP=34.6) &      One-stage \\ \hline
                      ESE-Seg  &                                                         Using inner center radius shape signature to parameterize the contour and Chebyshev polynomials  to fit the signatures &                                                                     MS COCO (Mask AP=21.6) &      One-stage \\ \hline
                     PolarMask &                                                                                                      Formulating segmentation as  a regression problem and the Polar IoU Loss &                                                                     MS COCO (Mask AP=32.9) &      One-stage \\ \hline
                    FourierNet &                                                                                                 Obtaining contour points with Inverse Fast Fourier Transform (IFFT) algorithm &                                                                     MS COCO (Mask AP=30.6) &      One-stage \\ \hline
                        MEInst &                                                                                  Mask representation with compact fixed-dimension vector through dictionary learning methods  &                                                                     MS COCO (Mask AP=38.2) &      One-stage \\ \hline
                    TensorMask &                                                    Representation of image content (e.g., masks) with structured high-dimensional tensors in a set of densely sliding windows &                                                                     MS COCO (Mask AP=37.3) &      One-stage \\ \hline
                        YOLACT &                                                                                                 Real-time instance segmentation through linear combination of prototype masks &                                                                     MS COCO (Mask AP=31.2) &      One-stage \\ \hline
                        YOLACT++ &                                                                   Adds a fast mask re-scoring branch and deformable convolutions to YOLACT, and optimizes the prediction head &                                                                     MS COCO (Mask AP=34.1) &      One-stage \\ \hline
                       SipMask &                                       Accurate delineation of spatially adjacent instances and improved mask predictions with a lightweight spatial preservation (SP) module  &                                                                     MS COCO (Mask AP=32.8) &      One-stage \\ \hline
                    SparseInst &                                                                                                                          Object representation with instance activation maps  &                                                                     MS COCO (Mask AP=37.9) &      One-stage \\ \hline
                     BlendMask &                                                                              Blender module incorporating rich instance-level information with accurate dense pixel features &                                                                     MS COCO (Mask AP=41.3) &      One-stage \\ \hline
                    CenterMask &                 Predicting segmentation mask inside detected box with Spatial Attention-Guided Mask (SAG-Mask)  by focusing on the informative pixels while suppressing noise &                                                                     MS COCO (Mask AP=41.8) &      One-stage \\ \hline
                      CondInst &                                                                                                   Dynamically generated convolutional filters conditioned on target instances &                                                                     MS COCO (Mask AP=40.1) &      One-stage \\ \hline
                          SOLO &                                                                                                 Transforms instance segmentation into two pixel-level classification problems &                                                                     MS COCO (Mask AP=37.8) &      One-stage \\ \hline
                        SOLOv2 &                                                                                       Decomposing mask learning to feature learning and dynamic convolution kernel generation &                                                                     MS COCO (Mask AP=41.7) &      One-stage \\ \hline
                          SOTR &                                                 Twin attention mechanism with sparse representation; dynamic convolution kernel generation and segmentation with Transformers &                                                                     MS COCO (Mask AP=42.1) &      One-stage \\ \hline
                          DETR &                                                                                                   Set-based global loss that forces unique predictions via bipartite matching &                                                              MS COCO (Panoptic Quality=46) &    Query-based \\ \hline
                     QueryInst &                                                                                                                                    Parallel supervision on dynamic mask heads &              MS COCO (Mask AP=42.8), Cityscapes (Mask AP=34.4), YouTube-VIS (Mask AP=36.2) &    Query-based \\ \hline
          Deep Metric Learning &                                                                                                                         Clustering pixel embeddings for instance segmentation &                                                        PASCAL VOC (Mask AP=62.21) &        Other \\ \hline
      Deep Watershed Transform &                                                                                                                       Extraction of object instance segments with energy map &                                                                  Cityscapes (Mask AP=19.4) &          Other \\ \hline
Soft Teacher and Box Jittering &                                                                                                          Semi-supervised training with both labeled and pseudo-labeled images &                                                                     MS COCO (Mask AP=53.0) &          Other \\ \hline
\end{longtable}
\end{scriptsize}
\end{center}

==> CGV-097-Final Files 2/journaldata/ACC-editorialboard.tex <==
%ACC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

%\journalchiefeditor{Stefan J. Reichelstein}{Stanford University\\United States}



\subsection{Executive Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Jonathan Glover, Editor-in-Chief}{Columbia University}
\journaleditor{Stephen Penman}{Columbia University}
\journaleditor{Stefan J. Reichelstein}{Stanford University and University of Mannheim}
\journaleditor{Dan Taylor}{University of Pennsylvania}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ACC-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{ACCcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {ACCcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Accounting}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACC}
\journalurl        {http://www.nowpublishers.com/ACC}
\journalissnprint  {1554-0642}
\journalissnonline {1554-0650}
\journaldoi        {10.1561/14}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Auditing}
\item{Corporate Governance}
\item{Cost Management}
\item{Disclosure}
\item{Event Studies/Market Efficiency Studies}
\item{Executive Compensation}
\item{Financial Reporting}
\item{Management Control}
\item{Performance Measurement}
\item{Taxation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ACC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{IFRS: Markets, Practice, and Politics}\\
Kirstin Becker, Jannis Bischof and Holger Daske\\
ISBN: 978-1-68083-830-5
\\
\\
\noindent \textit{Using Python for Text Analysis in Accounting Research}\\
Vic Anand, Khrystyna Bochkay, Roman Chychyla and Andrew Leone\\
ISBN: 978-1-68083-760-5
\\
\\
\noindent \textit{Research on Corporate Sustainability: Review and Directions for Future Research}\\
Jody Grewal and George Serafeim\\
ISBN: 978-1-68083-718-6
\\
\\
\noindent \textit{Field Experiments in Managerial Accounting Research}\\
Sofia M. Lourenco\\
ISBN: 978-1-68083-628-8

==> CGV-097-Final Files 2/journaldata/ACG-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Marc Goergen}{IE Business School\\Spain}
\journalchiefeditor{Geoffrey Wood}{Western University\\Canada}

\subsection{Founding Editor}

\editor{Douglas Cumming}{Florida Atlantic University, USA}

\subsection{Associate Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Renee Adams}{University of Oxford}
\journaleditor{Lucian Bebchuk}{Harvard University}
\journaleditor{William Judge}{Old Dominion University}
\journaleditor{Mark Roe}{Harvard University}
\journaleditor{Rene Stulz}{Ohio State University}
\journaleditor{James Westphal}{University of Michigan}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ACG-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ACGcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ACGcolor} %a color name. 
\journaltitle      {Annals of Corporate Governance}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACG}
\journalurl        {http://www.nowpublishers.com/ACG}
\journalissnprint  {2381-6724}
\journalissnonline {2381-6732}
\journaldoi        {10.1561/109	}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
Annals of Corporate Governancepublishes
 articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Boards of Directors}
\item{Ownership}
\item{National Corporate Governance Mechanisms}
\item{Comparative Corporate Governance Systems}
\item{Self Governance}
\item{Teaching Corporate Governance}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
 Annals of Corporate Governance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ACG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Social Purpose of the Modern Business Corporation}\\
Peter J. Buckley
\\ISBN: 978-1-68083-874-9
\\
\noindent \textit{Decentralized Autonomous Organizations: Internal Governance and External Legal Design}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-798-8
\\
\noindent \textit{Decentralized Corporate Governance via Blockchain Technology}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-676-9
\\
\noindent \textit{Corporate Governance in IPO Firms}\\
Erik E. Lehmann and Silvio Vismara
\\ISBN: 978-1-68083-634-9
\\
\noindent \textit{The Political and Governance Risks of Sovereign Wealth}\\
Paul Rose 
\\ISBN: 978-1-68083-624-0



==> CGV-097-Final Files 2/journaldata/ASTP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ASTP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ASTP-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Case Studies of Successful Technology Transfer from Federal Laboratories}\\
Gretchen B. Jordan, Christopher S. Hayter, Michael Hogan, Manuel A. Gonzalez and Alan C. O’Connor\\
ISBN: 978-1-68083-808-4\\

\noindent \textit{Toward More Effective Science and Technology Advice for Congress: The Historical Roots and Pathways Forward}\\
Peter D. Blair\\
ISBN: 978-1-68083-802-2\\

\noindent \textit{The Globalization of the Bayh–Dole Act}\\
Thorsten Gores and Albert N. Link\\
ISBN: 978-1-68083-754-4\\

\noindent \textit{Globalization and the High-Tech Policy Response}\\
Gregory Tassey\\
ISBN: 978-1-68083-690-5\\
\\
\noindent \textit{Evolution of Ireland’s Industrial, Science and Technology Policy}\\
James A. Cunningham, Patrick Collins and Majella Giblin\\
ISBN: 978-1-68083-680-6\\
\\
\noindent \textit{Public Support of Private Innovation: An Initial Assessment of the North Carolina SBIR/STTR Phase I Matching Funds Program}\\
John W. Hardin, David J. Kaiser and Albert N. Link\\
ISBN: 978-1-68083-674-5

==> CGV-097-Final Files 2/journaldata/CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Aaron Hertzmann }{Adobe Research, USA}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Facebook}
\journaleditor{Brian Curless}{University of Washington}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{William T. Freeman}{MIT}
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Stanford}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Luc Van Gool}{KU Leuven and ETH Zurich}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Deep Learning for Multimedia Forensics}\\
Irene Amerini, Aris Anagnostopoulos, Luca Maiano and Lorenzo Ricciardi Celsi\\
ISBN: 978-1-68083-854-1\\
\\
\noindent \textit{Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art}\\
Joel Janai, Fatma Güney, Aseem Behl and Andreas Geiger\\
ISBN: 978-1-68083-688-2\\
\\
\noindent \textit{Discrete Graphical Models - An Optimization Perspective}\\
Bogdan Savchynskyy\\
ISBN: 978-1-68083-638-7\\
\\
\noindent \textit{Line Drawings from 3D Models: A Tutorial}\\
Pierre Bénard and Aaron Hertzmann\\
ISBN: 978-1-68083-590-8\\
\\
\noindent \textit{Publishing and Consuming 3D Content on the Web: A Survey}\\
Marco Potenziani, Marco Callieri, Matteo Dellepiane and Roberto Scopigno\\
ISBN: 978-1-68083-536-6\\
\\
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\


==> CGV-097-Final Files 2/journaldata/CIT-editorialboard.tex <==
\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{Alexander Barg}{University of Maryland\\USA}

\subsection{Area Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Emmanuel Abbe}{Princeton University}
\journaleditor{Arya Mazumdar}{UMass Amherst}
\journaleditor{Olgica Milenkovic}{University of Illinois, Urbana-Champaign}
\journaleditor{Anelia Somekh-Baruch}{Bar-Ilan University}
\journaleditor{Himanshu Tyagi}{Indian Institute of Science}

\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Venkat Anantharam}{UC Berkeley}
\journaleditor{Giuseppe Caire}{TU Berlin}
\journaleditor{Daniel Costello}{University of Notre Dame}
%\journaleditor{Anthony Ephremides}{University of Maryland}
%\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Albert Guillen i Fabregas}{Pompeu Fabra University}
\journaleditor{Dongning Guo}{Northwestern University}
\journaleditor{Dave Forney}{MIT}
\journaleditor{Te Sun Han}{University of Tokyo}
\journaleditor{Babak Hassibi}{Caltech}
\journaleditor{Michael Honig}{Northwestern University}
%\journaleditor{Tara Javidi}{UC San Diego}

\journaleditor{Ioannis Kontoyiannis}{Cambridge University}
\journaleditor{Gerhard Kramer}{TU Munich}
\journaleditor{Amos Lapidoth}{ETH Zurich}
\journaleditor{Muriel Medard}{MIT}
\journaleditor{Neri Merhav}{Technion}
\journaleditor{David Neuhoff}{University of Michigan}
\journaleditor{Alon Orlitsky}{UC San Diego}
\journaleditor{Yury Polyanskiy}{MIT}
\journaleditor{Vincent Poor}{Princeton University}
%\journaleditor{Maxim Raginsky}{UIUC}
\journaleditor{Kannan Ramchandran}{UC Berkeley}
\journaleditor{Igal Sason}{Technion}
%\columnbreak
\journaleditor{Shlomo Shamai}{Technion}
\journaleditor{Amin Shokrollahi}{EPF Lausanne}
\journaleditor{Yossef Steinberg}{Technion}
\journaleditor{Wojciech Szpankowski}{Purdue University}
\journaleditor{David Tse}{Stanford University}
\journaleditor{Antonia Tulino}{Bell Labs}
\journaleditor{R\"{u}diger Urbanke}{EPF Lausanne}
\journaleditor{Emanuele Viterbo}{Monash University}
\journaleditor{Frans Willems}{TU Eindhoven}
\journaleditor{Raymond Yeung}{CUHK}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/CIT-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{CITcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {CITcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Communications and Information Theory}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CIT}
\journalurl        {http://www.nowpublishers.com/CIT}
\journalissnprint  {1567-2190}
\journalissnonline {1567-2328 }
\journaldoi        {10.1561/01}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Communications and Information Theory publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Coded modulation}
\item{Coding theory and practice}
\item{Communication complexity}
\item{Communication system design}
\item{Cryptology and data security}
\item{Data compression}
\item{Data networks}
\item{Demodulation and Equalization}
\item{Denoising}
\item{Detection and estimation}
\item{Information theory and statistics}
\item{Information theory and computer science}
\item{Joint source/channel coding}
\item{Modulation and signal design}
\item{Multiuser detection}
\item{Multiuser information theory}
\item{Optical communication channels}
\item{Pattern recognition and learning}
\item{Quantization}
\item{Quantum information processing}
\item{Rate-distortion theory}
\item{Shannon theory}
\item{Signal processing for communications}
\item{Source coding}
\item{Storage and recording codes}
\item{Speech and Image Compression}
\item{Wireless Communications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Communications and Information Theory, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/CIT-seriespage.tex <==
\vspace{12pt}
\\
\noindent \textit{An Algebraic and Probabilistic Framework for Network Information Theory}\\
S. Sandeep Pradhan, Arun Padakandla and Farhad Shirani\\
ISBN: 978-1-68083-766-7\\
\\
\noindent \textit{Theoretical Foundations of Adversarial Binary Detection}\\
Mauro Barni and Benedetta Tondi\\
ISBN: 978-1-68083-764-3\\
\\
\noindent \textit{Polynomial Methods in Statistical Inference}\\
Yihong Wu and Pengkun Yang\\
ISBN: 978-1-68083-730-8\\
\\
\noindent \textit{Information-Theoretic Foundations of Mismatched Decoding}\\
Jonathan Scarlett, Albert Guillen i Fabregas, Anelia Somekh-Baruch and Alfonso Martinez\\
ISBN: 978-1-68083-712-4\\
\\
\noindent \textit{Coded Computing: Mitigating Fundamental Bottlenecks in Large-Scale Distributed Computing and Machine Learning}\\
Songze Li and Salman Avestimehr \\
ISBN: 978-1-68083-704-9



==> CGV-097-Final Files 2/journaldata/DBS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Joseph M. Hellerstein}{University of California at Berkeley\\United States}
\journalchiefeditor{Surajit Chaudhuri}{Microsoft Research, Redmond\\United States}



\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Azza Abouzied}{NYU-Abu Dhabi}
\journaleditor{Gustavo Alonso}{ETH Zurich}
\journaleditor{Mike Cafarella}{University of Michigan}
\journaleditor{Alan Fekete}{University of Sydney}
\journaleditor{Ihab Ilyas}{University of Waterloo}
\journaleditor{Andy Pavlo}{Carnegie Mellon University}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/DBS-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{DBScolor}{officegreen}   %new color names can be defined before use
\journalcolor      {DBScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Databases}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {DBS}
\journalurl        {http://www.nowpublishers.com/DBS}
\journalissnprint  {1931-7883}
\journalissnonline {1931-7891}
\journaldoi        {10.1561/19}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Databases publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Data Models and Query Languages}
    \item{Query Processing and Optimization}
    \item{Storage, Access Methods, and Indexing}
    \item{Transaction Management, Concurrency Control and Recovery}
    \item{Deductive Databases}
    \item{Parallel and Distributed Database Systems}
    \item{Database Design and Tuning}
    \item{Metadata Management}
    \item{Object Management}
    \item{Trigger Processing and Active Databases}
    \item{Data Mining and OLAP}
    \item{Approximate and Interactive Query Processing}
    \item{Data Warehousing}
    \item{Adaptive Query Processing}
    \item{Data Stream Management}
    \item{Search and Query Integration}
    \item{XML and Semi-Structured Data}
    \item{Web Services and Middleware}
    \item{Data Integration and Exchange}
    \item{Private and Secure Data Management}
    \item{Peer-to-Peer, Sensornet and Mobile Data Management}
    \item{Scientific and Spatial Data Management}
    \item{Data Brokering and Publish/Subscribe}
    \item{Data Cleaning and Information Extraction}
    \item{Probabilistic Data Management}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Databases, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/DBS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Differential Privacy for Databases}\\
Joseph P. Near and Xi He\\
ISBN: 978-1-68083-850-3\\
\\
\noindent \textit{Database Systems on GPUs}\\
Johns Paul, Shengliang Lu and Bingsheng He\\
ISBN: 978-1-68083-848-0\\
\\
\noindent \textit{Machine Knowledge: Creation and Curation of Comprehensive Knowledge Bases}\\
Gerhard Weikum, Xin Luna Dong, Simon Razniewski and Fabian Suchanek\\
ISBN: 978-1-68083-836-7\\
\\
\noindent \textit{Cloud Data Services: Workloads, Architectures and Multi-Tenancy}\\
Vivek Narasayya and Surajit Chaudhuri\\
ISBN: 978-1-68083-774-2\\
\\
\noindent \textit{Data Provenance}\\
Boris Glavic\\
ISBN: 978-1-68083-828-2\\
\\
\noindent \textit{FPGA-Accelerated Analytics: From Single Nodes to Clusters}\\
Zsolt Istv\'an, Kaan Kara and David Sidler\\
ISBN: 978-1-68083-734-6\\
\\
\noindent \textit{Distributed Learning Systems with First-Order Methods}\\
Ji Liu and Ce Zhango\\
ISBN: 978-1-68083-700-1\\

==> CGV-097-Final Files 2/journaldata/ECO-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{William H. Greene}{New York University\\United States}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Manuel Arellano}{CEMFI Spain}
\journaleditor{Wiji Arulampalam}{University of Warwick}
\journaleditor{Orley Ashenfelter}{Princeton University}
\journaleditor{Jushan Bai}{Columbia University}
\journaleditor{Badi Baltagi}{Syracuse University}
\journaleditor{Anil Bera}{University of Illinois}
\journaleditor{Tim Bollerslev}{Duke University}
\journaleditor{David Brownstone}{UC Irvine}
\journaleditor{Xiaohong Chen}{Yale University}
\journaleditor{Steven Durlauf}{University of Chicago}
\journaleditor{Amos Golan}{American University}
\journaleditor{Bill Griffiths}{University of Melbourne}
\journaleditor{James Heckman}{University of Chicago}
\journaleditor{Jan Kiviet}{University of Amsterdam}
\journaleditor{Gary Koop}{The University of Strathclyde}
\journaleditor{Michael Lechner}{University of St. Gallen}
\journaleditor{Lung-Fei Lee}{Ohio State University}
\journaleditor{Larry Marsh}{Notre Dame University}
\journaleditor{James MacKinnon}{Queens University}
\journaleditor{Bruce McCullough}{Drexel University}
\journaleditor{Jeff Simonoff}{New York University}
\journaleditor{Joseph Terza}{Purdue University}
\journaleditor{Ken Train}{UC Berkeley}
\journaleditor{Pravin Trivedi}{Indiana University}
\journaleditor{Adonis Yatchew}{University of Toronto}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ECO-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ECOcolor}{brickred}   %new color names can be defined before use
\journalcolor      {ECOcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Econometrics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ECO}
\journalurl        {http://www.nowpublishers.com/ECO}
\journalissnprint  {1551-3076}
\journalissnonline {1551-3084}
\journaldoi        {10.1561/08}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Econometrics publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Econometric Models}
    \item{Simultaneous Equation Models}
    \item{Estimation Frameworks}
    \item{Biased Estimation}
    \item{Computational Problems}
    \item{Microeconometrics}
    \item{Treatment Modeling}
    \item{Discrete Choice Modeling}
    \item{Models for Count Data}
    \item{Duration Models}
   \item{Limited Dependent Variables}
    \item{Panel Data}
    \item{Time Series Analysis}
    \item{Latent Variable Models}
    \item{Qualitative Response Models}
    \item{Hypothesis Testing}
    \item{Econometric Theory}
    \item{Financial Econometrics}
    \item{Measurement Error in Survey Data}
    \item{Productivity Measurement and Analysis}
    \item{Semiparametric and Nonparametric Estimation}
    \item{Bootstrap Methods}
    \item{Nonstationary Time Series}
    \item{Robust Estimation}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Econometrics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ECO-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Climate Econometrics: An Overview}\\
Jennifer L. Castle and David F. Hendry\\
ISBN: 978-1-68083-708-7\\
\\
\noindent \textit{Foundations of Stated Preference Elicitation: Consumer Behavior\\ and Choice-based Conjoint Analysis}\\
Moshe Ben-Akiva, Daniel McFadden and Kenneth Train\\
ISBN: 978-1-68083-526-7\\
\\
\noindent \textit{Structural Econometrics of Auctions: A Review}\\
Matthew L. Gentry, Timothy P. Hubbard, Denis Nekipelov and\\ Harry J. Paarsch\\
ISBN: 978-1-68083-446-8\\
\\
\noindent \textit{Data Visualization and Health Econometrics}\\
Andrew M. Jones\\
ISBN: 978-1-68083-318-8\\


==> CGV-097-Final Files 2/journaldata/EDA-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Radu Marculescu}{Carnegie Mellon University}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Robert K. Brayton}{University of California, Berkeley}
\journaleditor{Raul Camposano}{Sage Design Atomation}
\journaleditor{K.T. Tim Cheng}{HKUST}
\journaleditor{Jason Cong}{University of California, Los Angeles}
\journaleditor{Masahiro Fujita}{University of Tokyo}
\journaleditor{Georges Gielen}{KU Leuven}
\journaleditor{Tom Henzinger}{IST Austria}
\journaleditor{Andrew Kahng}{University of California, San Diego}
\columnbreak
\journaleditor{Andreas Kuehlmann}{Synopsys}
\journaleditor{Sharad Malik}{Princeton University}
\journaleditor{Joel Phillips}{Cadence Berkeley Labs}
\journaleditor{Jonathan Rose}{University of Toronto}
\journaleditor{Rob Rutenbar}{University of Pittsburgh}
\journaleditor{Alberto Sangiovanni-Vincentelli}{University of California, Berkeley}
\journaleditor{Leon Stok}{IBM Research}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/EDA-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{EDAcolor}{brickred}   %new color names can be defined before use
\journalcolor      {EDAcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electronic Design Automation}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EDA}
\journalurl        {http://www.nowpublishers.com/EDA}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electronic Design Automation publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{System Level Design}
    \item{Behavioral Synthesis}
    \item{Logic Design}
    \item{Verification}
    \item{Test}
    \item{Physical Design}
    \item{Circuit Level Design}
    \item{Reconfigurable Systems}
    \item{Analog Design}
    \item{Embedded software and parallel programming}
   \item{Multicore, GPU, FPGA, and heterogeneous systems}
    \item{Distributed, networked embedded systems}
    \item{Real-time and cyberphysical systems}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Electronic Design Automation, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/EDA-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Smart Healthcare}\\
Hongxu Yin, Ayten Ozge Akmandor, Arsalan Mosenia and Niraj K. Jha\\
ISBN: 978-1-68083-440-6\\
\\
\noindent \textit{Contracts for System Design}\\
Albert Benveniste, Benoit Caillaud, Dejan Nickovic, Roberto Passerone, Jean-Baptiste Raclet, Philipp Reinkemeier, Alberto Sangiovanni-Vincentelli, Werner Damm, Thomas A. Henzinger and Kim G. Larsen\\
ISBN: 978-1-68083-402-4\\
\\
\noindent \textit{Non-Boolean Computing with Spintronic Devices}\\
Kawsher A. Roxy and Sanjukta Bhanja\\
ISBN: 978-1-68083-362-1

==> CGV-097-Final Files 2/journaldata/EES-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Marija D. Ili\'c}{MIT and Carnegie Mellon University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Hill}{University of Hong Kong and University of Sydney}
\journaleditor{Daniel Kirschen}{University of Washington}
\journaleditor{J. Zico Kolter}{Carnegie Mellon University}
\journaleditor{Chao Lu}{Tsinghua University}
\journaleditor{Steven Low}{California Institute of Technology}
\journaleditor{Ram Rajagopa}{Stanford University}
\journaleditor{Lou van der Sluis}{TU Delft}
\journaleditor{Goran Strbac}{Imperial College London}
\journaleditor{Robert J. Thomas}{Cornell University}
\journaleditor{David Tse}{University of California, Berkeley}
\journaleditor{Le Xie}{Texas A\&M University}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/EES-journaldata.tex <==
\definecolor{cinnabar}{rgb}{0.89, 0.26, 0.2}
\colorlet{EEScolor}{cinnabar}   %new color names can be defined before use
\journalcolor      {EEScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electric Energy Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EES}
\journalurl        {http://www.nowpublishers.com/EES}
\journalissnprint  {2332-6557}
\journalissnonline {2332-6565}
\journaldoi        {10.1561/31}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electric Energy Systems publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Advances in power dispatch}
\item{Demand-side and grid scale data analytics}
\item{Design and optimization of electric services}
\item{Distributed control and optimization of distribution networks}
\item{Distributed sensing for the grid}
\item{Distribution systems}
\item{Fault location and service restoration}
\item{Integration of physics-based and data-driven modeling of future electric energy systems}
\item{Integration of Power electronics, Networked FACTS}
\item{Integration of renewable energy sources}
\item{Interdependence of power system operations and planning and the electricity markets}
\item{Microgrids}
\item{Modern grid architecture}
\item{Power system analysis and computing}
\item{Power system dynamics}
\item{Power system operation}
\item{Power system planning}
\item{Power system reliability}
\item{Power system transients}
\item{Security and privacy}
\item{Stability and control for the whole multi-layer (granulated) network with new load models (to include storage, DR, EVs) and new generation}
\item{System protection and control}
\item{The new stability guidelines and control structures for supporting high penetration of renewables (>50\%)}
\item{Uncertainty quantification for the grid}
\item{System impacts of HVDC}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Electric Energy Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/EES-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Network-Based Analysis of Rotor Angle Stability of Power Systems}\\
Yue Song, David J. Hill and Tao Liu\\
ISBN: 978-1-68083-778-0\\
\\
\noindent \textit{A Survey of Relaxations and Approximations of the Power Flow Equations}\\
Daniel K. Molzahn and Ian A. Hiskens\\
ISBN: 978-1-68083-540-3\\
\\
\noindent \textit{HELM: The Holomorphic Embedding Load-Flow Method. Foundations and Implementations}\\
Antonio Trias\\
ISBN: 978-1-68083-516-8\\
\\
\noindent \textit{Combinatorial Optimization of Alternating Current Electric Power Systems}\\
Sid Chi-Kin Chau\\
ISBN: 978-1-68083-514-4

==> CGV-097-Final Files 2/journaldata/ENT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}
\journalchiefeditor{David B. Audretsch}{Indiana University\\United States}\\
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Howard Aldrich}{University of North Carolina}
\journaleditor{Sharon Alvarez}{University of Denver}
\journaleditor{Per Davidsson}{Queensland University of Technology}
\journaleditor{Michael Frese}{National University of Singapore}
\journaleditor{William B. Gartner}{Copenhagen Business School}
\journaleditor{Magnus Henrekson}{IFN Stockholm}
\journaleditor{Michael A. Hitt}{Texas A\&M University}
\journaleditor{Joshua Lerner}{Harvard University}
\columnbreak
\journaleditor{Jeff McMullen}{Indiana University}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Maria Minniti}{Syracuse University}
\journaleditor{Simon Parker}{University of Western Ontario}
\journaleditor{Holger Patzelt}{TU Munich}
\journaleditor{Saras Sarasvathy}{University of Virginia}
\journaleditor{Roy Thurik}{Erasmus University}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ENT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{ENTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {ENTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Entrepreneurship}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ENT}
\journalurl        {http://www.nowpublishers.com/ENT}
\journalissnprint  {1551-3114}
\journalissnonline {1551-3122}
\journaldoi        {10.1561/03}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Entrepreneurship publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Nascent and start-up entrepreneurs}
\item{Opportunity recognition}
\item{New venture creation process}
\item{Business formation}
\item{Firm ownership}
\item{Market value and firm growth}
\item{Franchising}
\item{Managerial characteristics and behavior of entrepreneurs}
\item{Strategic alliances and networks}
\item{Government programs and public policy}
\item{Gender and ethnicity}
\columnbreak
\item{New business financing:}
	\begin{itemize}
\item{Business angels}
\item{Bank financing, debt, and trade credit}
\item{Venture capital and private equity capital}
\item{Public equity and IPOs} 
\end{itemize}
\item{Family-owned firms}
\item{Management structure, governance and performance}
\item{Corporate entrepreneurship}
\item{High technology:}
	\begin{itemize}
        \item{Technology-based new firms}
        \item{High-tech clusters}
        \end{itemize}
\item{Small business and economic growth}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Entrepreneurship, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ENT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Ambidexterity and Entrepreneurship Studies: A Literature Review and Research Agenda}\\
Maribel Guerrero\\
ISBN: 978-1-68083-818-3\\
\\
\noindent \textit{Innovative Entrepreneurship as a Collaborative Effort: An Institutional Framework}\\
Niklas Elert and Magnus Henrekson\\
ISBN: 978-1-68083-810-7\\
\\
\noindent \textit{Entrepreneurial Finance: Emerging Approaches Using Machine Learning and Big Data}\\
Francesco Ferrati and Moreno Muffatto\\
ISBN: 978-1-68083-804-6\\
\\
\noindent \textit{Advice to Entrepreneurs and Small Business}\\
Kevin Mole\\
ISBN: 978-1-68083-758-2
\\
\noindent \textit{From Ethnic Enclaves to Transnational Landscapes: A Review of Immigrant Entrepreneurship Research}\\
Anuradha Basu and Sarika Pruthi\\
ISBN: 978-1-68083-756-8


==> CGV-097-Final Files 2/journaldata/FIN-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Sheridan Titman}{University of Texas at Austin\\United States}
\end{multicols}

\subsection{Associate Editors}
\begin{multicols}{1}
\journaleditor{Josef Zechner}{WU Vienna University of Economics and Finance}
\journaleditor{Chester Spatt}{Carnegie Mellon University}
\end{multicols}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/FIN-journaldata.tex <==
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\colorlet{FINcolor}{ceruleanblue}   %new color names can be defined before use
\journalcolor      {FINcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Finance}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {FIN}
\journalurl        {http://www.nowpublishers.com/FIN}
\journalissnprint  {1567-2395}
\journalissnonline {1567-2409}
\journaldoi        {10.1561/05}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Finance publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Corporate Finance}
\begin{itemize}
\item{Corporate Governance}
\item{Corporate Financing}
\item{Dividend Policy and Capital Structure}
\item{Corporate Control}
\item{Investment Policy}
\item{Agency Theory and Information}
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Financial Markets}
\begin{itemize}
\item{Market Microstructure}
\item{Portfolio Theory}
\item{Financial Intermediation}
\item{Investment Banking}
\item{Market Efficiency}
\item{Security Issuance}
\item{Anomalies and Behavioral Finance}
\end{itemize}
\end{itemize}
\end{multicols}
%}
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
%\columnbreak
%\begin{itemize}
\item{Asset Pricing}
\begin{itemize}
\item{Asset-Pricing Theory}
\item{Asset-Pricing Models}
\item{Tax Effects}
\item{Liquidity} 
\item{Equity Risk Premium} 
\item{Pricing Models and Volatility} 
\item{Fixed Income Securities} 
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Derivatives}
\begin{itemize}
\item{Computational Finance}
\item{Futures Markets and Hedging}
\item{Financial Engineering}
\item{Interest Rate Derivatives}
\item{Credit Derivatives}
\item{Financial Econometrics}
\item{Estimating Volatilities and Correlations}
\end{itemize}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Finance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/FIN-seriespage.tex <==
\vspace{12pt}

\noindent \textit{The Implications of Heterogeneity and Inequality for Asset Pricing}\\
Stavros Panageas\\
ISBN: 978-1-68083-750-6\\
\\
\noindent \textit{Risk Sharing Within the Firm: A Primer}\\
Marco Pagano\\
ISBN: 978-1-68083-740-7\\
\\
\noindent \textit{The Economics of Credit Rating Agencies}\\
Francesco Sangiorgi and Chester Spatt\\
ISBN: 978-1-68083-380-5\\
\\
\noindent \textit{Initial Public Offerings: A Synthesis of the Literature and Directions for Future Research}\\
Michelle Lowry, Roni Michaely and Ekaterina Volkova\\
ISBN: 978-1-68083-340-9\\
\\
\noindent \textit{Privatization, State Capitalism, and State Ownership of Business in the 21st Century}\\
William L. Megginson\\
ISBN: 978-1-68083-338-6\\

==> CGV-097-Final Files 2/journaldata/HCI-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Youn-Kyung Lim}{Korea Advanced Institute of Science and Technology}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Ben Bederson}{University of Maryland}
\journaleditor{Madeline Balaam}{KTH Royal Institute of Technology}
\journaleditor{Eun Kyoung Choe}{University of Maryland, College Park}
\journaleditor{Andy Cockburn}{University of Canterbury}
\journaleditor{Karrie Karahalios}{University of Illinois at Urbana-Champaign}
\journaleditor{Rohit Ashok Khot}{HAFP Research Lab, RMIT University}
\journaleditor{Uichin Lee}{Korea Advanced Institute of Science and Technology}
\journaleditor{Florian Mueller}{Exertion Games Lab, RMIT University}
\journaleditor{Bilge Mutlu}{University of Wisconsin-Madison}
\journaleditor{Marianna Obrist}{University of Sussex}
\journaleditor{Nuria Oliver}{Telefonica}
\journaleditor{Sameer Patil}{University of Utah}
\journaleditor{Orit Shaer}{Wellesley College}
\journaleditor{Desney S. Tan}{Microsoft Research}
\journaleditor{Koji Yatani}{University of Tokyo}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/HCI-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{HCIcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {HCIcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Human-Computer Interaction}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {HCI}
\journalurl        {http://www.nowpublishers.com/HCI}
\journalissnprint  {1551-3955}
\journalissnonline {1551-3963}
\journaldoi        {10.1561/11}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Human-Computer Interaction publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{History of the research community}
\item{Theory}
\item{Technology}
\item{Computer Supported Cooperative Work}
\item{Interdisciplinary influence}
\item{Advanced topics and trends}
\end{itemize}
%\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Human-Computer Interaction, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/HCI-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Improving HCI with Brain Input: Review, Trends, and Outlook}\\
Erin T. Solovey and Felix Putzer\\
ISBN: 978-1-68083-814-5\\
\\
\noindent \textit{Patient-Generated Health Data: Dimensions, Challenges, and Open Questions}\\
Mayara Costa Figueiredo and Yunan Cheng\\
ISBN: 978-1-68083-668-4\\
\\
\noindent \textit{Patterns and Themes in Designing with Children}\\
Jessica Korte\\
ISBN: 978-1-68083-660-8\\
\\
\noindent \textit{Gender-Inclusive HCI Research and Design: A Conceptual Review}\\
Simone Stumpf, Anicia Peters, Shaowen Bardzell, Margaret Burnett, Daniela Busse, Jessica Cauchard, Elizabeth Churchill\\
ISBN: 978-1-68083-656-1\\


==> CGV-097-Final Files 2/journaldata/ICS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Georges Gielen}{KU Leuven, Belgium}
%\end{multicols*}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alison Burdett}{Sensium Healthcare, UK}
\journaleditor{Malgorzata Chrzanowska-Jeske}{Portland State University, USA}
\journaleditor{Paulo Diniz}{UFRJ, Brazil}
\journaleditor{Peter Kennedy}{University College Dublin, Ireland}
\journaleditor{Maciej Ogorzalek}{Jagiellonian University, Poland}
\journaleditor{Jan van der Spiegel}{University of Pennsylvania, USA}
\journaleditor{Ljiljana Trajkovic}{Simon Fraser University, USA}
%\end{multicols*}

\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ICS-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ICScolor}{brickred}   %new color names can be defined before use
\journalcolor      {ICScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Integrated Circuits and Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ICS}
\journalurl        {http://www.nowpublishers.com/ICS}
\journalissnprint  {2693-9347}
\journalissnonline {2693-9355}
\journaldoi        {10.1561/35}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
 Integrated Circuits and Systems
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Analog, digital and mixed-signal circuits and systems}
\item{RF and mm-wave integrated circuits and systems}
\item{Wireless and wireline communication circuits and systems}
\item{Data converters and frequency generation}
\item{Power electronics and power management circuits}
\item{Biomedical circuits and systems}
\item{Sensor and imager circuits and cyber physical systems}
\item{Security and resilient circuits and systems}
\item{Circuits and systems in emerging non-CMOS technologies}
\item{Circuit theory, modeling, analysis and design methods}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Integrated Circuits and Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ICS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Welcome to the World of Single-Slope Column-Level Analog-to-Digital Converters for CMOS Image Sensors}\\
Albert Theuwissen and Guy Meynants\\
ISBN: 978-1-68083-812-1\\





==> CGV-097-Final Files 2/journaldata/INR-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Maarten de Rijke}{University of Amsterdam \\ and Ahold Delhaize\\The Netherlands}
\journalchiefeditor{Yiqun Liu}{Tsinghua University\\China}
\journalchiefeditor{Diane Kelly}{University of Tennessee\\USA}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Barbara Poblete}{University of Chile}
\journaleditor{Claudia Hauff}{Delft University of Technology}
\journaleditor{Doug Oard}{University of Maryland}
\journaleditor{Ellen M. Voorhees}{National Institute of Standards and Technology}
\journaleditor{Fabrizio Sebastiani}{Consiglio Nazionale delle Ricerche, Italy}
\journaleditor{Hang Li}{Bytedance Technology}
\journaleditor{Isabelle Moulinier}{Capital One}
\journaleditor{Jaap Kamps}{University of Amsterdam}
\journaleditor{Jimmy Lin}{University of Waterloo}
\journaleditor{Leif Azzopardi}{University of Glasgow}
\columnbreak
\journaleditor{Lynda Tamine}{University of Toulouse}
\journaleditor{Mark Sanderson}{RMIT University}
\journaleditor{Rodrygo Luis Teodoro Santos}{Universidade Federal de Minas Gerais}
\journaleditor{Ruihua Song}{Renmin University of China}
\journaleditor{Ryen White}{Microsoft Research}
\journaleditor{Shane Culpepper}{RMIT}
\journaleditor{Soumen Chakrabarti}{Indian Institute of Technology}
\journaleditor{Xuanjing Huang}{Fudan University}
\journaleditor{Zi Helen Huang}{University of Queensland}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/INR-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{INRcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {INRcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Retrieval}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {INR}
\journalurl        {http://www.nowpublishers.com/INR}
\journalissnprint  {1554-0669}
\journalissnonline {1554-0677}
\journaldoi        {10.1561/15}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Retrieval publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Applications of IR}
\item{Architectures for IR}
\item{Collaborative filtering and recommender systems}
\item{Cross-lingual and multilingual IR}
\item{Distributed IR and federated search}
\item{Evaluation issues and test collections for IR}
\item{Formal models and language models for IR}
\item{IR on mobile platforms}
\item{Indexing and retrieval of structured documents}
\item{Information categorization and clustering}
\item{Information extraction}
\item{Information filtering and routing}
\item{Metasearch, rank aggregation and data fusion}
\item{Natural language processing for IR}
\item{Performance issues for IR systems, including algorithms, data structures, optimization techniques, and scalability}
\item{Question answering}
\item{Summarization of single documents, multiple documents, and corpora}
\item{Text mining}
\item{Topic detection and tracking}
\item{Usability, interactivity, and visualization issues in IR}
\item{User modelling and user studies for IR}
\item{Web search}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Retrieval, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 5 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/INR-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Search and Discovery in Personal Email Collections}\\
Michael Bendersky, Xuanhui Wang, Marc Najork and Donald Metzler\\
ISBN: 978-1-68083-838-1\\

\noindent \textit{Extracting, Mining and Predicting Users’ Interests from Social Media}\\
Fattane Zarrinkalam, Stefano Faralli, Guangyuan Piao and Ebrahim Bagheri\\
ISBN: 978-1-68083-738-4\\

\noindent \textit{Knowledge Graphs: An Information Retrieval Perspective}\\
Ridho Reinanda, Edgar Meij and Maarten de Rijke\\
ISBN: 978-1-68083-728-5\\

\noindent \textit{Deep Learning for Matching in Search and Recommendation}\\
Jun Xu, Xiangnan He and Hang Li \\
ISBN: 978-1-68083-706-3\\

\noindent \textit{Explainable Recommendation: A Survey and New Perspectives}\\
Yongfeng Zhang and Xu Chen\\
ISBN: 978-1-68083-658-5\\



==> CGV-097-Final Files 2/journaldata/ISY-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{David Paradice}{Auburn University\\United States}
%\end{multicols}

\subsection{Honorary Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Izak Benbasat}{University of British Columbia}
\journaleditor{Alan R. Dennis}{Kelley School of Business, Indiana University}
\journaleditor{Jacqueline Rees Ulmer}{Iowa State University}
\journaleditor{Veda Storey}{Georgia State University}
\journaleditor{Detmar Straub}{Georgia State University}
\journaleditor{Hugh Watson}{University of Georgia}
%\end{multicols*}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Joey George}{Iowa State University}
\journaleditor{Alan Hevner}{University of South Florida}
\journaleditor{Carol Saunders}{University of Central Florida}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ISY-journaldata.tex <==
\definecolor{regalia}{rgb}{0.32, 0.18, 0.5}
\colorlet{ISYcolor}{regalia}   %new color names can be defined before use
\journalcolor      {ISYcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ISY}
\journalurl        {http://www.nowpublishers.com/ISY}
\journalissnprint  {2331-1231}
\journalissnonline {2331-124X}
\journaldoi        {10.1561/29}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Systems publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{IS and Individuals}
\item{IS and Groups}
\item{IS and Organizations}
\item{IS and Industries}
\item{IS and Society}
\item{IS Development}
\item{IS Economics}
\item{IS Management}
\item{IS Research Methods}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ISY-seriespage.tex <==
\vspace{12pt}
\noindent \textit{IT Project Management: Lessons Learned from Project Retrospectives 1999–2020}\\
R. Ryan Nelson\\
ISBN: 978-1-68083-776-6\\
\\
\noindent \textit{Speech Analytics for Actionable Insights: Current Status, Recommendation, and Guidance}\\
J. P. Shim, Aaron M. French and Bikesh Upreti\\
ISBN: 978-1-68083-696-7\\
\\
\noindent \textit{A Review of Personality in Human–Robot Interactions}\\
Lionel P. Robert Jr., Rasha Alahmad, Connor Esterwood, Sangmi Kim, Sangseok You and Qiaoning Zhang\\
ISBN: 978-1-68083-662-2\\
\\
\noindent \textit{Information Technology and Entrepreneurship: Factors that Shape Investment Support for Innovation}\\
Veda C. Storey and Linda Wallace\\
ISBN: 978-1-68083-602-8


==> CGV-097-Final Files 2/journaldata/MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Tensor Regression}\\
Jiani Liu, Ce Zhu, Zhen Long and Yipeng Liu\\
ISBN: 978-1-68083-886-2\\
\\
\noindent \textit{Minimum-Distortion Embedding}\\
Akshay Agrawal, Alnur Ali and Stephen Boyd\\
ISBN: 978-1-68083-888-6\\
\\
\noindent \textit{Graph Kernels: State-of-the-Art and Future Challenges}\\
Karsten Borgwardt, Elisabetta Ghisu, Felipe Llinares-López, Leslie O’Bray and Bastian Rieck\\
ISBN: 978-1-68083-770-4\\
\\
\noindent \textit{Data Analytics on Graphs Part III: Machine Learning on Graphs, from Graph Topology to Applications}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-16\\
\\
\noindent \textit{Data Analytics on Graphs Part II: Signals on Graphso}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\
\\
\noindent \textit{Data Analytics on Graphs Part I: Graphs and Spectra on Graphs}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\

==> CGV-097-Final Files 2/journaldata/MGT-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{2}\raggedright
\journalchiefeditor{Nicholas S. Argyres}{Olin Business School, Washington University\\United States}
\journalchiefeditor{Timothy M. Devinney}{Leeds University Business School\\United Kingdom}
\journalchiefeditor{James Campbell Quick}{The University of Texas at Arlington\\United States}
\end{multicols}

\subsection{Editors}
\begin{multicols}{3}\raggedright \raggedcolumns
\renewcommand\journaleditor[2]{\par\textbf{#1}\\#2}%
\subsubsection{\footnotesize International Business}

\journaleditor{Gabriel R.G. Benito}{BI Norwegian School of Management}
\journaleditor{Allan Bird}{Northeastern University}
\journaleditor{Julian Birkinshaw}{London Business School}
\journaleditor{Peter Buckley}{University of Leeds}
\journaleditor{Saul Estrin}{London School of Economics}
\journaleditor{Sarianna Lundin}{University of Bremen}
\journaleditor{Xavier Martin}{Tilburg University} 
\journaleditor{Ram Mudambi}{Temple University}

\columnbreak

\subsubsection{\footnotesize Organizational Behavior}

\journaleditor{Myrtle Bell}{University of Texas at Arlington}
\journaleditor{Cary Cooper}{Lancaster University}
\journaleditor{Richard Griffin}{Texas A\&M University}
\journaleditor{Sean Hannah}{Wake Forest University}
\journaleditor{Debra Nelson}{Oklahoma State University}
\journaleditor{Pamela Perrewe}{Florida State University}

\columnbreak

\subsubsection{\footnotesize Strategy}

\journaleditor{Rajshree Agarwal}{University of Maryland}
\journaleditor{Marvin Lieberman}{UCLA}) 
\journaleditor{Michael Lenox}{University of Virginia}
\journaleditor{Joseph Mahoney}{University of Illinois at Urbana-Champaign}
\journaleditor{Jesper Sørensen}{Stanford University}
\journaleditor{Olav Sorenson}{Yale University}
\end{multicols}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/MGT-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{MGTcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {MGTcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MGT}
\journalurl        {http://www.nowpublishers.com/MGT}
\journalissnprint  {2475-6946}
\journalissnonline {2475-6954}
\journaldoi        {10.1561/34}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management publishes
 survey and tutorial articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{International Business}
\item{Organizational Behavior}
\item{Strategic Management}
\end{itemize}
 %\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/MIC-editorialboard.tex <==
%MIC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{W. Kip Viscusi}{Vanderbilt University Law School\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Richard Carson}{University of California, San Diego}
\journaleditor{William Gentry}{Williams College}
\journaleditor{Tom Kniesner}{Syracuse University}
\journaleditor{Mark V. Pauly}{University of Pennsylvania}
\journaleditor{Yossi Spiegel}{Tel Aviv University}
\journaleditor{William Zame}{University of California, Los Angeles}
\journaleditor{James Ziliak}{University of Kentucky}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/MIC-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{MICcolor}{pinegreen}   %new color names can be defined before use   %new color names can be defined before use
\journalcolor      {MICcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Microeconomics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MIC}
\journalurl        {http://www.nowpublishers.com/MIC}
\journalissnprint  {1547-9846}
\journalissnonline {1547-9854}
\journaldoi        {10.1561/07}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Environmental economics}
\item{Health economics}
\item{Industrial organization}
\item{Labor economics}
\item{Law and economics}
\item{Public economics}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/MIC-seriespage.tex <==
\vspace{12pt}
\vspace{12pt}
\noindent \textit{Behavioral Economics of Multiperiod Insurance Purchasing Behavior: The Role of Emotions}\\
Howard Kunreuther and Mark Pauly
\\ISBN: 978-1-68083-524-3
\\
\\
\noindent \textit{Trade and Climate Change: Focus on Carbon Leakage, Border Carbon Adjustments and WTO Consistency}\\
ZhongXiang Zhang
\\ISBN: 978-1-68083-482-6
\\
\\
\noindent \textit{Natural Gas Pipeline Regulation in the United States: Past, Present, and Future}\\
Matthew E. Oliver
\\ISBN: 978-1-68083-452-9
\\
\\
\noindent \textit{The U.S. Market for Uranium: 70 Years of History}\\
Charles F. Mason
\\ISBN: 978-1-68083-382-9
\\
\\
\noindent \textit{Game Theory and Water Resources: Critical Review of its Contributions, Progress and Remaining Challenges}\\
Ariel Dinar and Margaret Hogarth
\\ISBN: 978-1-68083-016-3


==> CGV-097-Final Files 2/journaldata/MKT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Jehoshua Eliashberg}{University of Pennsylvania}

\subsection{Associate Editor}

\journaleditor{Bernd Schmitt}{Columbia University}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dawn Iacobucci}{Vanderbilt University}
\journaleditor{Ganesh Iyeri}{University of California, Berkeley}
\journaleditor{Anirban Mukhopadhyayi}{HKUST}
\journaleditor{Sharon Ngi}{Nanyang Technological University}
\journaleditor{Gerrit van Bruggeni}{Erasmus University}
\journaleditor{Miguel Villas Boasi}{University of California, Berkeley}
\journaleditor{Hema Yoganarasimhani}{University of Washington}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/MKT-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MKTcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MKTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Marketing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MKT}
\journalurl        {http://www.nowpublishers.com/MKT}
\journalissnprint  {1555-0753}
\journalissnonline {1555-0761}
\journaldoi        {10.1561/17}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Marketing publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{B2B Marketing}
\item{Bayesian Models}
\item{Behavioral Decision Making}
\item{Branding and Brand Equity}
\item{Channel Management}
\item{Choice Modeling}
\item{Comparative Market Structure}
\item{Competitive Marketing Strategy}
\item{Conjoint Analysis}
\item{Customer Equity}
\item{Customer Relationship Management}
\item{Game Theoretic Models}
\item{Group Choice and Negotiation}
\item{Discrete Choice Models}
\item{Individual Decision Making}
\item{Marketing Decisions Models}
\item{Market Forecasting}
\item{Marketing Information Systems}
\item{Market Response Models}
\item{Market Segmentation}
\item{Market Share Analysis}
\item{Multi-channel Marketing}
\item{New Product Diffusion}
\item{Pricing Models}
\item{Product Development}
\item{Product Innovation}
\item{Sales Forecasting}
\item{Sales Force Management}
\item{Sales Promotion}
\item{Services Marketing}
\item{Stochastic Model}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Marketing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/MKT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Brands: An Integrated Marketing, Finance, and Societal Perspective}\\
Bobby J. Calder\\
ISBN: 978-1-68083-746-9\\
\\
\noindent \textit{Machine Learning in Marketing: Overview, Learning Strategies, Applications, and Future Developments}\\
Vinicius Andrade Brei\\
ISBN: 978-1-68083-720-9\\
\\
\noindent \textit{Crowdfunding Platforms: Ecosystem and Evolution}\\
Yee Heng Tan and Srinivas K. Reddy\\
ISBN: 978-1-68083-698-1\\
\\
\noindent \textit{A Practical Approach to Sales Compensation: What Do We Know Now? What Should We Know in the Future?}\\
Doug J. Chung, Byungyeon Kim and Niladri B. Syam\\
ISBN: 978-1-68083-684-4\\


==> CGV-097-Final Files 2/journaldata/NET-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Anthony Ephremides}{University of Maryland\\United States}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fran\c{c}ois Baccelli}{University of Texas, Austin}
\journaleditor{Victor Bahl}{Microsoft Research}
\journaleditor{Helmut B\"{o}lcskei}{ETH Zurich}
\journaleditor{J.J. Garcia-Luna Aceves}{UC Santa Cruz}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Roch Guerin}{Washington University in Saint Louis}
\journaleditor{Bruce Hajek}{UIUC}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Frank Kelly}{University of Cambridge}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Steven Low}{Caltech}
\journaleditor{Eytan Modiano}{MIT}
\columnbreak
\journaleditor{Keith Ross}{Polytechnic Institute of NYU}
\journaleditor{Henning Schulzrinne}{Columbia University}
\journaleditor{Mani Srivastava}{UCLA}
\journaleditor{Leandros Tassiulas}{Yale University}
\journaleditor{Lang Tong}{Cornell University}
\journaleditor{Ozan Tonguz}{Carnegie Mellon University}
\journaleditor{Don Towsley}{University of Massachusetts, Amherst}
\journaleditor{Nitin Vaidya}{UIUC}
\journaleditor{Pravin Varaiya}{UC Berkeley}
\journaleditor{Roy Yates}{Rutgers University}
\journaleditor{Raymond Yeung}{Chinese University of Hong Kong}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/NET-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{NETcolor}{cerise}   %new color names can be defined before use
\journalcolor      {NETcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Networking}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {NET}
\journalurl        {http://www.nowpublishers.com/NET}
\journalissnprint  {1554-057X}
\journalissnonline {1554-0588}
\journaldoi        {10.1561/13}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Networking publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Modeling and Analysis of:}
	\begin{itemize}
	\item{Ad Hoc Wireless Networks}
	\item{Sensor Networks}
	\item{Optical Networks}
	\item{Local Area Networks}
	\item{Satellite and Hybrid Networks}
	\item{Cellular Networks}
	\item{Internet and Web Services}
	\end{itemize}
\item{Protocols and Cross-Layer Design}
\item{Network Coding}
\item{Energy-Efficiency Incentives/Pricing/Utility-based}
\item{Games (co-operative or not)}
\item{Security}
\item{Scalability}
\item{Topology}
\item{Control/Graph-theoretic models}
\item{Dynamics and Asymptotic Behavior of Networks}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Networking, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/NET-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Age of Information: A New Concept, Metric, and Tool}\\
Antzela Kosta, Nikolaos Pappas and Vangelis Angelakis\\
ISBN: 978-1-68083-360-7\\
\\
\noindent \textit{Network and Protocol Architectures for Future Satellite Systems}\\
Tomaso de Cola, Alberto Ginesi, Giovanni Giambene,\\ George C. Polyzos, Vasilios A. Siris, Nikos Fotiou and Yiannis Thomas\\
ISBN: 978-1-68083-334-8\\
\\
\noindent \textit{Duality of the Max-Plus and Min-Plus Network Calculus}\\
Jorg Liebeherr\\
ISBN: 978-1-68083-294-5\\
\\
\noindent \textit{Opportunistic Routing in Wireless Networks}\\
Tara Javidi and Eric Van Buhler\\
ISBN: 978-1-68083-150-4

==> CGV-097-Final Files 2/journaldata/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> CGV-097-Final Files 2/journaldata/OPT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Garud Iyengar}{Columbia University, USA}
%\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dimitris Bertsimas}{Massachusetts Institute of Technology}
\journaleditor{John R. Birge}{The University of Chicago}
\journaleditor{Robert E. Bixby}{Rice University}
\journaleditor{Emmanuel Candes}{Stanford University}
\journaleditor{David Donoho}{Stanford University}
\journaleditor{Laurent El Ghaoui}{University of California, Berkeley}
\journaleditor{Donald Goldfarb}{Columbia University}
\journaleditor{Michael I. Jordan}{University of California, Berkeley}
\journaleditor{Zhi-Quan (Tom) Luo}{University of Minnesota, Twin Cites}
\journaleditor{George L. Nemhauser}{Georgia Institute of Technology}
\journaleditor{Arkadi Nemirovski}{Georgia Institute of Technology}
\columnbreak
\journaleditor{Yurii Nesterov}{HSE University}
\journaleditor{Jorge Nocedal}{Northwestern University}
\journaleditor{Pablo A. Parrilo}{Massachusetts Institute of Technology}
\journaleditor{Boris T. Polyak}{Institute for Control Science, Moscow}
\journaleditor{Tam\'as Terlaky}{Lehigh University}
\journaleditor{Michael J. Todd}{Cornell University}
\journaleditor{Kim-Chuan Toh}{National University of Singapore}
\journaleditor{John N. Tsitsiklis}{Massachusetts Institute of Technology}
\journaleditor{Lieven Vandenberghe}{University of California, Los Angeles}
\journaleditor{Robert J. Vanderbei}{Princeton University}
\journaleditor{Stephen J. Wright}{University of Wisconsin}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/OPT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{OPTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {OPTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Optimization}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {OPT}
\journalurl        {http://www.nowpublishers.com/OPT}
\journalissnprint  {2167-3888}
\journalissnonline {2167-3918}
\journaldoi        {10.1561/24}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Optimization publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{algorithm design, analysis, and implementation (especially, on modern computing platforms}
\item{models and modeling systems, new optimization formulations for practical problems}
\item{applications of optimization in machine learning, statistics, and data analysis, signal and image processing, computational economics and finance, engineering design, scheduling and resource allocation, and other areas}
\end{itemize}
 %\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Optimization, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/OPT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Atomic Decomposition via Polar Alignment: The Geometry of Structured Optimization}\\
Zhenan Fan, Halyun Jeong, Yifan Sun and Michael P. Friedlander\\
ISBN: 978-1-68083-742-1\\
\\
\noindent \textit{Optimization Methods for Financial Index Tracking: From Theory to Practice}\\
Konstantinos Benidis, Yiyong Feng and Daniel P. Palomar\\
ISBN: 978-1-68083-464-2\\
\\
\noindent \textit{The Many Faces of Degeneracy in Conic Optimization}\\
Dmitriy Drusvyatskiy and Henry Wolkowicz\\
ISBN: 978-1-68083-390-4\\

==> CGV-097-Final Files 2/journaldata/PGL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Rupak Majumdari}{Max Planck Institute for Software Systems}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and UC Santa Cruz}
\journaleditor{Anindya Banerjee}{IMDEA Software Instituet}
\journaleditor{Patrick Cousot}{ENS, Paris and NYU}
\journaleditor{Oege De Moor}{University of Oxford}
\journaleditor{Matthias Felleisen}{Northeastern University}
\journaleditor{John Field}{Google}
\journaleditor{Cormac Flanagan}{UC Santa Cruz}
\journaleditor{Philippa Gardner}{Imperial College}
\journaleditor{Andrew Gordon}{Microsoft Research and University of Edinburgh}
\journaleditor{Dan Grossman}{University of Washington}
\journaleditor{Robert Harper}{CMU}
\journaleditor{Tim Harris}{Amazon}
\journaleditor{Fritz Henglein}{University of Copenhagen}
\journaleditor{Rupak Majumdar}{MPI and UCLA}
\journaleditor{Kenneth McMillan}{Microsoft Research}
\journaleditor{J. Eliot B. Moss}{University of Massachusetts, Amherst}
\journaleditor{Andrew C. Myers}{Cornell University}
\journaleditor{Hanne Riis Nielson}{Technical University of Denmark}
\journaleditor{Peter O'Hearni}{University College London}
\journaleditor{Benjamin C. Pierce}{University of Pennsylvania}
\journaleditor{Andrew Pittsi}{University of Cambridge}
\journaleditor{Ganesan Ramalingami}{Microsoft Research}
\journaleditor{Mooly Sagiv}{Tel Aviv University}
\journaleditor{Davide Sangiorgi}{University of Bologna}
\journaleditor{David Schmidt}{Kansas State University}
\journaleditor{Peter Sewell}{University of Cambridge}
\journaleditor{Scott Stoller}{Stony Brook University}
\journaleditor{Peter Stuckey}{University of Melbourne}
\journaleditor{Jan Vitek}{Northeastern University}
\journaleditor{Philip Wadler}{University of Edinburgh}
\journaleditor{David Walker}{Princeton University}
\journaleditor{Stephanie Weiric}{University of Pennsylvania}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/PGL-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{PGLcolor}{brickred}   %new color names can be defined before use
\journalcolor      {PGLcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Programming Languages}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {PGL}
\journalurl        {http://www.nowpublishers.com/PGL}
\journalissnprint  {2325-1107}
\journalissnonline {2325-1131}
\journaldoi        {10.1561/25}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Programming Languages publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Abstract Interpretation}
\item{Compilation and Interpretation Techniques}
\item{Domain Specific Languages}
\item{Formal Semantics, including Lambda Calculi, Process Calculi, and Process Algebra}
\item{Language Paradigms}
    \item{Mechanical Proof Checking}
    \item{Memory Management}
    \item{Partial Evaluation}
    \item{Program Logic}
    \item{Programming Language Implementation}
    \item{Programming Language Security}
    \item{Programming Languages for Concurrency}
    \item{Programming Languages for Parallelism}
    \item{Program Synthesis}
    \item{Program Transformations and Optimizations}
    \item{Program Verification}
    \item{Runtime Techniques for Programming Languages}
    \item{Software Model Checking}
    \item{Static and Dynamic Program Analysis}
    \item{Type Theory and Type Systems}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Programming Languages, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/PGL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Shape Analysis}\\
Bor-Yuh Evan Chang, Cezara Drăgoi, Roman Manevich, Noam Rinetzky and Xavier Rival\\
ISBN: 978-1-68083-732-2\\
\\
\noindent \textit{Progress of Concurrent Objects}\\
Hongjin Liang and Xinyu Feng\\
ISBN: 978-1-68083-672-1\\
\\
\noindent \textit{QED at Large: A Survey of Engineering of Formally Verified \\Software}\\
Talia Ringer, Karl Palmskog, Ilya Sergey, Milos Gligoric and \\Zachary Tatlock\\
ISBN: 978-1-68083-594-6\\
\\
\noindent \textit{Reconciling Abstraction with High Performance: A MetaOCaml \\approach}\\
Oleg Kiselyov\\
ISBN: 978-1-68083-436-9

==> CGV-097-Final Files 2/journaldata/ROB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}
\journalchiefeditor{Julie Shah}{Massachusetts Institute of Technology}

\subsection{Honorary Editors}
\journaleditor{Henrik Christensen}{University of California, San Diego}
\journaleditor{Roland Siegwart}{ETH Zurich}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Minoru Asada}{Osaka University}
\journaleditor{Antonio Bicchi}{University of Pisa}
\journaleditor{Aude Billard}{EPFL}
\journaleditor{Cynthia Breazeal}{Massachusetts Institute of Technology}
\journaleditor{Oliver Brock}{TU Berlin}
\journaleditor{Wolfram Burgard}{University of Freiburg}
\journaleditor{Udo Frese}{University of Bremen}
\journaleditor{Ken Goldberg}{University of California, Berkeley}
\journaleditor{Hiroshi Ishiguro}{Osaka University}
\journaleditor{Makoto Kaneko}{Osaka University}
\journaleditor{Danica Kragic}{KTH Stockholm}
\journaleditor{Vijay Kumar}{University of Pennsylvania}
\journaleditor{Simon Lacroix}{LAAS}
\journaleditor{Christian Laugier}{INRIA}
\journaleditor{Steve LaValle}{University of Illinois at Urbana-Champaign}
\journaleditor{Yoshihiko Nakamura}{The University of Tokyo}
\journaleditor{Brad Nelson}{ETH Zurich}
\journaleditor{Paul Newman}{University of Oxford}
\journaleditor{Daniela Rus}{Massachusetts Institute of Technology}
\journaleditor{Giulio Sandini}{University of Genova}
\journaleditor{Sebastian Thrun}{Stanford University}
\journaleditor{Manuela Veloso}{Carnegie Mellon University}
\journaleditor{Markus Vincze}{Vienna University}
\journaleditor{Alex Zelinsky}{DSTG}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/ROB-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{ROBcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {ROBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Robotics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ROB}
\journalurl        {http://www.nowpublishers.com/ROB}
\journalissnprint  {1935-8253}
\journalissnonline {1935-8261}
\journaldoi        {10.1561/23}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Robotics publishes
 survey and tutorial articles in the following topics:
\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Mathematical modelling}
\item{Kinematics}
\item{Dynamics}
\item{Estimation Methods}
\item{Robot Control}
\item{Planning}
\item{Artificial Intelligence in Robotics}
\item{Software Systems and Architectures}
\item{Mechanisms and Actuators}
\item{Sensors and Estimation}
\item{Planning and Control}
\item{Human-Robot Interaction}
\item{Industrial Robotics}
\item{Service Robotics }
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Robotics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/ROB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{A Roadmap for US Robotics – From Internet to Robotics 2020 Edition}\\
Henrik Christensen, Nancy Amato, Holly Yanco, Maja Mataric, Howie Choset, Ann Drobnis, Ken Goldberg, Jessy Grizzle, Gregory Hager, John Hollerbach, Seth Hutchinson, Venkat Krovi, Daniel Lee, Bill Smart, Jeff Trinkle and Gaurav Sukhatme\\
ISBN: 978-1-68083-858-9\\
\\
\noindent \textit{The State of Industrial Robotics: Emerging Technologies, Challenges, and Key Research Directions}\\
Lindsay Sanneman, Christopher Fourie and Julie A. Shah\\
ISBN: 978-1-68083-800-8\\
\\
\noindent \textit{Semantics for Robotic Mapping, Perception and Interaction: A Survey}\\
Sourav Garg, Niko Sünderhauf, Feras Dayoub, Douglas Morrison, Akansel Cosgun, Gustavo Carneiro, Qi Wu, Tat-Jun Chin, Ian Reid, Stephen Gould, Peter Corke and Michael Milford\\
ISBN: 978-1-68083-768-1\\


==> CGV-097-Final Files 2/journaldata/SEC-editorialboard.tex <==
%SEC-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Anupam Datta}{Carnegie Mellon University, USA}
\journalchiefeditor{Jeannette Wing}{Columbia University, USA}


\subsection{Editors}
\begin{multicols}{2}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and University of California, Santa Cruz}
\journaleditor{Michael Backes}{Saarland University}
\journaleditor{Dan Boneh}{Stanford University, USA}
\journaleditor{V\'eronique Cortier}{LORIA, CNRS, France}
\journaleditor{Lorrie Cranor}{Carnegie Mellon University}
\journaleditor{C\'edric Fournet}{Microsoft Research}
\journaleditor{Virgil Gligor}{Carnegie Mellon University}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Deirdre Mulligan}{University of California, Berkeley}
\journaleditor{Andrew Myers}{Cornell University}
\journaleditor{Helen Nissenbaum}{New York University}
\journaleditor{Michael Reiter}{University of North Carolina}
\journaleditor{Shankar Sastry}{University of California, Berkeley}
\journaleditor{Dawn Song}{University of California, Berkeley}
\journaleditor{Daniel Weitzner}{Massachusetts Institute of Technology}
\end{multicols}
\end{editorialboard} 


==> CGV-097-Final Files 2/journaldata/SEC-journaldata.tex <==
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}
\colorlet{SECcolor}{bananayellow}   %new color names can be defined before use
\journalcolor      {SECcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Privacy and Security}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SEC}
\journalurl        {http://nowpublishers.com/SEC}
\journalissnprint  {2474-1558}
\journalissnonline {2474-1566}
\journaldoi        {10.1561/33}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Privacy and Security publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Access control}
\item{Accountability}
\item{Anonymity}
\item{Application security}
\item{Artifical intelligence methods in security and privacy}
\item{Authentication}
\item{Big data analytics and privacy}
\item{Cloud security}
\item{Cyber-physical systems security and privacy}
\item{Distributed systems security and privacy}
\item{Embedded systems security and privacy}
\item{Forensics}
\item{Hardware security}
\item{Human factors in security and privacy}
\item{Information flow}
\item{Intrusion detection}
\item{Malware}
\item{Metrics}
\item{Mobile security and privacy}
\item{Language-based security and privacy}
\item{Network security}
\item{Privacy-preserving systems}
\item{Protocol security}
\item{Security and privacy policies}
\item{Security architectures}
\item{System security}
\item{Web security and privacy}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Privacy and Security, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/SEC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Contextual Integrity through the Lens of Computer Science}\\
Sebastian Benthall, Seda Gurses and Helen Nissenbaum\\
ISBN: 978-1-68083-384-3\\
\\
\noindent \textit{Methods for Location Privacy: A comparative overview}\\
Kostantinos Chatzikokolakis, Ehab ElSalamouny, Catuscia Palamidessi and Pazii Anna\\
ISBN: 978-1-68083-366-9\\
\\
\noindent \textit{Principles and Implementation Techniques of Software-Based Fault Isolation}\\
Gang Tan\\
ISBN: 978-1-68083-344-7\\
\\
\noindent \textit{Modeling and Verifying Security Protocols with the Applied Pi\\ Calculus and ProVerif}\\
Bruno Blanchet\\
ISBN: 978-1-68083-206-8

==> CGV-097-Final Files 2/journaldata/SIG-editorialboard.tex <==
%SIG-Editorialboard.

\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Yonina Eldar}{Weizmann Institute\\Israel}



\subsection{Editors}
\begin{multicols}{3}\raggedcolumns
\journaleditor{Pao-Chi Chang}{National Central University}
\journaleditor{Pamela Cosman}{University of California, San Diego}
\journaleditor{Michelle Effros}{California Institute of Technology}
\journaleditor{Yariv Ephraim}{George Mason University}
\journaleditor{Alfonso Farina}{Selex ES}
\journaleditor{Sadaoki Furui}{Tokyo Institute of Technology}
\journaleditor{Georgios Giannakis}{University of Minnesota}
\journaleditor{Vivek Goyal}{Boston University}
\journaleditor{Sinan Gunturk}{Courant Institute}
\journaleditor{Christine Guillemot}{INRIA}
\journaleditor{Robert W. Heath, Jr.}{The University of Texas at Austin}
\journaleditor{Sheila Hemami}{Northeastern University}
\journaleditor{Lina Karam}{Arizona State University}
\journaleditor{Nick Kingsbury}{University of Cambridge}
\journaleditor{Alex Kot}{Nanyang Technical University}
\journaleditor{Jelena Kovacevic}{New York University}
\journaleditor{Geert Leus}{TU Delft}
\journaleditor{Jia Li}{Pennsylvania State University}
\journaleditor{Henrique Malvar}{Microsoft Research}
\journaleditor{B.S. Manjunath}{University of California, Santa Barbara}
\journaleditor{Urbashi Mitra}{University of Southern California}
\journaleditor{Bj\"{o}rn Ottersten}{KTH Stockholm}
\journaleditor{Vincent Poor}{Princeton University}
\journaleditor{Anna Scaglione}{University of California, Davis}
\journaleditor{Mihaela van der Shaar}{University of California, Los Angeles}
\journaleditor{Nicholas D. Sidiropoulos}{Technical University of Crete}
\journaleditor{Michael Unser}{EPFL}
\journaleditor{P.P. Vaidyanathan}{California Institute of Technology}
\journaleditor{Ami Wiesel}{The Hebrew University of Jerusalem}
\journaleditor{Min Wu}{University of Maryland}
\journaleditor{Josiane Zerubia}{INRIA}
\end{multicols}
\end{editorialboard} 


==> CGV-097-Final Files 2/journaldata/SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/SIG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Recent Advances in Clock Synchronization for Packet-Switched Networks}\\
Anantha K. Karthik and Rick S. Blum\\
ISBN: 978-1-68083-726-1\\
\\
\noindent \textit{Biomedical Image Reconstruction: From the Foundations to Deep Neural Networks}\\
Michael T. McCann and Michael Unser\\
ISBN: 978-1-68083-650-9\\
\\
\noindent \textit{Compressed Sensing with Applications in Wireless Networks}\\
Markus Leinonen, Marian Codreanu and Georgios B. Giannakis\\
ISBN: 978-1-68083-646-2\\

==> CGV-097-Final Files 2/journaldata/STP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/STP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/SYS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Panos J. Antsaklis}{University of Notre Dame\\United States}
\journalchiefeditor{Alessandro Astolfi}{Imperial College London, United Kingdom\\ University of Rome ''Tor Vergata'', Italy}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{John Baillieul}{Boston University}
\journaleditor{Peter Caines}{McGill University}
\journaleditor{Christos Cassandras}{Boston University}
\journaleditor{Denis Dochain}{UC Louvain}
\journaleditor{Magnus Egerstedt}{Georgia Institute of Technology}
\journaleditor{Karl Henrik Johansson}{KTH Stockholm}
\journaleditor{Miroslav Krstic}{University of California, San Diego}
\journaleditor{Jan Maciejowski}{University of Cambridge}
\columnbreak
\journaleditor{Dragan Nesic}{The University of Melbourne}
\journaleditor{Marios Polycarpou}{University of Cyprus}
\journaleditor{J\"{o}rg Raisch}{Technical University Berlin}
\journaleditor{Arjan van der Schaft}{University of Groningen}
\journaleditor{M. Elena Valcher}{University of Padova}
\journaleditor{Richard Vinter}{Imperial College London}
\journaleditor{George Weiss}{Tel Aviv University}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/SYS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet {SYScolor}{cobalt} %new color names can be defined before use
\journalcolor      {SYScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Systems and Control}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SYS}
\journalurl        {http://www.nowpublishers.com/SYS}
\journalissnprint  {2325-6818}
\journalissnonline {2325-6826}
\journaldoi        {10.1561/26}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Systems and Control publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Control of:}
	\begin{itemize}
	\item{Hybrid and Discrete Event Systems}
	\item{Nonlinear Systems}
	\item{Network Systems}
	\item{Stochastic Systems}
	\item{Multi-agent Systems}
	\item{Distributed Parameter Systems}
	\item{Delay Systems}
	\end{itemize}
	\columnbreak
\item{Filtering, Estimation, Identification}
\item{Optimal Control}
\item{Systems Theory}
\item{Control Applications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Systems and Control, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/SYS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Learning-Based Control: A Tutorial and Some Recent Results}\\
Zhong-Ping Jiang, Tao Bian and Weinan Gao\\
ISBN: 978-1-68083-752-0\\
\\
\noindent \textit{Synchronous Reinforcement Learning-Based Control for Cognitive Autonomy}\\
Kyriakos G. Vamvoudakis and Nick-Marios T. Kokolakis\\
ISBN: 978-1-68083-744-5\\
\\
\noindent \textit{Achieving Ecological Resilience Through Regime Shift Management}\\
M. D. Lemmon\\
ISBN: 978-1-68083-716-2\\
\\
\noindent \textit{Distributed Optimization for Smart Cyber-Physical Networks}\\
Giuseppe Notarstefano, Ivano Notarnicola and Andrea Camisa\\
ISBN: 978-1-68083-618-9\\
\\
\noindent \textit{Resilient Control in Cyber-Physical Systems: Countering Uncertainty, Constraints, and Adversarial Behavior}\\
Sean Weerakkody, Omur Ozel, Yilin Mo and Bruno Sinopoli\\
ISBN: 978-1-68083-586-1


==> CGV-097-Final Files 2/journaldata/TCS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Salil Vadhan}{Harvard University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Bernard Chazelle}{Princeton University}
\journaleditor{Oded Goldreich}{Weizmann Institute}
\journaleditor{Shafi Goldwasser}{Massachusetts Institute of Technology and Weizmann Institute}
\journaleditor{Sanjeev Khanna}{University of Pennsylvania}
\journaleditor{Jon Kleinberg}{Cornell University}
\journaleditor{L\'aszl\'o Lov\'asz}{Eötvös Lor\'and University}
\journaleditor{Christos Papadimitriou}{University of California, Berkeley}
\journaleditor{Peter Shor}{Massachusetts Institute of Technology}
\journaleditor{Eva Tardos}{Cornell University}
\journaleditor{Salil Vadhan}{Cornell University}
\journaleditor{Avi Wigderson}{AIS, Princeton University}
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/TCS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{TCScolor}{cobalt}   %new color names can be defined before use
\journalcolor      {TCScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TCS}
\journalurl        {http://www.nowpublishers.com/TCS}
\journalissnprint  {1551-305X}
\journalissnonline {1551-3068}
\journaldoi        {10.1561/04}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Algorithmic game theory}
    \item{Computational algebra}
    \item{Computational aspects of combinatorics and graph theory}
    \item{Computational aspects of communication}
    \item{Computational biology}
    \item{Computational complexity}
    \item{Computational geometry}
    \item{Computational learning}
    \item{Computational Models and Complexity}
    \item{Computational Number Theory}
    \item{Cryptography and information security}
    \item{Data structures}
    \item{Database theory}
    \item{Design and analysis of algorithms}
    \item{Distributed computing}
    \item{Information retrieval}
    \item{Operations Research}
    \item{Parallel algorithms}
    \item{Quantum Computation}
    \item{Randomness in Computation}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/TCS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Higher-order Fourier Analysis and Applications}\\
Hamed Hatami, Pooya Hatami and Shachar Lovett\\
ISBN: 978-1-68083-592-2\\
\\
\noindent \textit{On Doubly-Efficient Interactive Proof Systems}\\
Oded Goldreich \\
ISBN: 978-1-68083-424-6\\
\\
\noindent \textit{Coding for Interactive Communication: A Survey}\\
Ran Gelles\\
ISBN: 978-1-68083-346-1\\

==> CGV-097-Final Files 2/journaldata/TOM-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Panos Kouvelis}{Washington University St. Louis\\USA}

\subsection{Editors}
\journaleditor{Charles Corbett}{UCLA, USA}
\journaleditor{Uday Karmarkar}{UCLA, USA}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Onur Bayabatli}{Singapore Management University, Singapore}
\journaleditor{Jan Fransoo}{Tilburg University, The Netherlands} 
\journaleditor{Chuck Munson}{Washington State University, USA} 
\journaleditor{Nicholas Petruzzi}{Pennsylvania State University, USA}
\journaleditor{Guillaume Roels}{INSEAD, France}
\journaleditor{Nicola Secomandi}{Carnegie-Mellon University, USA} 
\journaleditor{Zuo-Jun Max Shen}{University of California, Berkeley, USA} 
\journaleditor{Sherri Xiaole Wu}{Fudan University, China} 
\journaleditor{Y. Karen Zheng}{MIT, USA} 
%\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/TOM-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{TOMcolor}{cerise}   %new color names can be defined before use
\journalcolor      {TOMcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Technology, Information and Operations Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TOM}
\journalurl        {http://www.nowpublishers.com/TOM}
\journalissnprint  {1571-9545}
\journalissnonline {1571-9553}
\journaldoi        {10.1561/02}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Technology, Information and Operations Management publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{B2B Commerce}
\item{Business Process Engineering and Design}
\item{Business Process Outsourcing}
\item{Capacity Planning}
\item{Competitive Operations}
\item{Contracting in Supply Chains}
\item{E-Commerce and E-Business Models}
\item{Electronic markets, auctions and exchanges}
\item{Enterprise Management Systems}
\item{Facility Location}
\item{Information Chain Structure and Competition}
\item{International Operations}
\item{Marketing/Manufacturing Interfaces}
\item{Multi-location inventory theory}
\item{New Product \& Service Design}
\item{Queuing Networks}
\item{Reverse Logistics}
\item{Service Logistics and Product Support}
\item{Supply Chain Management}
\item{Technology Management and Strategy}
\item{Technology, Information and Operations in:}
	\begin{itemize}
	\item{Automotive Industries}
	\item{Electronics manufacturing}
	\item{Financial Services}
	\item{Health Care}
	\item{Media and Entertainment}
	\item{Process Industries}
	\item{Retailing}
	\item{Telecommunications}
	\end{itemize}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Technology, Information and Operations Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/TOM-seriespage.tex <==
\vspace{12pt}
\noindent \textit{AI and Business Models: The Good, The Bad and The Ugly}\\
Vania Sena and Manuela Nocker
\\ISBN: 978-1-68083-794-0
\\
\\
\noindent \textit{The Business of Electric Vehicles: A Platform Perspective}\\
Jonas Boehm, Hemant K. Bhargava and Geoffrey G. Parker
\\ISBN: 978-1-68083-762-9
\\
\\
\noindent \textit{Advances in Supply Chain Finance and FinTech Innovations Overview}\\
Panos Kouvelis, Ling Dong and Danko Turcic
\\ISBN: 978-1-68083-722-3

==> CGV-097-Final Files 2/journaldata/WEB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}%\raggedcolumns
\journalchiefeditor{Wendy Hall}{University of Southampton, UK}
\journalchiefeditor{Noshir R. Contractor}{Northwestern University, USA}
\journalchiefeditor{Kieron O'Hara}{University of Southampton, UK}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Tim Berners-Lee}{Massachusetts Institute of Technology}
\journaleditor{Noshir Contractor}{Northwestern University}
\journaleditor{Lorrie Crano}{Carnegie Mellon University}
\journaleditor{Dieter Fensel}{University of Innsbruck}
\journaleditor{Carole Goble}{University of Manchester}
\journaleditor{Pat Hayes}{IHMC}
\journaleditor{James Hendler}{Rensselaer Polytechnic Institute}
\journaleditor{Arun Iyengar}{IBM Research}
%\columnbreak
\journaleditor{Craig Knoblock}{University of Southern California}
\journaleditor{Ora Lassila}{Pegasystems}
\journaleditor{Sun Maosong}{Tsinghua University}
\journaleditor{Cathy Marshall}{Microsoft}
\journaleditor{Peter Monge}{University of Southern California}
\journaleditor{Ben Shneiderman}{University of Maryland}
\journaleditor{Danny Weitzner}{Massachusetts Institute of Technology}
\journaleditor{Yorick Wilks}{University of Sheffield}
\end{multicols*}
\end{editorialboard} 

==> CGV-097-Final Files 2/journaldata/WEB-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{WEBcolor}{brickred}   %new color names can be defined before use
\journalcolor      {WEBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Web Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {WEB}
\journalurl        {http://www.nowpublishers.com/WEB}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Web Science publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Agents and the Semantic Web}
    \item{Collective Intelligence}
    \item{Content Management}
    \item{Databases on the Web}
    \item{Data Mining}
    \item{Democracy and the Web}
    \item{Dependability}
    \item{Economics of information and the Web}
    \item{E-Crime}
    \item{E-Government}
    \item{Emergent behaviour}
    \item{Ethics}
    \item{Hypertext/Hypermedia}
    \item{Identity}
    \item{Languages on the Web}
    \item{Memories for Life}
    \item{Mobile/Pervasive}
    \item{Network Infrastructures}
    \item{Performance}
    \item{Privacy}
    \item{Scalability}
    \item{Security}
    \item{Semantic Web}
    \item{Social Networking}
    \item{Standards}
    \item{The Law and the Web}
    \item{The Web as an Educational Tool}
    \item{The Web in the Developing World}
    \item{Trust and Provenance}
    \item{Universal Usability}
    \item{User Interfaces}
    \item{Virtual Reality}
    \item{Web Art}
    \item{Web Governance}
    \item{Search}
    \item{Web Services}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Web Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-097-Final Files 2/journaldata/WEB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{An Introduction to Hybrid Human-Machine Information Systems}\\
Gianluca Demartini, Djellel Eddine Difallah, Ujwal Gadiraju and\\ Michele Catasta\\
ISBN: 978-1-68083-374-4\\
\\
\noindent \textit{Minds Online: The Interface between Web Science, Cognitive Science and the Philosophy of Mind}\\
Paul Smart, Robert Clowes and Richard Heersmink\\
ISBN: 978-1-68083-322-5\\
\\
\noindent \textit{Collective Attention on the Web}\\
Christian Bauckhage and Kristian Kersting\\
ISBN: 978-1-68083-204-4

==> CGV-097-Final Files 2/methods_table.tex <==
\begin{tabular}{llllllllllllllllllllllllll}
\toprule
{} &                                               Name &         FCN & Skip Connections & Boundary Awareness & Multi-scale Feature Maps & Dilated Convolutions & Dynamic Parameters &        RNNs &        LSTM & Deformable Convolution &   Attention &          EM & Graphical representation & 3D segmentation &         GAN & Semi-supervision & Reinforcement Learning & Contour-based & Region Proposals &   One-stage & Meta-learning & Query-based &                                            Summary &                        Benchmarks and Performances &                  Notes \\
\midrule
0  &                                                FCN &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  End-to-end dense learning with fully convoluti... &  PASCAL VOC (62.2), NYUDv2 (34.0), SIFT Flow (3... &                        \\
1  &                                              U-Net &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &                                   Skip connections &                 PhC-U373 (92.03), DIC-HeLa (77.56) &                        \\
2  &                                             SegNet &  \checkmark &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &                                    Pooling indices &                                   SUN-RGBD (31.84) &                        \\
3  &                                                SDS &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Multiscale Combinatorial Grouping (MCN) algori... &                                  PASCAL VOC (52.6) &                        \\
4  &                                                SDN &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  SDN unit - shallow deconvolutional network wit... &    PASCAL VOC (86.6), CamVid (71.8), GATECH (55.9) &                        \\
5  &                                            LSD-Net &  \checkmark &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &               Boundary refinement and RGB-D fusion &                                NYU-Depth v2 (45.9) &                        \\
6  &                                                FPN &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Feature pyramids with top-down and bottom-up p... &                              MS COCO val (AR=48.1) &                        \\
7  &                                             PSPNet &  \checkmark &       \checkmark &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Pyramid Pooling Module that takes global infor... &               PASCAL VOC (85.4), Cityscapes (80.2) &                        \\
8  &                                              DMNet &  \checkmark &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Dynamic Convolutional Module that generates co... &  PASCAL VOC (84.4), ADE20K (45.50), PASCAL-Cont... &                        \\
9  &                                             APCNet &  \checkmark &                  &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Adaptive Context Module that estimate Global-g... &  PASCAL VOC (84.2), ADE20K (45.38), PASCAL-Cont... &                        \\
10 &                                                CCN &  \checkmark &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Selectively aggregation of appropriate scale f... &  Pascal Context (51.6), SUN-RGBD (47.1), COCO S... &                        \\
11 &                                               MSCI &  \checkmark &                  &                    &               \checkmark &                      &                    &             &  \checkmark &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Contextual information exchange through bidire... &  PASCAL VOC (88.0), NYUDv2 (49.0), PASCAL-Conte... &                        \\
12 &                                           ParseNet &  \checkmark &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Global Pooling and simple global feature map i... &  PASCAL VOC (69.8), SIFT Flow (40.4), PASCAL-Co... &                        \\
13 &                                          RefineNet &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Residual Convolution Units for end-to-end trai... &  PASCAL VOC (83.4), ADE20K (40.7), PASCAL-Conte... &                        \\
14 &                                              DANet &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Dual-attention modules for incoporating contex... &  Cityscapes (81.5), PASCAL VOC (82.6), PASCAL-C... &                        \\
15 &                                             PSANet &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Distribute and Collect attention branches for ... &  ADE20K (43.77), PASCAL VOC (85.7), Cityscapes ... &                        \\
16 &                                             GT-OCR &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Aggregation of object region representations b... &  Cityscapes (84.5), LIP (56.65), PASCAL-Context... &                        \\
17 &                                               FaPN &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &             \checkmark &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Feature alignment between top-down and bottom ... &  ADE20K(56.7), Cityscapes (80.0),  COCO-Stuff (... &                        \\
18 &                                          DeepLab3+ &             &                  &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Segmentation quality improvement with atrous c... &                                  PASCAL VOC (89.0) &                        \\
19 &                                         Dilation10 &             &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Aggretation of contextual information through ... &                                  PASCAL VOC (75.3) &                        \\
20 &                                    ResNet-DUC-HDC  &             &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Solve "Gridding" issue from dilated convolutio... &                                  PASCAL VOC (83.1) &                        \\
21 &                                          DenseASPP &             &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Dense multi-scale feature map generation with ... &                                  Cityscapes (80.6) &                        \\
22 &                                               GALD &             &       \checkmark &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Improves small pattern segmentation with Globa... &          Cityscapes (83.3), MS-COCO (Mask AP=37.8) &                        \\
23 &                                               MRFM &             &                  &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Adaptive selection of receptive field and edge... &               PASCAL VOC (88.4), Cityscapes (83.0) &                        \\
24 &                                          SegFormer &             &                  &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Hierarchical Transformer encoder and all-MLP d... &  Cityscapes (84.0), ADE20K(50.3), COCO-Stuff (4... &                        \\
25 &                                             ExFuse &             &                  &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  More effective multi-scale feature fusion with... &                                  PASCAL VOC (87.9) &                        \\
26 &                                              SANet &  \checkmark &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &      Class-wise mask generation for pixel grouping &           PASCAL VOC (86.1), PASCAL-Context (54.4) &                        \\
27 &                                               Swin &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Efficient computation of hierarchical feature ... &              ADE20K (53.5), MS-COCO (Mask AP=51.1) &                        \\
28 &                                            EMA-Net &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &  \checkmark &                          &                 &             &                  &                        &               &                  &             &               &             &  Formulation of attention into Expectation-Maxi... &  PASCAL VOC (88.2), PASCAL-Context (53.1), COCO... &                        \\
29 &                                                DFN &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Application of different weights to different ... &               PASCAL VOC (86.2), Cityscapes (80.3) &                        \\
30 &                                              CCNet &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Impvorves efficiency of attention mechanism wi... &                  ADE20K (45.22), Cityscapes (81.4) &                        \\
31 &                Hierarchical Multi-scale Attention  &             &                  &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Hierarchical attention-based approach that lea... &           Cityscapes test (85.1), Mapillary (61.1) &                        \\
32 &                                         MaskFormer &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Solves semantic and instance segmentation in u... &  ADE20K (55.6), Cityscapes (78.5), COCO-Stuff (... &                        \\
33 &                                            CRF-RNN &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Integrates CRF modeling with CNN by formulatin... &                                  PASCAL VOC (74.7) &                        \\
34 &                                          Piecewise &             &                  &                    &               \checkmark &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Formulates CNN-based general pairwise potentia... &  PASCAL VOC (78.0), NYUDv2 (40.6), SIFT-flow (4... &                        \\
35 &                                                DPN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Solves Markov Random Fields with a single CNN ... &                                  PASCAL VOC (77.5) &                        \\
36 &                                               GCRF &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Unification of Mean Field algorithm with CNN u... &                                  PASCAL VOC (73.2) &                        \\
37 &                                   Domain Transform &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Boundary learning with domain transfer edge-pr... &                                  PASCAL VOC (71.8) &                        \\
38 &                                              GSCNN &             &       \checkmark &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &   Boundary detection improvement with shape stream &                             Cityscapes test (82.8) &                        \\
39 &                                             EncNet &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Context Encoding Module that captures the sema... &  PASCAL-Context (51.7), PASCAL VOC (85.9), ADE2... &                        \\
40 &                                              ReSeg &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Incorporation of contextual information with R... &  CamVid (58.8), Weizmann Horses (91.6), Oxford ... &                        \\
41 &                                            DAG-RNN &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Leveraging long-range contextual information w... &  SIFT Flow (global pixel acc=85.3), CamVid (glo... &                        \\
42 &                                            2D LSTM &             &                  &                    &                          &                      &                    &             &  \checkmark &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Capturing global and local dependencies with 2... &             SIFT Flow (70.11), Stanford BG (78.56) &                        \\
43 &                                            LSTM-CF &             &                  &                    &                          &                      &                    &             &  \checkmark &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Capturing and fusion of contextual information... &                     SUN-RGBD (48.1), NYUDv2 (49.7) &                        \\
44 &                                         Graph LSTM &             &                  &                    &                          &                      &                    &             &  \checkmark &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Modeling natural visual pattern flows with gra... &                         PASCAL-Person-Part (60.35) &                        \\
45 &  Segmenting Images based on natural language ex... &  \checkmark &                  &                    &                          &                      &                    &  \checkmark &  \checkmark &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  End-to-end trainable recurrent convolutional n... &                                    ReferIt (48.03) &                        \\
46 &         Convolutional GAN with weakly-labeled data &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &  \checkmark &       \checkmark &                        &               &                  &             &               &             &         GAN-based CNN leveraging three input types &  all labeled + unlabeled PASCAL VOC (65.8), ful... &                        \\
47 &  Semi-supervised semantic segmentation using an... &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &  \checkmark &       \checkmark &                        &               &                  &             &               &             &  Leveraging unlabeled images to enhance the seg... &  1/2 of PASCAL VOC (73.8), 1/2 of Cityscapes (6... &                        \\
48 &                                              SegAN &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &             \checkmark &               &                  &             &               &             &  Segmentor and a critic network trained in an a... &                  BRATS 2015 test (Dice score=85.0) &                        \\
49 &                                              V-Net &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Loss function based on Dice coefficient for ta... &                     PROMISE2012 (Dice score=82.39) &                        \\
50 &                                             DA-RNN &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Injection of Semantic labels into 3D scenes wi... &        Synthetic ShapeNet Scene dataset (acc=85.9) &                        \\
51 &                                             3D-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &                   3D point cloud data segmentation &  Large Lidar point cloud dataset of the urban a... &                        \\
52 &                                      3DCNN-DQN-RNN &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &      \checkmark &             &                  &             \checkmark &               &                  &             &               &             &  Combining CNN, RNN, and Deep Q-Network for 3D ... &  Stanford 3D semantic parsing (acc=70.76), SUNC... &                        \\
53 &                                           PointNet &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Raw point clouds segmentation with feature tra... &                               ShapeNet part (83.7) &                        \\
54 &                                 Clockwork Convnets &             &                  &                    &                          &                      &         \checkmark &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Clockwork convnets driven by fixed or adaptive... &  Youtube-Objects (70.0), NYUD (28.9), and Citys... &                        \\
55 &                                End2End Voxel2Voxel &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  End-to-end trainable 3D convolutional architec... &                                      GATECH (76.0) &                        \\
56 &                                              RSNet &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Extraction of feature dependencies with slice ... &  S3DIS (51.93),  ScanNet (39.35), ShapeNet (acc... &                        \\
57 &                                                SPG &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &               \checkmark &      \checkmark &             &                  &                        &               &                  &             &               &             &  Novel 3D point cloud representation capturing ... &                   S3DIS (62.1),  Semantic3D (76.2) &                        \\
58 &                                         RandLA-Net &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Random sampling of point clouds and local feat... &            Semantic3D (77.4), SemanticKITTI (53.9) &                        \\
59 &                                            SCF-Net &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Spatial Contextual Feature learning from large... &                   S3DIS (71.6),  Semantic3D (77.6) &                        \\
60 &                                           BAAF-Net &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Local context augmentation with bilateral bloc... &  S3DIS (72.2),  Semantic3D (76.2), SemanticKITT... &                        \\
61 &                                  Point Transformer &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &      Vector self-attention based transformer layer &        S3DIS (73.5), ShapeNetPart (ins. mIoU=86.6) &                        \\
62 &                                         Cylinder3D &             &       \checkmark &                    &                          &                      &         \checkmark &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Cylindrical partition of point clouds and asym... &             SemanticKITTI (67.8), nuScenes (76.1)  &                        \\
63 &      Dense U-Net-based active contour segmentation &             &       \checkmark &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Loss function combining contour length and reg... &  ACDC 2017 Challenge (Hausdorff Dist. is 33.8%,... &                        \\
64 &  Unsupervised Microvascular Image Segmentation ... &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Novel pooling layer mimicking curvature morpho... &                   VesselNN (76.0), DeepVess (83.8) &                        \\
65 &                    Trainable Deep Active Contours  &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Integration of Active Contour Models and CNNs ... &                 Vaihingen (84.0), Bing huts (65.0) &                        \\
66 &                                           DeepMask &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &         Region proposals and object classification &    MS COCO (AR= 36.6), PASCAL VOC 2007 (AR = 43.3) &  Proposal accuracy: AR \\
67 &                                          SharpMask &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Augmenting feedforward nets for object segment... &                                 MS COCO (AR= 39.3) &                        \\
68 &                                       MultiPathNet &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Capturing multi-scale contexts with foveal str... &                             MS COCO (Mask AP=25.0) &                        \\
69 &                                         Mask R-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Extends Faster R-CNN by adding a branch for pr... &  Cityscapes (Mask AP=36.4), MS COCO (ResNeXt-10... &                        \\
70 &                                 Mask Scoring R-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  MaskIoU head trained with simple regression fo... &                             MS COCO (Mask AP=39.6) &                        \\
71 &                                              PANet &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Bottom-up path augmentation; adaptive feature ... &  MS COCO (Mask AP=42.0), Cityscapes (Mask AP=41.4) &                        \\
72 &                                               MNCs &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Three-stage network consisting of instance dif... &  PASCAL VOC (Mask AP(IOU=0.5)=63.5), MS COCO (M... &                        \\
73 &                                        MaskX R-CNN &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Weight transfer function that maps a category’... &                             MS COCO (Mask AP=29.5) &                        \\
74 &                                            MaskLab &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Three branches consisting of box detection, se... &                             MS COCO (Mask AP=43.0) &                        \\
75 &                                                OMN &             &       \checkmark &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  inference of object segment representation bas... &  PASCAL VOC (MASK AP(IOU=0.5)=65.69), Cityscape... &                        \\
76 &                                               FCOS &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Center-ness loss measuring how “centered” is t... &                             MS COCO (Mask AP=44.7) &                        \\
77 &                                         ExtremeNet &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Extreme points used approximate an instance se... &                             MS COCO (Mask AP=34.6) &                        \\
78 &                                           ESE-Seg  &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Using inner center radius shape signature to p... &                             MS COCO (Mask AP=21.6) &                        \\
79 &                                          PolarMask &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Formulating segmentation as  a regression prob... &                             MS COCO (Mask AP=32.9) &                        \\
80 &                                         FourierNet &             &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Obtaining contour points with Inverse Fast Fou... &                             MS COCO (Mask AP=30.6) &                        \\
81 &                                             MEInst &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Mask representation with compact fixed-dimensi... &                             MS COCO (Mask AP=38.2) &                        \\
82 &                                         TensorMask &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Representation of image content (e.g., masks) ... &                             MS COCO (Mask AP=37.3) &                        \\
83 &                                             YOLACT &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Real-time instance segmentation through linear... &                             MS COCO (Mask AP=31.2) &                        \\
84 &                                          BlendMask &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Blender module incorporating rich instance-lev... &                             MS COCO (Mask AP=41.3) &                        \\
85 &                                         CenterMask &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Predicting segmentation mask inside detected b... &                             MS COCO (Mask AP=41.8) &                        \\
86 &                                               SOLO &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Transforms instance segmentation into two pixe... &                             MS COCO (Mask AP=37.8) &                        \\
87 &                                             SOLOv2 &  \checkmark &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Decomposing mask learning to feature learning ... &                             MS COCO (Mask AP=41.7) &                        \\
88 &                                           CondInst &             &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Dynamically generated convolutional filters co... &                             MS COCO (Mask AP=40.1) &                        \\
89 &                           Deep Watershed Transform &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Extraction of object instance segments with en... &                          Cityscapes (Mask AP=19.4) &                        \\
90 &                               Deep Metric Learning &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Clustering pixel embeddings for instance segme... &                PASCAL VOC (MASK AP(IOU=0.5)=62.21) &                        \\
91 &                                 Cascade Mask R-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Progressively improves boudning box quaality w... &                 MS COCO (2017 val)  (Mask AP=42.3) &                        \\
92 &                     Soft Teacher and Box Jittering &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &       \checkmark &             \checkmark &               &                  &             &               &             &  Semi-supervised training with both labeled and... &                             MS COCO (Mask AP=53.0) &                        \\
93 &                                               SOTR &             &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Twin attention mechanism with sparse represent... &                             MS COCO (Mask AP=42.1) &                        \\
94 &                                              DCNAS &             &                  &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &    \checkmark &             &  Direct search of optimal network structure for... &  Cityscapes test (84.3), PASCAL VOC (86.9), ADE... &                        \\
95 &                                                DPC &             &                  &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &    \checkmark &             &  Recursive search space for optimal network str... &  Cityscapes test (82.7), PASCAL VOC (87.9), PAS... &                        \\
96 &                                               DETR &             &                  &                    &                          &                      &         \checkmark &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &  \checkmark &  Set-based global loss that forces unique predi... &                      MS COCO (Panoptic Quality=46) &                        \\
97 &                                          QueryInst &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &  \checkmark &         Parallel supervision on dynamic mask heads &  MS COCO (Mask AP=42.8), Cityscapes (Mask AP=34... &                        \\
\bottomrule
\end{tabular}


==> CGV-097-Final Files 2/new_datasets_tables.tex <==
\begin{tabular}{lllllll}
\toprule
Dataset Name & Object Detection & Semantic Segmentation & Instance Segmentation & Panoptic Segmentation & 3D segmentation & Video segmentation \\
\midrule
  Cityscapes &                  &             checkmark &             checkmark &             checkmark &                 &          checkmark \\
    ShapeNet &                  &             checkmark &                       &                       &       checkmark &                    \\
       S3DIS &                  &             checkmark &                       &                       &       checkmark &                    \\
       NYUv2 &                  &             checkmark &             checkmark &                       &                 &                    \\
     ScanNet &                  &             checkmark &                       &             checkmark &       checkmark &                    \\
       DAVIS &                  &                       &                       &                       &                 &          checkmark \\
      ADE20K &                  &             checkmark &                       &                       &                 &                    \\
   Sun RGB-D &        checkmark &             checkmark &                       &                       &                 &                    \\
  Semantic3D &                  &             checkmark &                       &                       &                 &                    \\
  PASCAL VOC &        checkmark &             checkmark &                       &                       &                 &                    \\
      CamVid &                  &             checkmark &                       &                       &                 &          checkmark \\
         LIP &                  &             checkmark &                       &                       &                 &                    \\
        COCO &        checkmark &             checkmark &             checkmark &             checkmark &                 &                    \\
       KITTI &        checkmark &             checkmark &                       &             checkmark &                 &                    \\
 YouTube-VOS &                  &                       &                       &                       &                 &          checkmark \\
    nuScenes &        checkmark &             checkmark &             checkmark &                       &       checkmark &                    \\
    nuImages &        checkmark &             checkmark &             checkmark &                       &                 &                    \\
        LVIS &        checkmark &                       &             checkmark &                       &                 &                    \\
     PartNet &                  &                       &                       &                       &       checkmark &                    \\
       DRIVE &                  &             checkmark &                       &                       &                 &                    \\
   PROMISE12 &                  &             checkmark &                       &                       &                 &                    \\
\bottomrule
\end{tabular}
\begin{tabular}{lllllll}
\toprule
Dataset Name &                                   Others (Specify) &                                \# of object classes &                                               Size &   Scene &                                              Notes &                                              Links \\
\midrule
  Cityscapes & Image-to-image Translation, Real-Time Semantic ... &                                                 30 & 5000 fine annotated images, 20000 coarse annota... &  street &                                                    &                                                    \\
    ShapeNet &                                  3D Reconstruction &                                               3135 &                  over 300M models, 220k classified & variety & ShapeNet Parts subset contains 31,693 meshes ca... &                                                    \\
       S3DIS &                                                    &                                                 12 &          6 large-scale indoor areas with 271 rooms &  indoor & 3D Instance Segmentation and 3D Semantic Segmen... &                                                    \\
       NYUv2 & 3D Object Detection, Scene Segmentation, Monocu... &                                                 26 & 1449 densely labeled pairs of aligned RGB and d... &  indoor &                                                    &                                                    \\
     ScanNet & Scene Segmentation, 3D Object Detection, Depth ... &                                                 20 & 1513 annotated scans of labeled voxels with an ... &  indoor &                                       2D \& 3D data &                                                    \\
       DAVIS & Interactive Segmentation, Video Denoising, Vide... &                                                    & 50 video sequences with 3455 densely annotated ... & variety &                                                    &                                                    \\
      ADE20K & Image-to-Image Translation, Scene Recognition, ... &                                                150 & 20K scene-centric images exhaustively annotated... & variety & Scene Parsing Benchmark (SceneParse150) is a sm... &                                                    \\
   Sun RGB-D & 3D Object Detection, Monocular 3D Obeject Detec... &                                                700 & 10335 real RGB-D images of room scenes. Each RG... &  indoor &                                                    &                                                    \\
  Semantic3D &                                                    &                                                  8 & over 3 billion points, 15 training and 15 test ... & outdoor &                                                    &                                                    \\
  PASCAL VOC & Weakly-supervised instance segmentation, Weakly... &                                                 20 & 1,464 images for training, 1,449 images for val... & variety &                                                    &                                                    \\
      CamVid &                    Real-Time Semantic Segmentation &                                                 32 &                                         701 frames &  street &                                                    &                                                    \\
         LIP &                                                    &                                                 19 & 50,000 images with elaborated pixel-wise annota... &  people &                                                    &                                                    \\
        COCO & Real-Time Object Detection, Pose Estimation, Ke... & object detection: 80, keypoints detection: 17, ... &                                        328K images & variety &                                                    &                                                    \\
       KITTI & 3D Object Detection, Vehicle Pose Estimation, M... &                                                    & 180 GB sensor streams with images, OXTS, and Ve... &  street & Not all sequences are annotated, i.e. only the ... & http://www.cvlibs.net/publications/Geiger2013IJ... \\
 YouTube-VOS & Visual Object Tracking, One-shot visual object ... &                                               7800 & 4,453 videos, 340+ minutes, labeled with dense ... &         &                                                    &                                                    \\
    nuScenes & 3D Object Detection, 3D Multi-Object Tracking, ... &                                                 10 &                    28130 samples from 1,000 scenes &  street &                                                    &                                                    \\
    nuImages &                                                    &                                                 10 &                            93,000 annotated images &  street &                                                    &                                                    \\
        LVIS &                                                    &                                                1k+ &                                        164k images & variety &                    Has a long tail of rare objects &               https://arxiv.org/pdf/1908.03195.pdf \\
     PartNet &                                                    &                                                 24 &       573,585 part instances over 26,671 3D models &         & annotated with fine-grained, instance-level, an... &                   https://partnet.cs.stanford.edu/ \\
       DRIVE &                         Medical Image Segmentation &                                                    &                                          40 images & medical &                                                    &                                                    \\
   PROMISE12 &                         Medical Image Segmentation &                                                    &                                  50 training cases & medical &                                                    &                                                    \\
\bottomrule
\end{tabular}


==> CGV-097-Final Files 2/panoptic_segmentation.tex <==
\begin{scriptsize}
\begin{longtable}{|L{1.5cm}|L{3.7cm}|L{3.7cm}|L{1cm}|} 
\caption{Summary of Popular Panoptic Segmentation Methods.} \label{tab:panoptic} \\

\hline                         \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances (default metric: PQ (\%))} &                  \textbf{Categorization} \\ \hline
\endfirsthead

\caption* {\textbf{Table 6.1 Continued}}\\

\hline  \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances (default metric: PQ (\%))} &                  \textbf{Categorization} \\
\endhead

\hline \multicolumn{4}{|r|}{{Cont.}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

            JSIS-Net &                                                                                   Joint semantic and instance segmentation with a single network &                                                                                                   COCO panoptic val (26.9) &        Top-down (two-stage) \\ \hline
                 Panoptic FPN &                                        Single network incorporating Feature Pyramid Network that generates instances and segments simultaneously &                                                                                COCO test-dev (40.9); Cityscapes val (58.1) &        Top-down (two-stage) \\ \hline
                  EfficientPS &                                 Shared backbone with 2-way FPN and parallel semantic and instance segmentation heads followed by panoptic fusion &                                                                                        Cityscapes val (67.1); KITTI (43.7) &        Top-down (two-stage) \\ \hline
                Auto-Panoptic &                                           Automatic architectural search for the best backbone, segmentation/instance branches and fusion module &                                                                                COCO panoptic val (44.8); ADE20K val (32.4) &        Top-down (two-stage) \\ \hline
                        OANet &                                                                  Spatial ranking module which addresses occlusions among the predicted instances &                                                                             COCO panoptic val (40.7); COCO test-dev (41.3) &        Top-down (two-stage) \\ \hline
                     OCFusion &                         Model overlap between two instances as a binary relation problem and train it with ground truth from dataset annotations &                                                      COCO panoptic val (46.3); COCO test-dev (46.7); Cityscapes val (60.2) &        Top-down (two-stage) \\ \hline
                       SOGNet &                                 Model the occlusions via a scene overlapping graph where objects are points and relations between them are edges &                                                      COCO panoptic val (43.7); COCO test-dev (47.8); Cityscapes val (60.0) &        Top-down (two-stage) \\ \hline
                       BGRNet &                                                                         Model the correlations between objects and the background with graph CNN &                                                                                COCO panoptic val (43.2); ADE20K val (31.8) &        Top-down (two-stage) \\ \hline
                       UPSNet &                                       Parameter-free panoptic head to merge the predictions from the semantic and instance segmentation networks &                                                      COCO panoptic val (43.2); COCO test-dev (46.6); Cityscapes val (61.8) &        Top-down (two-stage) \\ \hline
        \citet{li2020unifying} &                                                                                   End-to-end panoptic segmentation model without post-processing &                                                      COCO panoptic val (43.4); COCO test-dev (47.2); Cityscapes val (61.4) &        Top-down (two-stage) \\ \hline
                        AUNet &                                               Unified architecture with a foreground and background segmentation branches and a third RPN branch &                                                      COCO panoptic val (39.6); COCO test-dev (46.5); Cityscapes val (59.0) &        Top-down (two-stage) \\ \hline
    \citet{porzi2021improving} &                                                    Bounding box regression loss that addresses the problem caused by using crops during training &                                          Mapillary Vistas val (45.1); Indian Driving Dataset (50.7); Cityscapes val (66.7) &        Top-down (two-stage) \\ \hline
                  Ada-Segment &                                                                                    Automatically adjust multiple training losses during training &                                                                             COCO panoptic val (43.7); COCO test-dev (48.5) &        Top-down (two-stage) \\ \hline
                       FPSNet &                                                              Panoptic segmentation module is formulated into a dense pixel classification module &                                                                                   PASCAL VOC (57.8); Cityscapes val (55.1) &        Top-down (one-stage) \\ \hline
         \citet{Hou_2020_CVPR} &                        Parameter-free method to compute the mask by distilling information from the semantic segmentation and detection branches &                                                                            Cityscapes val (58.8); COCO panoptic val (37.1) &        Top-down (one-stage) \\ \hline
                       EPSNet &                                                 Linear combination of prototype masks and mask coefficients are used to generate the final masks &                                                                             COCO panoptic val (38.6); COCO test-dev (38.9) &        Top-down (one-stage) \\ \hline
               \citet{9466324} &                                  Additional module is added to the detection network to predict the category- and instance-aware pixel embedding &                                                                             COCO panoptic val (45.7); COCO test-dev (46.3) &        Top-down (one-stage) \\ \hline
                    DeeperLab &                        First bottom-up panoptic segmentation approach which parses the image in a single pass over a fully convolutional network &                                                                                               Mapillary Vistas val (31.95) &                 Single-path \\ \hline
             Panoptic-DeepLab &                                               Incorporates dual ASPP for semantic segmentation and dual decoder network for instance segmentation & COCO panoptic val (41.2); COCO test-dev (41.4); Cityscapes val (67.0); Cityscapes test (65.5); Mapillary Vistas val (40.3) &                 Single-path \\ \hline
                Axial-DeepLab &                                                                      Factorizing 2D self-attention into two 1D self-attentions for global region & COCO panoptic val (43.9); COCO test-dev (44.2); Mapillary Vistas val (41.1); Cityscapes val (68.5); Cityscapes test (66.6) &                 Single-path \\ \hline
                 Panoptic FCN &                                                              Using a fully convolutional network for unifying semantic and instance segmentation &                         COCO panoptic val (44.3); COCO test-dev (47.5); Mapillary Vistas val (36.9); Cityscapes val (61.4) &                 Single-path \\ \hline
                        K-Net &                                                                                        Restrict a kernel to predict a single mask for one object &                                                                             COCO panoptic val (54.6); COCO test-dev (55.2) &                 Single-path \\ \hline
                      DR1Mask &                                              Dynamic module to learn a shared feature representation for both semantic and instance segmentation &                                                                             COCO panoptic val (42.9); COCO test-dev (46.1) &                 Single-path \\ \hline
                         DETR &                                            Transformer-based encoder-decoder architecture and bipartite matching for obtaining unique predictions &                                                                                                   COCO panoptic val (45.1) &                 Single-path \\ \hline
                  MaX-DeepLab &                                   First panoptic segmentation model where a masktransformer is trained with a panoptic quality metric based loss &                                                                                                       COCO test-dev (51.3) &                 Single-path \\ \hline
                   MaskFormer &                                                                     Solves semantic and instance segmentation in unison with mask classification &                                                                                                   COCO panoptic val (52.7) &                 Single-path \\ \hline
                   Mask2Former &                                            Masked attention that restricts the attention to localized features centered around predicted segment &                                                                                                   COCO panoptic val (57.8) &                 Single-path \\ \hline
                Bipartite CRF &                                                                                                     Casting panoptic segmentation as a CRF model &                                                      PASCAL VOC (71.76); Cityscapes val (50.299); COCO panoptic val (41.7) &                 Single-path \\ \hline
          \citet{Li_2018_ECCV} &    First weakly-supervised method that jointly produces non-overlapping instance and semantic segmentation for both “thing” and “stuff” classes &                                                                                   PASCAL VOC (63.1); Cityscapes val (53.8) &  Weakly-super\-vised Learning \\ \hline
\citet{yang2020omnisupervised} & Uses unlabeled panoramic images and labeled pinhole images to generate segmentation on panoramic images in an omni-supervised learning framework &                                                                                                      Currently unavailable &  Weakly-super\-vised Learning \\ \hline
                       VPSNet &                                                    Proposes the task of video panoptic segmentation and re-organizes the synthetic VIPER dataset &                                                          VIPER (PQ=55.4, VPQ=51.9), Cityscapes-VPS val (PQ=62.2, VPQ=56.1) & Video Panoptic Segmentation \\ \hline
                  ViP-DeepLab &                            Jointly performs video panoptic segmentation and monocular depth estimation and solves the inverse projection problem &                                                                                              Cityscapes-VPS val (VPQ=63.1) & Video Panoptic Segmentation \\ \hline
    \citet{graber2021panoptic} &                                                       Predict the panoptic segmentation of future frames of video given a set of observed frames &                                                                                                      Cityscapes val (49.0) & Video Panoptic Segmentation \\ \hline
               \citet{9340837} &                              Single-stage real-time point cloud panoptic segmentation using a shared encoder and a semantic and instance decoder &                                                                                                  SemanticKITTI test (65.8) &          LiDAR Point Clouds \\ \hline
                       DS-Net &                                                        Dynamic shifting module to address the problems caused by uneven point cloud distribution &                                                   SemanticKITTI val (57.7); SemanticKITTI test (55.9); nuScenes val (42.5) &          LiDAR Point Clouds \\ \hline
            Panoptic-PolarNet &                                                  Combines 3D semantic predictions with PolarNet and 2D instance predictions with majority voting &                                                   SemanticKITTI val (59.1); SemanticKITTI test (54.1); nuScenes val (67.7) &          LiDAR Point Clouds \\ \hline
                     Panoster &                                                               Clustering pixels via a loss function instead of grouping pixels in multiple steps &                                                                        SemanticKITTI val (55.6); SemanticKITTI test (52.7) &          LiDAR Point Clouds \\ \hline
\end{longtable}
\end{scriptsize}

==> CGV-097-Final Files 2/polarization_seg.tex <==
\section{Polarization Driven Semantic Segmentation}
For effective and robust segmentation, using RGB cameras alone is not sufficient. Low illumination, mirror-like reflections, poor visibility due to rain and fog can severely degrade segmentation performance \citep{li2022unconventional}. One of the emerging imaging technologies that are used for segmentation is a polarization cameras. Polarization is a property that refers to the orientation of light wave's oscillation. Natural light can be converted to polarized light via reflection from surfaces \citep{li2022unconventional}. Imaging sensors can consist of a polarizer that polarizes light in a particular orientation - which is then easy to analyze in vision systems. This has already shown improvement in car detection on roads \citep{blin2019road,blin2020new}. Other works have demonstrated empirical improvement in car and window segmentation based on polarization features \citep{blanchon2019outdoor,xiang2021polarization}. \citet{xiang2021polarization} propose a polarization driven architecture called EAFNet for semantic segmentation by fusing the polarization and conventional features. They also propose a new RGB-P dataset that comprise of 394 annotated pixel aligned RGB-polarization images. Other modalities (like thermal and depth information) are fused along with polarization in \citet{yan2021nlfnet} for multimodal semantic segmentation. 

==> CGV-097-Final Files 2/seg_largeFoV.tex <==
\let\mysectionmark\sectionmark
\renewcommand\sectionmark[1]{}
\section[Semantic Segmentation in Large Field of View (FoV) \\ Images]{Semantic Segmentation in Large Field of View (FoV) Images}
\let\sectionmark\mysectionmark
\sectionmark{Semantic Segmentation in Large Field of View (FoV) Images}
With rapid advancement in visual understanding, parsing a scene is not limited to low FoV images captured with a pinhole camera. This has led to wide FoV image capturing systems such as fisheye cameras, surround view cameras etc. These systems provide a 360\degree~holistic understanding of the visual world and their applications range from self-driving cars, security cameras to atmospheric inspection from satellite images. However, segmenting these images requires expensive training data so various workarounds are proposed in the research community to alleviate this issue. 

\subsection{Fisheye Segmentation}
A fisheye camera captures scenes with an 180\degree~FoV or sometimes more. This results in more information captured compared to traditional pinhole cameras. \citet{deng2017cnn} are the first to propose a system for fisheye image segmentation where the authors begin with a pinhole segmentation dataset \citep{cordts2016cityscapes} and convert it to a synthetic one. They refer to this process as zoom augmentation. This is then used to train a deep CNN-based model. \citet{blott2018semantic} propose a fisheye segmentation framework which does not require an expensive training data generation step. Their core contribution is to use a projection model transformation to convert rectilinear images to fisheye images and design a CNN based model to train on this dataset. \citet{deng2019restricted} propose Restricted Deformable Convolution (RDC) to address the large distortion issue in fisheye images. Their proposed multi-task learning architecture trains an end-to-end segmentation model with a new loss weighting method for real images and the transformed images. They test this system using surround-view cameras (four fisheye cameras providing 360\degree~view of the scene). \citet{ye2020universal} propose a seven degree of freedom (DoF) augmentation framework for transforming rectilinear images to synthetic fisheye images. This is then applied to road scene segmentation on urban driving images. Similarly, \citet{dufour2020instance} propose an augmentation method for instance segmentation on fisheye images. 

\subsection{Panoramic Segmentation}
Another type of visual scene is captured by a panoramic annular lens which creates less distortion and is more compact than fisheye optical system.  \citet{yang2019can} propose the Panoramic Annular Semantic Segmentation (\textbf{PASS}) framework that segments images from a single panoramic annular lens camera with a distortion of less than 1\%. They train with pinhole camera images and pair it with a network adaptation strategy to use the similarity between pinhole features and the features from panoramic segments with a similar FoV. An improvement to PASS is proposed by \citet{yang2020ds} using attention between the low-level encoder layers and the high-level decoder layers. Their proposed model is more efficient than PASS and they apply their method to robotics as well as vehicles. \citet{yang2020omnisupervised} leverage omnisupervised learning in a multi-task framework which was extended by \citet{yang2021capturing}. Doing away with the issue of not taking global context into account and high latency of PASS/DS-PASS methods, \citet{yang2021capturing} propose Efficient Concurrent Attention Networks (\textbf{ECANets}) that capture omni-range dependencies across the 360\degree~FoV. The model also integrates unlabeled full-size panoramic images into the training strategy. They also contribute WildPASS dataset which comprises panoramic images collected from 6 continents and 65 cities. \citet{yang2021context} extend the context-aware omnisupervised segmentation model to work in a single pass. Their model jointly extracts vertical and horizontal contextual information in panoramas to integrate them in the multi-source omnisupervised training scheme. \citet{zhang2022bending} propose a distortion-aware transformer-based framework named Transformer for Panoramic Semantic Segmentation (\textbf{Trans4PASS}) integrating deformable patch embedding and deformable MLP modules to handle distortions and mix patches. They also employ Mutual Prototypical Adaptation, a domain adaptation framework that transfers knowledge from the label-rich pinhole to the label-scarce panoramic domain \citep{zhang2022bending}.

There are several works exploring panoramic segmentation from a domain adaptation perspective \citep{ma2021densepass,zhang2021transfer}. Other applications of panoramic segmentation include aerial imagery \citep{sun2021aerial,wang2022high} and panoptic segmentation \citep{jaus2021panoramic}. 

==> CGV-097-Final Files 2/semantic_segmentation.tex <==
\begin{center}
\scriptsize
\begin{longtable}{|L{1.1cm}|L{3.8cm}|L{3.6cm}|L{1.4cm}|} 
\caption{Summary of Popular Semantic Segmentation Methods.} \label{tab:semantic} \\

\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances (default metric: mIoU (\%))} &                  \textbf{Categorization} \\
                               \hline
\endfirsthead

\caption* {\textbf{Table 3.1 Continued}}\\

\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks and Performances (default metric: mIoU (\%))} &                  \textbf{Categorization} \\
                               \hline
\endhead

\hline \multicolumn{4}{|r|}{{Cont.}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

                                                                FCN &                                                                                                                   End-to-end dense learning with fully convolutional layers &                                                                                                           PASCAL VOC (62.2), NYUDv2 (34.0), SIFT Flow (39.5), PASCAL-Context (53.5) &                       FCN-based \\ \hline
                              U-Net &                                                                                                                                                            Skip connections &                                                                                                                                                  PhC-U373 (92.03), DIC-HeLa (77.56) &                       FCN-based \\ \hline
                          DeconvNet &                                                                                                                         First to use deconvolution to generate feature maps &                                                                                                                                                                    PASCAL VOC (72.5) &                   Deconvolution \\ \hline
                             SegNet &                                                                                                                                                             Pooling indices &                                                                                                                                                                    SUN-RGBD (31.84) &                   Deconvolution \\ \hline
                                SDN &                                                                   SDN unit - shallow deconvolutional network with two downsampling blocks followed by two upsampling blocks &                                                                                                                                     PASCAL VOC (86.6), CamVid (71.8), GATECH (55.9) &                   Deconvolution \\ \hline
                            LSD-Net &                                                                                                                                        Boundary refinement and RGB-D fusion &                                                                                                                                                                 NYU-Depth v2 (45.9) &                   Deconvolution \\ \hline
                                FPN &                                                                                                                      Feature pyramids with top-down and bottom-up pathways  &                                                                                                                                                               MS COCO val (AR=48.1) & Multi-resolution Features-based \\ \hline
                             PSPNet &                                                                            Pyramid Pooling Module that takes global information into account while making local predictions &                                                                                                                                                PASCAL VOC (85.4), Cityscapes (80.2) & Multi-resolution Features-based \\ \hline
                              DMNet &                                                                                                           Dynamic Convolutional Module that generates context-aware filters &                                                                                                                            PASCAL VOC (84.4), ADE20K (45.50), PASCAL-Context (54.4) & Multi-resolution Features-based \\ \hline
                                CCN &                                                                                                        Selective aggregation of appropriate scale features with gated sum &                                                                                                                           Pascal Context (51.6), SUN-RGBD (47.1), COCO Stuff (35.7) & Multi-resolution Features-based \\ \hline
                               MSCI &                                                   Contextual information exchange through bidirectional connections between high-resolution and low-resolution feature maps &                                                                                                            PASCAL VOC (88.0), NYUDv2 (49.0), PASCAL-Context (50.3), SUN-RGBD (50.4) & Multi-resolution Features-based \\ \hline
                           ParseNet &                                                                                                                   Global pooling and simple global feature map incoporation &                                                                                                                          PASCAL VOC (69.8), SIFT Flow (40.4), PASCAL-Context (40.4) & Multi-resolution Features-based \\ \hline
                          RefineNet &                                                              Residual Convolution Units for end-to-end training and chained residual pooling for multi-scale context fusion &                                                                                                            PASCAL VOC (83.4), ADE20K (40.7), PASCAL-Context (47.3), SUN-RGBD (45.9) & Multi-resolution Features-based \\ \hline
                               FaPN &                                                        Feature alignment between top-down and bottom-up pathways with Feature Selection Module and Feature Alignment Module &                                                                                                                                 ADE20K(56.7), Cityscapes (80.0),  COCO-Stuff (40.6) & Multi-resolution Features-based \\ \hline
                             ExFuse &                                                                                                           More effective multi-scale feature fusion with semantic embedding &                                                                                                                                                                   PASCAL VOC (87.9) & Multi-resolution Features-based \\ \hline
                             APCNet &                                                   Adaptive Context Module that estimate Global-guided Local Affinity coefficients for dynamic weight assignments for pixels &                                                                                                                            PASCAL VOC (84.2), ADE20K (45.38), PASCAL-Context (54.7) & Multi-resolution Features-based \\ \hline
                         DilatedNet &                                                                             Aggretation of contextual information through dilated convolutions with multiple sampling rates &                                                                                                                                                                   PASCAL VOC (75.3) &        Atrous convolution-based \\ \hline
                          DeepLab3+ &                                                     Segmentation quality improvement with atrous convolution, atrous spatial pyramid pooling, and conditional random fields &                                                                                                                                                                   PASCAL VOC (89.0) &        Atrous convolution-based \\ \hline
                    ResNet-DUC-HDC  &                 Solve ``Gridding'' issue from dilated convolutions using hybrid dilated convolutions; achieve improved pixel-level decoding with Dense Upsampling Convolution &                                                                                                                                                                   PASCAL VOC (83.1) &        Atrous convolution-based \\ \hline
                          DenseASPP &                                                                                         Dense multi-scale feature map generation with densely connected atrous convolutions &                                                                                                                                                                   Cityscapes (80.6) &        Atrous convolution-based \\ \hline
                               GALD &                                                                            Improves small pattern segmentation with Global Aggregation Module and Local Distribution Module &                                                                                                                                           Cityscapes (83.3), MS-COCO (Mask AP=37.8) &        Atrous convolution-based \\ \hline
                               MRFM &                                                                                                          Adaptive selection of receptive field and edge-aware loss function &                                                                                                                                                PASCAL VOC (88.4), Cityscapes (83.0) &        Atrous convolution-based \\ \hline
                              DANet &                                                                                                              Dual-attention modules for incoporating contextual information &                                                                                                      Cityscapes (81.5), PASCAL VOC (82.6), PASCAL-Context (52.6), COCO Stuff (39.7) &                 Attention-based \\ \hline
                             PSANet &                                                                                                       Distribute and collect attention branches for feature representations &                                                                                                                                ADE20K (43.77), PASCAL VOC (85.7), Cityscapes (81.4) &                 Attention-based \\ \hline
                             GT-OCR &                                                         Aggregation of object region representations based on the relationship between object regions and contextual pixels &                                                                                             Cityscapes (84.5), LIP (56.65), PASCAL-Context (56.2), ADE20K(45.66), COCO Stuff (40.5) &                 Attention-based \\ \hline
                          SegFormer &                                                                                                                        Hierarchical Transformer encoder and all-MLP decoder &                                                                                                                                  Cityscapes (84.0), ADE20K(50.3), COCO-Stuff (46.7) &                 Attention-based \\ \hline
                            EMA-Net &                                                                          Formulation of attention into Expectation-Maximization for efficient computation of attention maps &                                                                                                                         PASCAL VOC (88.2), PASCAL-Context (53.1), COCO-Stuff (39.9) &                 Attention-based \\ \hline
                                DFN &                         Application of different weights to different channels using Channel Attention Block to improve intra-class consistency and inter-class distinction &                                                                                                                                                PASCAL VOC (86.2), Cityscapes (80.3) &                 Attention-based \\ \hline
                              SANet &                                                                                                                               Class-wise mask generation for pixel grouping &                                                                                                                                            PASCAL VOC (86.1), PASCAL-Context (54.4) &                 Attention-based \\ \hline
                               Swin &                                                                         Efficient computation of hierarchical feature maps with shifted windows and effective patch merging &                                                                                                                                               ADE20K (53.5), MS-COCO (Mask AP=51.1) &                 Attention-based \\ \hline
                              CCNet &                                                                                               Improves efficiency of attention mechanism with criss-cross path connections &                                                                                                                                                   ADE20K (45.22), Cityscapes (81.4) &                 Attention-based \\ \hline
\citet{chen2016attention}  &                                                                          Hierarchical attention-based approach that learns relative attention mask between adjacent scales  &                                                                                                                                            Cityscapes test (85.1), Mapillary (61.1) &                 Attention-based \\ \hline
                         MaskFormer &                                                                                                Solves semantic and instance segmentation in unison with mask classification &                                                                                                                                 ADE20K (55.6), Cityscapes (78.5), COCO-Stuff (37.1) &                 Attention-based \\ \hline
                         Mask2-Former &                                                                       Masked attention that restricts the attention to localized features centered around predicted segment &                                                                                                                                                    ADE20K (56.4), Cityscapes (83.3) &                 Attention-based \\ \hline
                            CRF-RNN &                                                                                   Integrates CRF modeling with CNN by formulating CRF as RNN using Mean Field Approximation &                                                                                                                                                                   PASCAL VOC (74.7) &                Graphical models \\ \hline
                          Piecewise & Formulates CNN-based general pairwise potential functions in CRFs to explicitly model patch-patch semantic relations; approximate training using piecewise training of CRFs &                                                                                                                                  PASCAL VOC (78.0), NYUDv2 (40.6), SIFT-flow (44.9) &                Graphical models \\ \hline
                                DPN &                           Solves Markov Random Fields with a single CNN while incoporating high-order relations and mixtures of label contexts with pairwise terms modeling &                                                                                                                                                                   PASCAL VOC (77.5) &                Graphical models \\ \hline
                               GCRF &                                               Unification of Mean Field algorithm with CNN using Gaussian CRFs and fixed number unfolding of Gaussian mean field iterations &                                                                                                                                                                   PASCAL VOC (73.2) &                Graphical models \\ \hline
                   Domain Transform &                                                                                              Boundary learning with domain transfer edge-preserving filter with unified CNN &                                                                                                                                                                   PASCAL VOC (71.8) &      Other contextual knowledge \\ \hline
                              GSCNN &                                                                                                                            Boundary detection improvement with shape stream &                                                                                                                                                              Cityscapes test (82.8) &      Other contextual knowledge \\ \hline
                             EncNet &                                                Context Encoding Module that captures the semantic context of scenes and selectively highlights class-dependent feature maps &                                                                                                                            PASCAL-Context (51.7), PASCAL VOC (85.9), ADE20K (44.65) &      Other contextual knowledge \\ \hline
                              ReSeg &                                  Incorporation of contextual information with RNN layers that performs horizontal and vertical sweeps of the image and hidden layer outputs &                                                                                                                        CamVid (58.8), Weizmann Horses (91.6), Oxford Flowers (93.7) &                       RNN-based \\ \hline
                            DAG-RNN &                                                                                                  Leveraging long-range contextual information with directed acyclic graphs  &                                                                                SIFT Flow (global pixel acc=85.3), CamVid (global pixel acc=91.6), Barcelona (global pixel acc=74.6) &                       RNN-based \\ \hline
                            2D LSTM &                                                                                                                       Capturing global and local dependencies with 2D LSTM  &                                                                                                                                              SIFT Flow (70.11), Stanford BG (78.56) &                      LSTM-based \\ \hline
                            LSTM-CF &                           Capturing and fusion of contextual information from multiple channels of photometric and depth data with Long Short-Term Memorized Context Fusion &                                                                                                                                                      SUN-RGBD (48.1), NYUDv2 (49.7) &                      LSTM-based \\ \hline
                         Graph LSTM &                                                                                                                       Modeling natural visual pattern flows with graph LSTM &                                                                                                                                                          PASCAL-Person-Part (60.35) &                      LSTM-based \\ \hline
                   \citet{luc2016semantic} &                                             Incorporation of GAN to discriminate between ground truth segmentation maps and the output label maps from segmentation network &                                                                                                                                               PASCAL VOC (73.3), Stanford BG (72.0) &                       GAN-based \\ \hline
                 \citet{souly2017semi} &                                   GAN-based CNN leveraging limited pixel-level annotations, large amount of image-level class labels, and fake data from generative network & all labeled + unlabeled PASCAL VOC (65.8), fully labeled + 2000 unlabeled SIFT Flow (35.1), all labeled + 10k unlabeled Stanford BG (63.3), unlabeled + 11k unlabeled CamVid (58.2) &                       GAN-based \\ \hline
                  \citet{hung2018adversarial} &                               Segmentation network trained by minimizing a multi-task loss composed of a cross-entropyloss, an adversarial loss, and a semi-supervised loss &                                                                                                                                                                   PASCAL VOC (74.9) &                       GAN-based \\ \hline
                              SegAN &                                                                                                            Segmentor and a critic network trained in an alternating fashion &                                                                                                                                                   BRATS 2015 test (Dice score=85.0) &                       GAN-based \\ \hline
                              DCNAS &                                                                 Direct search of optimal network structure for semantic image segmentation within a densely connected space &                                                                                                                           Cityscapes test (84.3), PASCAL VOC (86.9), ADE20K (47.12) &                   Meta-learning \\ \hline
                                DPC &                                                         Recursive search space for optimal network structure represented by a DAG encoding multi-scale context information  &                                                                                                               Cityscapes test (82.7), PASCAL VOC (87.9), PASCAL-Person-Part (71.34) &                   Meta-learning \\ \hline
                                DMAda &                                  Progressively build the adaptability of the models trained on daytime scenes to nighttime with an intermediate twilight domain as a bridge &                                                                                                                                                              Dark Zurich-test(36.1) &               Domain Adaptation \\ \hline
                             DANNet &                                                                                   Multi-target domain adaptation via joint training of relighting and segmentation networks &                                                                                                                                                              Dark Zurich-test(47.7) &               Domain Adaptation \\ \hline
                             CIConv &                                                                                        Trainable layer that generates a domain invariant representation of the input image  &                                                                                                                                                              Dark Zurich-test(41.6) &               Domain Adaptation \\ \hline
                             EDCNet &                                                               Captures dynamic context from event-based data to bridge the domain gap between normal and accident imageries &                                                                                                                                              Cityscapes val (69.4), DADA-seg (28.3) &               Domain Adaptation \\ \hline
                              MMUDA &                                                            Uses Multi-Domain Mixed Sampling (MDMS) to augment the training data and meta-learning for domain generalization &                                                                                                                                                                    DADA-seg (46.97) &               Domain Adaptation \\ \hline
                              E-Net &                                                                                                                                        Compact encoder-decoder architecture &                                                                                                                                                              Cityscapes test (58.3) &                       real-time \\ \hline
                             EDANet &                                                                                  Lightweight point-wise convolution layer, assymetric convolution, and dilated convolution  &                                                                                                                                                              Cityscapes test (67.3) &                       real-time \\ \hline
                             LEDNet &                                                                                                                         Lightweight asymmetric encoder-decoder architecture &                                                                                                                                                              Cityscapes test (70.6) &                       real-time \\ \hline
                              SFNet &                    Flow Alignment Module (FAM) that learns the Semantic Flow between feature maps of adjacent levels and efficiently fuses high-level and low-level feature &                                                                                                                                                              Cityscapes test (80.4) &                       real-time \\ \hline
                            BiSeNet &                                Two-branch model incorporating a Spatial Path for preserving spatial information and a Context Path for obtaining sufficient receptive field &                                                                                                                                                              Cityscapes test (74.7) &                       real-time \\ \hline
                              ICNet &                                                                                   Combines semantic information from low resolution and details from high-resolution images &                                                                                                                                                              Cityscapes test (70.6) &                       real-time \\ \hline
                             LDFNet &                                                                         Two-branch architecture that incorporates luminance, depth, and color information from RGB-D images &                                                                                                                                                              Cityscapes test (71.3) &                       real-time \\ \hline
                             DDRNet &                                                             A  family of efficient backbone architectures with deep dual resolution branches and multiple bilateral fusions &                                                                                                                                                              Cityscapes test (77.4) &                       real-time \\ \hline
                             PIDNet &                                                                                                Three-branch network for parsing detailed, context, and boundary information &                                                                                                                                                              Cityscapes test (80.6) &                       real-time \\ \hline
\end{longtable}
\end{center}

==> CGV-097-Final Files 2/video_segmentation.tex <==
\begin{scriptsize}
\begin{longtable}{|L{1.5cm}|L{3.7cm}|L{3.7cm}|L{1cm}|} 
\caption{Summary of Popular Video Segmentation Methods.} \label{tab:video} \\

\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances} &                  \textbf{Categorization} \\
                               \hline
\endfirsthead

\multicolumn{4}{c}%
{{\bfseries \tablename\ \thetable{} Continued}} \\
\hline \textbf{Name} &                                                                                                                                                           \textbf{Main Contribution} &                                                                                                                                                         \textbf{Benchmarks Performances} &                  \textbf{Categorization} \\
                               \hline
\endhead

\hline \multicolumn{4}{|r|}{{Cont.}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

             SSTVOS &                                                                Uses self-attention to learn to search for similar regions and reference masks in the temporal history of video frames & DAVIS17 val (Jaccard Mean: 75.4), Youtube-VOS 2018 val (Jaccard Seen: 80.9; Jaccard Unseen: 76.6) &   Video Object Segmentation \\ \hline
              MBNM &                                                Identifies regions with motion patterns similar to those of non-object regions to associate static objects with the background &                                                                      DAVIS16 val (Avg MAE: 0.031) &   Video Object Segmentation \\ \hline
             DFNet &                                                                        Capture inherent correlation among video frames through feature distribution from a global perspective &                                                                  DAVIS16 val (Jaccard Mean: 83.4) &   Video Object Segmentation \\ \hline
           3DC-Seg &                                                                                                                      End-to-end 3D convolutions for video object segmentation &                                                                  DAVIS16 val (Jaccard Mean: 84.3) &   Video Object Segmentation \\ \hline
         VideoGCRF &                                                                                                CNN-based per-frame feature extraction and CRF-based spatio-temporal reasoning &                                                                               CamVId (mIoU: 75.2) & Video Semantic Segmentation \\ \hline
Clockwork Convnets & Clockwork convnets driven by fixed or adaptive clock signals that schedule the processing of different layers at different update rates according to their semantic stability &                      Youtube-Objects (mIoU: 70.0), NYUD (mIoU: 28.9), and Cityscapes (mIoU: 64.4) & Video Semantic Segmentation \\ \hline
            TMANet &                                                                                   First framework applying memory and self-attention to build the temporal relation in videos &                                                  CamVId (mIoU: 76.5), Cityscapes val (mIoU: 80.3) & Video Semantic Segmentation \\ \hline
     ETC-MobileNet &                                                              Motion guided temporal loss that enforces the network to assign consistent labels for a pixel across time frames &                                                                               CamVId (mIoU: 76.3) & Video Semantic Segmentation \\ \hline
       Voxel2Voxel &                                                                                                 End-to-end trainable 3D convolutional architecture for voxel-level prediction &                                                                                     GATECH (accuracy: 76.0) & Video Semantic Segmentation \\ \hline
\end{longtable}
\end{scriptsize}

==> CGV-097-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {CGV-097}


==> CGV-097-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {CGV-097}


==> CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Aaron Hertzmann }{Adobe Research, USA}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Facebook}
\journaleditor{Brian Curless}{University of Washington}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{William T. Freeman}{MIT}
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Stanford}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Luc Van Gool}{KU Leuven and ETH Zurich}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Deep Learning for Multimedia Forensics}\\
Irene Amerini, Aris Anagnostopoulos, Luca Maiano and Lorenzo Ricciardi Celsi\\
ISBN: 978-1-68083-854-1\\
\\
\noindent \textit{Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art}\\
Joel Janai, Fatma Güney, Aseem Behl and Andreas Geiger\\
ISBN: 978-1-68083-688-2\\
\\
\noindent \textit{Discrete Graphical Models - An Optimization Perspective}\\
Bogdan Savchynskyy\\
ISBN: 978-1-68083-638-7\\
\\
\noindent \textit{Line Drawings from 3D Models: A Tutorial}\\
Pierre Bénard and Aaron Hertzmann\\
ISBN: 978-1-68083-590-8\\
\\
\noindent \textit{Publishing and Consuming 3D Content on the Web: A Survey}\\
Marco Potenziani, Marco Callieri, Matteo Dellepiane and Roberto Scopigno\\
ISBN: 978-1-68083-536-6\\
\\
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\


==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> cleaned_dataset_tasks.tex <==
\begin{tabulary}{\linewidth}{LLLLLLL}
\toprule
Dataset Name & Object Detection & Semantic Segmentation & Instance Segmentation & Panoptic Segmentation & 3D segmentation & Video segmentation \\
\midrule
  Cityscapes &                  &             \checkmark &             \checkmark &             \checkmark &                 &          \checkmark \\
    ShapeNet &                  &             \checkmark &                       &                       &       \checkmark &                    \\
       S3DIS &                  &             \checkmark &                       &                       &       \checkmark &                    \\
       NYUv2 &                  &             \checkmark &             \checkmark &                       &                 &                    \\
     ScanNet &                  &             \checkmark &                       &             \checkmark &       \checkmark &                    \\
       DAVIS &                  &                       &                       &                       &                 &          \checkmark \\
      ADE20K &                  &             \checkmark &                       &                       &                 &                    \\
   Sun RGB-D &        \checkmark &             \checkmark &                       &                       &                 &                    \\
  Semantic3D &                  &             \checkmark &                       &                       &                 &                    \\
  PASCAL VOC &        \checkmark &             \checkmark &                       &                       &                 &                    \\
      CamVid &                  &             \checkmark &                       &                       &                 &          \checkmark \\
         LIP &                  &             \checkmark &                       &                       &                 &                    \\
        COCO &        \checkmark &             \checkmark &             \checkmark &             \checkmark &                 &                    \\
       KITTI &        \checkmark &             \checkmark &                       &             \checkmark &                 &                    \\
 YouTube-VOS &                  &                       &                       &                       &                 &          \checkmark \\
    nuScenes &        \checkmark &             \checkmark &             \checkmark &                       &       \checkmark &                    \\
    nuImages &        \checkmark &             \checkmark &             \checkmark &                       &                 &                    \\
        LVIS &        \checkmark &                       &             \checkmark &                       &                 &                    \\
     PartNet &                  &                       &                       &                       &       \checkmark &                    \\
       DRIVE &                  &             \checkmark &                       &                       &                 &                    \\
   PROMISE12 &                  &             \checkmark &                       &                       &                 &                    \\
\bottomrule
\end{tabulary}

==> dataset_table.tex <==
\begin{tabular}{llllllllllllllllllllllllllll}
\toprule
{} &                                       Dataset Name & Object Detection & Semantic Segmentation & Instance Segmentation & Panoptic Segmentation & 3D segmentation & Video segmentation &                                   Others (Specify) &                                # of object classes &                                               Size &    Scene &                                              Notes &                                        Unnamed: 12 & Unnamed: 13 & Unnamed: 14 & Unnamed: 15 & Unnamed: 16 & Unnamed: 17 & Unnamed: 18 & Unnamed: 19 & Unnamed: 20 & Unnamed: 21 & Unnamed: 22 & Unnamed: 23 & Unnamed: 24 & Unnamed: 25 & Unnamed: 26 \\
\midrule
0  &                                         Cityscapes &                  &            \checkmark &            \checkmark &            \checkmark &                 &         \checkmark &  Image-to-image Translation, Real-Time Semantic... &                                                 30 &  5000 fine annotated images, 20000 coarse annot... &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
1  &                                           ShapeNet &                  &            \checkmark &                       &                       &      \checkmark &                    &                                  3D Reconstruction &                                               3135 &                  over 300M models, 220k classified &  variety &  ShapeNet Parts subset contains 31,693 meshes c... &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
2  &           Stanford 3D Indoor Scene Dataset (S3DIS) &                  &            \checkmark &                       &                       &      \checkmark &                    &                                                    &                                                 12 &          6 large-scale indoor areas with 271 rooms &   indoor &  3D Instance Segmentation and 3D Semantic Segme... &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
3  &                               NYU-Depth V2 (NYUv2) &                  &            \checkmark &            \checkmark &                       &                 &                    &  3D Object Detection, Scene Segmentation, Monoc... &                                                 26 &  1449 densely labeled pairs of aligned RGB and ... &   indoor &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
4  &                                            ScanNet &                  &            \checkmark &                       &            \checkmark &      \checkmark &                    &  Scene Segmentation, 3D Object Detection, Depth... &                                                 20 &  1513 annotated scans of labeled voxels with an... &   indoor &                                       2D & 3D data &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
5  &  Densely Annotation Video Segmentation dataset ... &                  &                       &                       &                       &                 &         \checkmark &  Interactive Segmentation, Video Denoising, Vid... &                                                    &  50 video sequences with 3455 densely annotated... &  variety &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
6  &                                             ADE20K &                  &            \checkmark &                       &                       &                 &                    &  Image-to-Image Translation, Scene Recognition,... &                                                150 &  20K scene-centric images exhaustively annotate... &  variety &  Scene Parsing Benchmark (SceneParse150) is a s... &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
7  &                                          Sun RGB-D &       \checkmark &            \checkmark &                       &                       &                 &                    &  3D Object Detection, Monocular 3D Obeject Dete... &                                                700 &  10335 real RGB-D images of room scenes. Each R... &   indoor &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
8  &                                         Semantic3D &                  &            \checkmark &                       &                       &                 &                    &                                                    &                                                  8 &  over 3 billion points, 15 training and 15 test... &  outdoor &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
9  &  PASCAL Visual Object Classes Challenge (PASCAL... &       \checkmark &            \checkmark &                       &                       &                 &                    &  Weakly-supervised instance segmentation, Weakl... &                                                    &  1,464 images for training, 1,449 images for va... &  variety &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
10 &  Cambridge-driving Labeled Video Database (CamVid) &                  &            \checkmark &                       &                       &                 &         \checkmark &                    Real-Time Semantic Segmentation &                                                 32 &                                         701 frames &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
11 &                             Look into Person (LIP) &                  &            \checkmark &                       &                       &                 &                    &                                                    &  19 semantic human part labels and 2D human pos... &  50,000 images with elaborated pixel-wise annot... &   people &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
12 &         Microsoft Common Objects in Context (COCO) &       \checkmark &            \checkmark &            \checkmark &            \checkmark &                 &                    &  Real-Time Object Detection, Pose Estimation, K... &  object detection: 80, keypoints detection: 17,... &                                        328K images &  variety &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
13 &  Karlsruhe Institute of Technology and Toyota T... &       \checkmark &            \checkmark &                       &            \checkmark &                 &                    &  3D Object Detection, Vehicle Pose Estimation, ... &                                                    &  180 GB sensor streams with images, OXTS, and V... &   street &  Not all sequences are annotated, i.e. only the... &  http://www.cvlibs.net/publications/Geiger2013I... &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
14 &    YouTube-VOS (Youtube Video Object Segmentation) &                  &                       &                       &                       &                 &         \checkmark &  Visual Object Tracking, One-shot visual object... &                                               7800 &  4,453 videos, 340+ minutes, labeled with dense... &          &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
15 &                                           nuScenes &       \checkmark &            \checkmark &            \checkmark &                       &      \checkmark &                    &  3D Object Detection, 3D Multi-Object Tracking,... &                                                 10 &                    28130 samples from 1,000 scenes &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
16 &                                           nuImages &       \checkmark &            \checkmark &            \checkmark &                       &                 &                    &                                                    &                                                 10 &                            93,000 annotated images &   street &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
17 &      Large Vocabulary Instance Segmentation (LVIS) &       \checkmark &                       &            \checkmark &                       &                 &                    &                                                    &                                                1k+ &                                        164k images &  variety &                    Has a long tail of rare objects &               https://arxiv.org/pdf/1908.03195.pdf &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
18 &                                            PartNet &                  &                       &                       &                       &      \checkmark &                    &                                                    &                                                 24 &       573,585 part instances over 26,671 3D models &          &  annotated with fine-grained, instance-level, a... &                   https://partnet.cs.stanford.edu/ &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
19 &  Digital Retinal Images for Vessel Extraction (... &                  &            \checkmark &                       &                       &                 &                    &                         Medical Image Segmentation &                                                    &                                          40 images &  medical &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
20 &                                          PROMISE12 &                  &            \checkmark &                       &                       &                 &                    &                         Medical Image Segmentation &                                                    &                                  50 training cases &  medical &                                                    &                                                    &             &             &             &             &             &             &             &             &             &             &             &             &             &             \\
\bottomrule
\end{tabular}


==> journaldata/ACC-editorialboard.tex <==
%ACC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

%\journalchiefeditor{Stefan J. Reichelstein}{Stanford University\\United States}



\subsection{Executive Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Jonathan Glover, Editor-in-Chief}{Columbia University}
\journaleditor{Stephen Penman}{Columbia University}
\journaleditor{Stefan J. Reichelstein}{Stanford University and University of Mannheim}
\journaleditor{Dan Taylor}{University of Pennsylvania}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACC-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{ACCcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {ACCcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Accounting}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACC}
\journalurl        {http://www.nowpublishers.com/ACC}
\journalissnprint  {1554-0642}
\journalissnonline {1554-0650}
\journaldoi        {10.1561/14}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Auditing}
\item{Corporate Governance}
\item{Cost Management}
\item{Disclosure}
\item{Event Studies/Market Efficiency Studies}
\item{Executive Compensation}
\item{Financial Reporting}
\item{Management Control}
\item{Performance Measurement}
\item{Taxation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{IFRS: Markets, Practice, and Politics}\\
Kirstin Becker, Jannis Bischof and Holger Daske\\
ISBN: 978-1-68083-830-5
\\
\\
\noindent \textit{Using Python for Text Analysis in Accounting Research}\\
Vic Anand, Khrystyna Bochkay, Roman Chychyla and Andrew Leone\\
ISBN: 978-1-68083-760-5
\\
\\
\noindent \textit{Research on Corporate Sustainability: Review and Directions for Future Research}\\
Jody Grewal and George Serafeim\\
ISBN: 978-1-68083-718-6
\\
\\
\noindent \textit{Field Experiments in Managerial Accounting Research}\\
Sofia M. Lourenco\\
ISBN: 978-1-68083-628-8

==> journaldata/ACG-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Marc Goergen}{IE Business School\\Spain}
\journalchiefeditor{Geoffrey Wood}{Western University\\Canada}

\subsection{Founding Editor}

\editor{Douglas Cumming}{Florida Atlantic University, USA}

\subsection{Associate Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Renee Adams}{University of Oxford}
\journaleditor{Lucian Bebchuk}{Harvard University}
\journaleditor{William Judge}{Old Dominion University}
\journaleditor{Mark Roe}{Harvard University}
\journaleditor{Rene Stulz}{Ohio State University}
\journaleditor{James Westphal}{University of Michigan}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACG-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ACGcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ACGcolor} %a color name. 
\journaltitle      {Annals of Corporate Governance}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACG}
\journalurl        {http://www.nowpublishers.com/ACG}
\journalissnprint  {2381-6724}
\journalissnonline {2381-6732}
\journaldoi        {10.1561/109	}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
Annals of Corporate Governancepublishes
 articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Boards of Directors}
\item{Ownership}
\item{National Corporate Governance Mechanisms}
\item{Comparative Corporate Governance Systems}
\item{Self Governance}
\item{Teaching Corporate Governance}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
 Annals of Corporate Governance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Social Purpose of the Modern Business Corporation}\\
Peter J. Buckley
\\ISBN: 978-1-68083-874-9
\\
\noindent \textit{Decentralized Autonomous Organizations: Internal Governance and External Legal Design}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-798-8
\\
\noindent \textit{Decentralized Corporate Governance via Blockchain Technology}\\
Wulf A. Kaal
\\ISBN: 978-1-68083-676-9
\\
\noindent \textit{Corporate Governance in IPO Firms}\\
Erik E. Lehmann and Silvio Vismara
\\ISBN: 978-1-68083-634-9
\\
\noindent \textit{The Political and Governance Risks of Sovereign Wealth}\\
Paul Rose 
\\ISBN: 978-1-68083-624-0



==> journaldata/ASTP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ASTP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ASTP-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Case Studies of Successful Technology Transfer from Federal Laboratories}\\
Gretchen B. Jordan, Christopher S. Hayter, Michael Hogan, Manuel A. Gonzalez and Alan C. O’Connor\\
ISBN: 978-1-68083-808-4\\

\noindent \textit{Toward More Effective Science and Technology Advice for Congress: The Historical Roots and Pathways Forward}\\
Peter D. Blair\\
ISBN: 978-1-68083-802-2\\

\noindent \textit{The Globalization of the Bayh–Dole Act}\\
Thorsten Gores and Albert N. Link\\
ISBN: 978-1-68083-754-4\\

\noindent \textit{Globalization and the High-Tech Policy Response}\\
Gregory Tassey\\
ISBN: 978-1-68083-690-5\\
\\
\noindent \textit{Evolution of Ireland’s Industrial, Science and Technology Policy}\\
James A. Cunningham, Patrick Collins and Majella Giblin\\
ISBN: 978-1-68083-680-6\\
\\
\noindent \textit{Public Support of Private Innovation: An Initial Assessment of the North Carolina SBIR/STTR Phase I Matching Funds Program}\\
John W. Hardin, David J. Kaiser and Albert N. Link\\
ISBN: 978-1-68083-674-5

==> journaldata/CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Aaron Hertzmann }{Adobe Research, USA}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Facebook}
\journaleditor{Brian Curless}{University of Washington}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{William T. Freeman}{MIT}
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Stanford}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Luc Van Gool}{KU Leuven and ETH Zurich}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Deep Learning for Multimedia Forensics}\\
Irene Amerini, Aris Anagnostopoulos, Luca Maiano and Lorenzo Ricciardi Celsi\\
ISBN: 978-1-68083-854-1\\
\\
\noindent \textit{Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art}\\
Joel Janai, Fatma Güney, Aseem Behl and Andreas Geiger\\
ISBN: 978-1-68083-688-2\\
\\
\noindent \textit{Discrete Graphical Models - An Optimization Perspective}\\
Bogdan Savchynskyy\\
ISBN: 978-1-68083-638-7\\
\\
\noindent \textit{Line Drawings from 3D Models: A Tutorial}\\
Pierre Bénard and Aaron Hertzmann\\
ISBN: 978-1-68083-590-8\\
\\
\noindent \textit{Publishing and Consuming 3D Content on the Web: A Survey}\\
Marco Potenziani, Marco Callieri, Matteo Dellepiane and Roberto Scopigno\\
ISBN: 978-1-68083-536-6\\
\\
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\


==> journaldata/CIT-editorialboard.tex <==
\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{Alexander Barg}{University of Maryland\\USA}

\subsection{Area Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Emmanuel Abbe}{Princeton University}
\journaleditor{Arya Mazumdar}{UMass Amherst}
\journaleditor{Olgica Milenkovic}{University of Illinois, Urbana-Champaign}
\journaleditor{Anelia Somekh-Baruch}{Bar-Ilan University}
\journaleditor{Himanshu Tyagi}{Indian Institute of Science}

\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Venkat Anantharam}{UC Berkeley}
\journaleditor{Giuseppe Caire}{TU Berlin}
\journaleditor{Daniel Costello}{University of Notre Dame}
%\journaleditor{Anthony Ephremides}{University of Maryland}
%\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Albert Guillen i Fabregas}{Pompeu Fabra University}
\journaleditor{Dongning Guo}{Northwestern University}
\journaleditor{Dave Forney}{MIT}
\journaleditor{Te Sun Han}{University of Tokyo}
\journaleditor{Babak Hassibi}{Caltech}
\journaleditor{Michael Honig}{Northwestern University}
%\journaleditor{Tara Javidi}{UC San Diego}

\journaleditor{Ioannis Kontoyiannis}{Cambridge University}
\journaleditor{Gerhard Kramer}{TU Munich}
\journaleditor{Amos Lapidoth}{ETH Zurich}
\journaleditor{Muriel Medard}{MIT}
\journaleditor{Neri Merhav}{Technion}
\journaleditor{David Neuhoff}{University of Michigan}
\journaleditor{Alon Orlitsky}{UC San Diego}
\journaleditor{Yury Polyanskiy}{MIT}
\journaleditor{Vincent Poor}{Princeton University}
%\journaleditor{Maxim Raginsky}{UIUC}
\journaleditor{Kannan Ramchandran}{UC Berkeley}
\journaleditor{Igal Sason}{Technion}
%\columnbreak
\journaleditor{Shlomo Shamai}{Technion}
\journaleditor{Amin Shokrollahi}{EPF Lausanne}
\journaleditor{Yossef Steinberg}{Technion}
\journaleditor{Wojciech Szpankowski}{Purdue University}
\journaleditor{David Tse}{Stanford University}
\journaleditor{Antonia Tulino}{Bell Labs}
\journaleditor{R\"{u}diger Urbanke}{EPF Lausanne}
\journaleditor{Emanuele Viterbo}{Monash University}
\journaleditor{Frans Willems}{TU Eindhoven}
\journaleditor{Raymond Yeung}{CUHK}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CIT-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{CITcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {CITcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Communications and Information Theory}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CIT}
\journalurl        {http://www.nowpublishers.com/CIT}
\journalissnprint  {1567-2190}
\journalissnonline {1567-2328 }
\journaldoi        {10.1561/01}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Communications and Information Theory publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Coded modulation}
\item{Coding theory and practice}
\item{Communication complexity}
\item{Communication system design}
\item{Cryptology and data security}
\item{Data compression}
\item{Data networks}
\item{Demodulation and Equalization}
\item{Denoising}
\item{Detection and estimation}
\item{Information theory and statistics}
\item{Information theory and computer science}
\item{Joint source/channel coding}
\item{Modulation and signal design}
\item{Multiuser detection}
\item{Multiuser information theory}
\item{Optical communication channels}
\item{Pattern recognition and learning}
\item{Quantization}
\item{Quantum information processing}
\item{Rate-distortion theory}
\item{Shannon theory}
\item{Signal processing for communications}
\item{Source coding}
\item{Storage and recording codes}
\item{Speech and Image Compression}
\item{Wireless Communications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Communications and Information Theory, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CIT-seriespage.tex <==
\vspace{12pt}
\\
\noindent \textit{An Algebraic and Probabilistic Framework for Network Information Theory}\\
S. Sandeep Pradhan, Arun Padakandla and Farhad Shirani\\
ISBN: 978-1-68083-766-7\\
\\
\noindent \textit{Theoretical Foundations of Adversarial Binary Detection}\\
Mauro Barni and Benedetta Tondi\\
ISBN: 978-1-68083-764-3\\
\\
\noindent \textit{Polynomial Methods in Statistical Inference}\\
Yihong Wu and Pengkun Yang\\
ISBN: 978-1-68083-730-8\\
\\
\noindent \textit{Information-Theoretic Foundations of Mismatched Decoding}\\
Jonathan Scarlett, Albert Guillen i Fabregas, Anelia Somekh-Baruch and Alfonso Martinez\\
ISBN: 978-1-68083-712-4\\
\\
\noindent \textit{Coded Computing: Mitigating Fundamental Bottlenecks in Large-Scale Distributed Computing and Machine Learning}\\
Songze Li and Salman Avestimehr \\
ISBN: 978-1-68083-704-9



==> journaldata/DBS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Joseph M. Hellerstein}{University of California at Berkeley\\United States}
\journalchiefeditor{Surajit Chaudhuri}{Microsoft Research, Redmond\\United States}



\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Azza Abouzied}{NYU-Abu Dhabi}
\journaleditor{Gustavo Alonso}{ETH Zurich}
\journaleditor{Mike Cafarella}{University of Michigan}
\journaleditor{Alan Fekete}{University of Sydney}
\journaleditor{Ihab Ilyas}{University of Waterloo}
\journaleditor{Andy Pavlo}{Carnegie Mellon University}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/DBS-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{DBScolor}{officegreen}   %new color names can be defined before use
\journalcolor      {DBScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Databases}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {DBS}
\journalurl        {http://www.nowpublishers.com/DBS}
\journalissnprint  {1931-7883}
\journalissnonline {1931-7891}
\journaldoi        {10.1561/19}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Databases publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Data Models and Query Languages}
    \item{Query Processing and Optimization}
    \item{Storage, Access Methods, and Indexing}
    \item{Transaction Management, Concurrency Control and Recovery}
    \item{Deductive Databases}
    \item{Parallel and Distributed Database Systems}
    \item{Database Design and Tuning}
    \item{Metadata Management}
    \item{Object Management}
    \item{Trigger Processing and Active Databases}
    \item{Data Mining and OLAP}
    \item{Approximate and Interactive Query Processing}
    \item{Data Warehousing}
    \item{Adaptive Query Processing}
    \item{Data Stream Management}
    \item{Search and Query Integration}
    \item{XML and Semi-Structured Data}
    \item{Web Services and Middleware}
    \item{Data Integration and Exchange}
    \item{Private and Secure Data Management}
    \item{Peer-to-Peer, Sensornet and Mobile Data Management}
    \item{Scientific and Spatial Data Management}
    \item{Data Brokering and Publish/Subscribe}
    \item{Data Cleaning and Information Extraction}
    \item{Probabilistic Data Management}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Databases, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/DBS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Differential Privacy for Databases}\\
Joseph P. Near and Xi He\\
ISBN: 978-1-68083-850-3\\
\\
\noindent \textit{Database Systems on GPUs}\\
Johns Paul, Shengliang Lu and Bingsheng He\\
ISBN: 978-1-68083-848-0\\
\\
\noindent \textit{Machine Knowledge: Creation and Curation of Comprehensive Knowledge Bases}\\
Gerhard Weikum, Xin Luna Dong, Simon Razniewski and Fabian Suchanek\\
ISBN: 978-1-68083-836-7\\
\\
\noindent \textit{Cloud Data Services: Workloads, Architectures and Multi-Tenancy}\\
Vivek Narasayya and Surajit Chaudhuri\\
ISBN: 978-1-68083-774-2\\
\\
\noindent \textit{Data Provenance}\\
Boris Glavic\\
ISBN: 978-1-68083-828-2\\
\\
\noindent \textit{FPGA-Accelerated Analytics: From Single Nodes to Clusters}\\
Zsolt Istv\'an, Kaan Kara and David Sidler\\
ISBN: 978-1-68083-734-6\\
\\
\noindent \textit{Distributed Learning Systems with First-Order Methods}\\
Ji Liu and Ce Zhango\\
ISBN: 978-1-68083-700-1\\

==> journaldata/ECO-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{William H. Greene}{New York University\\United States}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Manuel Arellano}{CEMFI Spain}
\journaleditor{Wiji Arulampalam}{University of Warwick}
\journaleditor{Orley Ashenfelter}{Princeton University}
\journaleditor{Jushan Bai}{Columbia University}
\journaleditor{Badi Baltagi}{Syracuse University}
\journaleditor{Anil Bera}{University of Illinois}
\journaleditor{Tim Bollerslev}{Duke University}
\journaleditor{David Brownstone}{UC Irvine}
\journaleditor{Xiaohong Chen}{Yale University}
\journaleditor{Steven Durlauf}{University of Chicago}
\journaleditor{Amos Golan}{American University}
\journaleditor{Bill Griffiths}{University of Melbourne}
\journaleditor{James Heckman}{University of Chicago}
\journaleditor{Jan Kiviet}{University of Amsterdam}
\journaleditor{Gary Koop}{The University of Strathclyde}
\journaleditor{Michael Lechner}{University of St. Gallen}
\journaleditor{Lung-Fei Lee}{Ohio State University}
\journaleditor{Larry Marsh}{Notre Dame University}
\journaleditor{James MacKinnon}{Queens University}
\journaleditor{Bruce McCullough}{Drexel University}
\journaleditor{Jeff Simonoff}{New York University}
\journaleditor{Joseph Terza}{Purdue University}
\journaleditor{Ken Train}{UC Berkeley}
\journaleditor{Pravin Trivedi}{Indiana University}
\journaleditor{Adonis Yatchew}{University of Toronto}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ECO-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ECOcolor}{brickred}   %new color names can be defined before use
\journalcolor      {ECOcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Econometrics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ECO}
\journalurl        {http://www.nowpublishers.com/ECO}
\journalissnprint  {1551-3076}
\journalissnonline {1551-3084}
\journaldoi        {10.1561/08}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Econometrics publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Econometric Models}
    \item{Simultaneous Equation Models}
    \item{Estimation Frameworks}
    \item{Biased Estimation}
    \item{Computational Problems}
    \item{Microeconometrics}
    \item{Treatment Modeling}
    \item{Discrete Choice Modeling}
    \item{Models for Count Data}
    \item{Duration Models}
   \item{Limited Dependent Variables}
    \item{Panel Data}
    \item{Time Series Analysis}
    \item{Latent Variable Models}
    \item{Qualitative Response Models}
    \item{Hypothesis Testing}
    \item{Econometric Theory}
    \item{Financial Econometrics}
    \item{Measurement Error in Survey Data}
    \item{Productivity Measurement and Analysis}
    \item{Semiparametric and Nonparametric Estimation}
    \item{Bootstrap Methods}
    \item{Nonstationary Time Series}
    \item{Robust Estimation}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Econometrics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ECO-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Climate Econometrics: An Overview}\\
Jennifer L. Castle and David F. Hendry\\
ISBN: 978-1-68083-708-7\\
\\
\noindent \textit{Foundations of Stated Preference Elicitation: Consumer Behavior\\ and Choice-based Conjoint Analysis}\\
Moshe Ben-Akiva, Daniel McFadden and Kenneth Train\\
ISBN: 978-1-68083-526-7\\
\\
\noindent \textit{Structural Econometrics of Auctions: A Review}\\
Matthew L. Gentry, Timothy P. Hubbard, Denis Nekipelov and\\ Harry J. Paarsch\\
ISBN: 978-1-68083-446-8\\
\\
\noindent \textit{Data Visualization and Health Econometrics}\\
Andrew M. Jones\\
ISBN: 978-1-68083-318-8\\


==> journaldata/EDA-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Radu Marculescu}{Carnegie Mellon University}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Robert K. Brayton}{University of California, Berkeley}
\journaleditor{Raul Camposano}{Sage Design Atomation}
\journaleditor{K.T. Tim Cheng}{HKUST}
\journaleditor{Jason Cong}{University of California, Los Angeles}
\journaleditor{Masahiro Fujita}{University of Tokyo}
\journaleditor{Georges Gielen}{KU Leuven}
\journaleditor{Tom Henzinger}{IST Austria}
\journaleditor{Andrew Kahng}{University of California, San Diego}
\columnbreak
\journaleditor{Andreas Kuehlmann}{Synopsys}
\journaleditor{Sharad Malik}{Princeton University}
\journaleditor{Joel Phillips}{Cadence Berkeley Labs}
\journaleditor{Jonathan Rose}{University of Toronto}
\journaleditor{Rob Rutenbar}{University of Pittsburgh}
\journaleditor{Alberto Sangiovanni-Vincentelli}{University of California, Berkeley}
\journaleditor{Leon Stok}{IBM Research}
\end{multicols*}
\end{editorialboard} 

==> journaldata/EDA-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{EDAcolor}{brickred}   %new color names can be defined before use
\journalcolor      {EDAcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electronic Design Automation}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EDA}
\journalurl        {http://www.nowpublishers.com/EDA}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electronic Design Automation publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{System Level Design}
    \item{Behavioral Synthesis}
    \item{Logic Design}
    \item{Verification}
    \item{Test}
    \item{Physical Design}
    \item{Circuit Level Design}
    \item{Reconfigurable Systems}
    \item{Analog Design}
    \item{Embedded software and parallel programming}
   \item{Multicore, GPU, FPGA, and heterogeneous systems}
    \item{Distributed, networked embedded systems}
    \item{Real-time and cyberphysical systems}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Electronic Design Automation, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EDA-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Smart Healthcare}\\
Hongxu Yin, Ayten Ozge Akmandor, Arsalan Mosenia and Niraj K. Jha\\
ISBN: 978-1-68083-440-6\\
\\
\noindent \textit{Contracts for System Design}\\
Albert Benveniste, Benoit Caillaud, Dejan Nickovic, Roberto Passerone, Jean-Baptiste Raclet, Philipp Reinkemeier, Alberto Sangiovanni-Vincentelli, Werner Damm, Thomas A. Henzinger and Kim G. Larsen\\
ISBN: 978-1-68083-402-4\\
\\
\noindent \textit{Non-Boolean Computing with Spintronic Devices}\\
Kawsher A. Roxy and Sanjukta Bhanja\\
ISBN: 978-1-68083-362-1

==> journaldata/EES-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Marija D. Ili\'c}{MIT and Carnegie Mellon University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Hill}{University of Hong Kong and University of Sydney}
\journaleditor{Daniel Kirschen}{University of Washington}
\journaleditor{J. Zico Kolter}{Carnegie Mellon University}
\journaleditor{Chao Lu}{Tsinghua University}
\journaleditor{Steven Low}{California Institute of Technology}
\journaleditor{Ram Rajagopa}{Stanford University}
\journaleditor{Lou van der Sluis}{TU Delft}
\journaleditor{Goran Strbac}{Imperial College London}
\journaleditor{Robert J. Thomas}{Cornell University}
\journaleditor{David Tse}{University of California, Berkeley}
\journaleditor{Le Xie}{Texas A\&M University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/EES-journaldata.tex <==
\definecolor{cinnabar}{rgb}{0.89, 0.26, 0.2}
\colorlet{EEScolor}{cinnabar}   %new color names can be defined before use
\journalcolor      {EEScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electric Energy Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EES}
\journalurl        {http://www.nowpublishers.com/EES}
\journalissnprint  {2332-6557}
\journalissnonline {2332-6565}
\journaldoi        {10.1561/31}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electric Energy Systems publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Advances in power dispatch}
\item{Demand-side and grid scale data analytics}
\item{Design and optimization of electric services}
\item{Distributed control and optimization of distribution networks}
\item{Distributed sensing for the grid}
\item{Distribution systems}
\item{Fault location and service restoration}
\item{Integration of physics-based and data-driven modeling of future electric energy systems}
\item{Integration of Power electronics, Networked FACTS}
\item{Integration of renewable energy sources}
\item{Interdependence of power system operations and planning and the electricity markets}
\item{Microgrids}
\item{Modern grid architecture}
\item{Power system analysis and computing}
\item{Power system dynamics}
\item{Power system operation}
\item{Power system planning}
\item{Power system reliability}
\item{Power system transients}
\item{Security and privacy}
\item{Stability and control for the whole multi-layer (granulated) network with new load models (to include storage, DR, EVs) and new generation}
\item{System protection and control}
\item{The new stability guidelines and control structures for supporting high penetration of renewables (>50\%)}
\item{Uncertainty quantification for the grid}
\item{System impacts of HVDC}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Electric Energy Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EES-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Network-Based Analysis of Rotor Angle Stability of Power Systems}\\
Yue Song, David J. Hill and Tao Liu\\
ISBN: 978-1-68083-778-0\\
\\
\noindent \textit{A Survey of Relaxations and Approximations of the Power Flow Equations}\\
Daniel K. Molzahn and Ian A. Hiskens\\
ISBN: 978-1-68083-540-3\\
\\
\noindent \textit{HELM: The Holomorphic Embedding Load-Flow Method. Foundations and Implementations}\\
Antonio Trias\\
ISBN: 978-1-68083-516-8\\
\\
\noindent \textit{Combinatorial Optimization of Alternating Current Electric Power Systems}\\
Sid Chi-Kin Chau\\
ISBN: 978-1-68083-514-4

==> journaldata/ENT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}
\journalchiefeditor{David B. Audretsch}{Indiana University\\United States}\\
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Howard Aldrich}{University of North Carolina}
\journaleditor{Sharon Alvarez}{University of Denver}
\journaleditor{Per Davidsson}{Queensland University of Technology}
\journaleditor{Michael Frese}{National University of Singapore}
\journaleditor{William B. Gartner}{Copenhagen Business School}
\journaleditor{Magnus Henrekson}{IFN Stockholm}
\journaleditor{Michael A. Hitt}{Texas A\&M University}
\journaleditor{Joshua Lerner}{Harvard University}
\columnbreak
\journaleditor{Jeff McMullen}{Indiana University}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Maria Minniti}{Syracuse University}
\journaleditor{Simon Parker}{University of Western Ontario}
\journaleditor{Holger Patzelt}{TU Munich}
\journaleditor{Saras Sarasvathy}{University of Virginia}
\journaleditor{Roy Thurik}{Erasmus University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ENT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{ENTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {ENTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Entrepreneurship}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ENT}
\journalurl        {http://www.nowpublishers.com/ENT}
\journalissnprint  {1551-3114}
\journalissnonline {1551-3122}
\journaldoi        {10.1561/03}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Entrepreneurship publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Nascent and start-up entrepreneurs}
\item{Opportunity recognition}
\item{New venture creation process}
\item{Business formation}
\item{Firm ownership}
\item{Market value and firm growth}
\item{Franchising}
\item{Managerial characteristics and behavior of entrepreneurs}
\item{Strategic alliances and networks}
\item{Government programs and public policy}
\item{Gender and ethnicity}
\columnbreak
\item{New business financing:}
	\begin{itemize}
\item{Business angels}
\item{Bank financing, debt, and trade credit}
\item{Venture capital and private equity capital}
\item{Public equity and IPOs} 
\end{itemize}
\item{Family-owned firms}
\item{Management structure, governance and performance}
\item{Corporate entrepreneurship}
\item{High technology:}
	\begin{itemize}
        \item{Technology-based new firms}
        \item{High-tech clusters}
        \end{itemize}
\item{Small business and economic growth}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Entrepreneurship, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ENT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Ambidexterity and Entrepreneurship Studies: A Literature Review and Research Agenda}\\
Maribel Guerrero\\
ISBN: 978-1-68083-818-3\\
\\
\noindent \textit{Innovative Entrepreneurship as a Collaborative Effort: An Institutional Framework}\\
Niklas Elert and Magnus Henrekson\\
ISBN: 978-1-68083-810-7\\
\\
\noindent \textit{Entrepreneurial Finance: Emerging Approaches Using Machine Learning and Big Data}\\
Francesco Ferrati and Moreno Muffatto\\
ISBN: 978-1-68083-804-6\\
\\
\noindent \textit{Advice to Entrepreneurs and Small Business}\\
Kevin Mole\\
ISBN: 978-1-68083-758-2
\\
\noindent \textit{From Ethnic Enclaves to Transnational Landscapes: A Review of Immigrant Entrepreneurship Research}\\
Anuradha Basu and Sarika Pruthi\\
ISBN: 978-1-68083-756-8


==> journaldata/FIN-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Sheridan Titman}{University of Texas at Austin\\United States}
\end{multicols}

\subsection{Associate Editors}
\begin{multicols}{1}
\journaleditor{Josef Zechner}{WU Vienna University of Economics and Finance}
\journaleditor{Chester Spatt}{Carnegie Mellon University}
\end{multicols}
\end{editorialboard} 

==> journaldata/FIN-journaldata.tex <==
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\colorlet{FINcolor}{ceruleanblue}   %new color names can be defined before use
\journalcolor      {FINcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Finance}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {FIN}
\journalurl        {http://www.nowpublishers.com/FIN}
\journalissnprint  {1567-2395}
\journalissnonline {1567-2409}
\journaldoi        {10.1561/05}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Finance publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Corporate Finance}
\begin{itemize}
\item{Corporate Governance}
\item{Corporate Financing}
\item{Dividend Policy and Capital Structure}
\item{Corporate Control}
\item{Investment Policy}
\item{Agency Theory and Information}
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Financial Markets}
\begin{itemize}
\item{Market Microstructure}
\item{Portfolio Theory}
\item{Financial Intermediation}
\item{Investment Banking}
\item{Market Efficiency}
\item{Security Issuance}
\item{Anomalies and Behavioral Finance}
\end{itemize}
\end{itemize}
\end{multicols}
%}
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
%\columnbreak
%\begin{itemize}
\item{Asset Pricing}
\begin{itemize}
\item{Asset-Pricing Theory}
\item{Asset-Pricing Models}
\item{Tax Effects}
\item{Liquidity} 
\item{Equity Risk Premium} 
\item{Pricing Models and Volatility} 
\item{Fixed Income Securities} 
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Derivatives}
\begin{itemize}
\item{Computational Finance}
\item{Futures Markets and Hedging}
\item{Financial Engineering}
\item{Interest Rate Derivatives}
\item{Credit Derivatives}
\item{Financial Econometrics}
\item{Estimating Volatilities and Correlations}
\end{itemize}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Finance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/FIN-seriespage.tex <==
\vspace{12pt}

\noindent \textit{The Implications of Heterogeneity and Inequality for Asset Pricing}\\
Stavros Panageas\\
ISBN: 978-1-68083-750-6\\
\\
\noindent \textit{Risk Sharing Within the Firm: A Primer}\\
Marco Pagano\\
ISBN: 978-1-68083-740-7\\
\\
\noindent \textit{The Economics of Credit Rating Agencies}\\
Francesco Sangiorgi and Chester Spatt\\
ISBN: 978-1-68083-380-5\\
\\
\noindent \textit{Initial Public Offerings: A Synthesis of the Literature and Directions for Future Research}\\
Michelle Lowry, Roni Michaely and Ekaterina Volkova\\
ISBN: 978-1-68083-340-9\\
\\
\noindent \textit{Privatization, State Capitalism, and State Ownership of Business in the 21st Century}\\
William L. Megginson\\
ISBN: 978-1-68083-338-6\\

==> journaldata/HCI-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Youn-Kyung Lim}{Korea Advanced Institute of Science and Technology}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Ben Bederson}{University of Maryland}
\journaleditor{Madeline Balaam}{KTH Royal Institute of Technology}
\journaleditor{Eun Kyoung Choe}{University of Maryland, College Park}
\journaleditor{Andy Cockburn}{University of Canterbury}
\journaleditor{Karrie Karahalios}{University of Illinois at Urbana-Champaign}
\journaleditor{Rohit Ashok Khot}{HAFP Research Lab, RMIT University}
\journaleditor{Uichin Lee}{Korea Advanced Institute of Science and Technology}
\journaleditor{Florian Mueller}{Exertion Games Lab, RMIT University}
\journaleditor{Bilge Mutlu}{University of Wisconsin-Madison}
\journaleditor{Marianna Obrist}{University of Sussex}
\journaleditor{Nuria Oliver}{Telefonica}
\journaleditor{Sameer Patil}{University of Utah}
\journaleditor{Orit Shaer}{Wellesley College}
\journaleditor{Desney S. Tan}{Microsoft Research}
\journaleditor{Koji Yatani}{University of Tokyo}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/HCI-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{HCIcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {HCIcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Human-Computer Interaction}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {HCI}
\journalurl        {http://www.nowpublishers.com/HCI}
\journalissnprint  {1551-3955}
\journalissnonline {1551-3963}
\journaldoi        {10.1561/11}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Human-Computer Interaction publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{History of the research community}
\item{Theory}
\item{Technology}
\item{Computer Supported Cooperative Work}
\item{Interdisciplinary influence}
\item{Advanced topics and trends}
\end{itemize}
%\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Human-Computer Interaction, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/HCI-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Improving HCI with Brain Input: Review, Trends, and Outlook}\\
Erin T. Solovey and Felix Putzer\\
ISBN: 978-1-68083-814-5\\
\\
\noindent \textit{Patient-Generated Health Data: Dimensions, Challenges, and Open Questions}\\
Mayara Costa Figueiredo and Yunan Cheng\\
ISBN: 978-1-68083-668-4\\
\\
\noindent \textit{Patterns and Themes in Designing with Children}\\
Jessica Korte\\
ISBN: 978-1-68083-660-8\\
\\
\noindent \textit{Gender-Inclusive HCI Research and Design: A Conceptual Review}\\
Simone Stumpf, Anicia Peters, Shaowen Bardzell, Margaret Burnett, Daniela Busse, Jessica Cauchard, Elizabeth Churchill\\
ISBN: 978-1-68083-656-1\\


==> journaldata/ICS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Georges Gielen}{KU Leuven, Belgium}
%\end{multicols*}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alison Burdett}{Sensium Healthcare, UK}
\journaleditor{Malgorzata Chrzanowska-Jeske}{Portland State University, USA}
\journaleditor{Paulo Diniz}{UFRJ, Brazil}
\journaleditor{Peter Kennedy}{University College Dublin, Ireland}
\journaleditor{Maciej Ogorzalek}{Jagiellonian University, Poland}
\journaleditor{Jan van der Spiegel}{University of Pennsylvania, USA}
\journaleditor{Ljiljana Trajkovic}{Simon Fraser University, USA}
%\end{multicols*}

\end{editorialboard} 

==> journaldata/ICS-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ICScolor}{brickred}   %new color names can be defined before use
\journalcolor      {ICScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Integrated Circuits and Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ICS}
\journalurl        {http://www.nowpublishers.com/ICS}
\journalissnprint  {2693-9347}
\journalissnonline {2693-9355}
\journaldoi        {10.1561/35}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
 Integrated Circuits and Systems
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Analog, digital and mixed-signal circuits and systems}
\item{RF and mm-wave integrated circuits and systems}
\item{Wireless and wireline communication circuits and systems}
\item{Data converters and frequency generation}
\item{Power electronics and power management circuits}
\item{Biomedical circuits and systems}
\item{Sensor and imager circuits and cyber physical systems}
\item{Security and resilient circuits and systems}
\item{Circuits and systems in emerging non-CMOS technologies}
\item{Circuit theory, modeling, analysis and design methods}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Integrated Circuits and Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ICS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Welcome to the World of Single-Slope Column-Level Analog-to-Digital Converters for CMOS Image Sensors}\\
Albert Theuwissen and Guy Meynants\\
ISBN: 978-1-68083-812-1\\





==> journaldata/INR-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Maarten de Rijke}{University of Amsterdam \\ and Ahold Delhaize\\The Netherlands}
\journalchiefeditor{Yiqun Liu}{Tsinghua University\\China}
\journalchiefeditor{Diane Kelly}{University of Tennessee\\USA}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Barbara Poblete}{University of Chile}
\journaleditor{Claudia Hauff}{Delft University of Technology}
\journaleditor{Doug Oard}{University of Maryland}
\journaleditor{Ellen M. Voorhees}{National Institute of Standards and Technology}
\journaleditor{Fabrizio Sebastiani}{Consiglio Nazionale delle Ricerche, Italy}
\journaleditor{Hang Li}{Bytedance Technology}
\journaleditor{Isabelle Moulinier}{Capital One}
\journaleditor{Jaap Kamps}{University of Amsterdam}
\journaleditor{Jimmy Lin}{University of Waterloo}
\journaleditor{Leif Azzopardi}{University of Glasgow}
\columnbreak
\journaleditor{Lynda Tamine}{University of Toulouse}
\journaleditor{Mark Sanderson}{RMIT University}
\journaleditor{Rodrygo Luis Teodoro Santos}{Universidade Federal de Minas Gerais}
\journaleditor{Ruihua Song}{Renmin University of China}
\journaleditor{Ryen White}{Microsoft Research}
\journaleditor{Shane Culpepper}{RMIT}
\journaleditor{Soumen Chakrabarti}{Indian Institute of Technology}
\journaleditor{Xuanjing Huang}{Fudan University}
\journaleditor{Zi Helen Huang}{University of Queensland}
\end{multicols*}
\end{editorialboard} 

==> journaldata/INR-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{INRcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {INRcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Retrieval}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {INR}
\journalurl        {http://www.nowpublishers.com/INR}
\journalissnprint  {1554-0669}
\journalissnonline {1554-0677}
\journaldoi        {10.1561/15}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Retrieval publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Applications of IR}
\item{Architectures for IR}
\item{Collaborative filtering and recommender systems}
\item{Cross-lingual and multilingual IR}
\item{Distributed IR and federated search}
\item{Evaluation issues and test collections for IR}
\item{Formal models and language models for IR}
\item{IR on mobile platforms}
\item{Indexing and retrieval of structured documents}
\item{Information categorization and clustering}
\item{Information extraction}
\item{Information filtering and routing}
\item{Metasearch, rank aggregation and data fusion}
\item{Natural language processing for IR}
\item{Performance issues for IR systems, including algorithms, data structures, optimization techniques, and scalability}
\item{Question answering}
\item{Summarization of single documents, multiple documents, and corpora}
\item{Text mining}
\item{Topic detection and tracking}
\item{Usability, interactivity, and visualization issues in IR}
\item{User modelling and user studies for IR}
\item{Web search}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Retrieval, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 5 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/INR-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Search and Discovery in Personal Email Collections}\\
Michael Bendersky, Xuanhui Wang, Marc Najork and Donald Metzler\\
ISBN: 978-1-68083-838-1\\

\noindent \textit{Extracting, Mining and Predicting Users’ Interests from Social Media}\\
Fattane Zarrinkalam, Stefano Faralli, Guangyuan Piao and Ebrahim Bagheri\\
ISBN: 978-1-68083-738-4\\

\noindent \textit{Knowledge Graphs: An Information Retrieval Perspective}\\
Ridho Reinanda, Edgar Meij and Maarten de Rijke\\
ISBN: 978-1-68083-728-5\\

\noindent \textit{Deep Learning for Matching in Search and Recommendation}\\
Jun Xu, Xiangnan He and Hang Li \\
ISBN: 978-1-68083-706-3\\

\noindent \textit{Explainable Recommendation: A Survey and New Perspectives}\\
Yongfeng Zhang and Xu Chen\\
ISBN: 978-1-68083-658-5\\



==> journaldata/ISY-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{David Paradice}{Auburn University\\United States}
%\end{multicols}

\subsection{Honorary Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Izak Benbasat}{University of British Columbia}
\journaleditor{Alan R. Dennis}{Kelley School of Business, Indiana University}
\journaleditor{Jacqueline Rees Ulmer}{Iowa State University}
\journaleditor{Veda Storey}{Georgia State University}
\journaleditor{Detmar Straub}{Georgia State University}
\journaleditor{Hugh Watson}{University of Georgia}
%\end{multicols*}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Joey George}{Iowa State University}
\journaleditor{Alan Hevner}{University of South Florida}
\journaleditor{Carol Saunders}{University of Central Florida}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ISY-journaldata.tex <==
\definecolor{regalia}{rgb}{0.32, 0.18, 0.5}
\colorlet{ISYcolor}{regalia}   %new color names can be defined before use
\journalcolor      {ISYcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ISY}
\journalurl        {http://www.nowpublishers.com/ISY}
\journalissnprint  {2331-1231}
\journalissnonline {2331-124X}
\journaldoi        {10.1561/29}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Systems publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{IS and Individuals}
\item{IS and Groups}
\item{IS and Organizations}
\item{IS and Industries}
\item{IS and Society}
\item{IS Development}
\item{IS Economics}
\item{IS Management}
\item{IS Research Methods}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ISY-seriespage.tex <==
\vspace{12pt}
\noindent \textit{IT Project Management: Lessons Learned from Project Retrospectives 1999–2020}\\
R. Ryan Nelson\\
ISBN: 978-1-68083-776-6\\
\\
\noindent \textit{Speech Analytics for Actionable Insights: Current Status, Recommendation, and Guidance}\\
J. P. Shim, Aaron M. French and Bikesh Upreti\\
ISBN: 978-1-68083-696-7\\
\\
\noindent \textit{A Review of Personality in Human–Robot Interactions}\\
Lionel P. Robert Jr., Rasha Alahmad, Connor Esterwood, Sangmi Kim, Sangseok You and Qiaoning Zhang\\
ISBN: 978-1-68083-662-2\\
\\
\noindent \textit{Information Technology and Entrepreneurship: Factors that Shape Investment Support for Innovation}\\
Veda C. Storey and Linda Wallace\\
ISBN: 978-1-68083-602-8


==> journaldata/MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Tensor Regression}\\
Jiani Liu, Ce Zhu, Zhen Long and Yipeng Liu\\
ISBN: 978-1-68083-886-2\\
\\
\noindent \textit{Minimum-Distortion Embedding}\\
Akshay Agrawal, Alnur Ali and Stephen Boyd\\
ISBN: 978-1-68083-888-6\\
\\
\noindent \textit{Graph Kernels: State-of-the-Art and Future Challenges}\\
Karsten Borgwardt, Elisabetta Ghisu, Felipe Llinares-López, Leslie O’Bray and Bastian Rieck\\
ISBN: 978-1-68083-770-4\\
\\
\noindent \textit{Data Analytics on Graphs Part III: Machine Learning on Graphs, from Graph Topology to Applications}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-16\\
\\
\noindent \textit{Data Analytics on Graphs Part II: Signals on Graphso}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\
\\
\noindent \textit{Data Analytics on Graphs Part I: Graphs and Spectra on Graphs}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\

==> journaldata/MGT-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{2}\raggedright
\journalchiefeditor{Nicholas S. Argyres}{Olin Business School, Washington University\\United States}
\journalchiefeditor{Timothy M. Devinney}{Leeds University Business School\\United Kingdom}
\journalchiefeditor{James Campbell Quick}{The University of Texas at Arlington\\United States}
\end{multicols}

\subsection{Editors}
\begin{multicols}{3}\raggedright \raggedcolumns
\renewcommand\journaleditor[2]{\par\textbf{#1}\\#2}%
\subsubsection{\footnotesize International Business}

\journaleditor{Gabriel R.G. Benito}{BI Norwegian School of Management}
\journaleditor{Allan Bird}{Northeastern University}
\journaleditor{Julian Birkinshaw}{London Business School}
\journaleditor{Peter Buckley}{University of Leeds}
\journaleditor{Saul Estrin}{London School of Economics}
\journaleditor{Sarianna Lundin}{University of Bremen}
\journaleditor{Xavier Martin}{Tilburg University} 
\journaleditor{Ram Mudambi}{Temple University}

\columnbreak

\subsubsection{\footnotesize Organizational Behavior}

\journaleditor{Myrtle Bell}{University of Texas at Arlington}
\journaleditor{Cary Cooper}{Lancaster University}
\journaleditor{Richard Griffin}{Texas A\&M University}
\journaleditor{Sean Hannah}{Wake Forest University}
\journaleditor{Debra Nelson}{Oklahoma State University}
\journaleditor{Pamela Perrewe}{Florida State University}

\columnbreak

\subsubsection{\footnotesize Strategy}

\journaleditor{Rajshree Agarwal}{University of Maryland}
\journaleditor{Marvin Lieberman}{UCLA}) 
\journaleditor{Michael Lenox}{University of Virginia}
\journaleditor{Joseph Mahoney}{University of Illinois at Urbana-Champaign}
\journaleditor{Jesper Sørensen}{Stanford University}
\journaleditor{Olav Sorenson}{Yale University}
\end{multicols}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MGT-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{MGTcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {MGTcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MGT}
\journalurl        {http://www.nowpublishers.com/MGT}
\journalissnprint  {2475-6946}
\journalissnonline {2475-6954}
\journaldoi        {10.1561/34}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management publishes
 survey and tutorial articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{International Business}
\item{Organizational Behavior}
\item{Strategic Management}
\end{itemize}
 %\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-editorialboard.tex <==
%MIC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{W. Kip Viscusi}{Vanderbilt University Law School\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Richard Carson}{University of California, San Diego}
\journaleditor{William Gentry}{Williams College}
\journaleditor{Tom Kniesner}{Syracuse University}
\journaleditor{Mark V. Pauly}{University of Pennsylvania}
\journaleditor{Yossi Spiegel}{Tel Aviv University}
\journaleditor{William Zame}{University of California, Los Angeles}
\journaleditor{James Ziliak}{University of Kentucky}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MIC-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{MICcolor}{pinegreen}   %new color names can be defined before use   %new color names can be defined before use
\journalcolor      {MICcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Microeconomics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MIC}
\journalurl        {http://www.nowpublishers.com/MIC}
\journalissnprint  {1547-9846}
\journalissnonline {1547-9854}
\journaldoi        {10.1561/07}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Environmental economics}
\item{Health economics}
\item{Industrial organization}
\item{Labor economics}
\item{Law and economics}
\item{Public economics}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-seriespage.tex <==
\vspace{12pt}
\vspace{12pt}
\noindent \textit{Behavioral Economics of Multiperiod Insurance Purchasing Behavior: The Role of Emotions}\\
Howard Kunreuther and Mark Pauly
\\ISBN: 978-1-68083-524-3
\\
\\
\noindent \textit{Trade and Climate Change: Focus on Carbon Leakage, Border Carbon Adjustments and WTO Consistency}\\
ZhongXiang Zhang
\\ISBN: 978-1-68083-482-6
\\
\\
\noindent \textit{Natural Gas Pipeline Regulation in the United States: Past, Present, and Future}\\
Matthew E. Oliver
\\ISBN: 978-1-68083-452-9
\\
\\
\noindent \textit{The U.S. Market for Uranium: 70 Years of History}\\
Charles F. Mason
\\ISBN: 978-1-68083-382-9
\\
\\
\noindent \textit{Game Theory and Water Resources: Critical Review of its Contributions, Progress and Remaining Challenges}\\
Ariel Dinar and Margaret Hogarth
\\ISBN: 978-1-68083-016-3


==> journaldata/MKT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Jehoshua Eliashberg}{University of Pennsylvania}

\subsection{Associate Editor}

\journaleditor{Bernd Schmitt}{Columbia University}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dawn Iacobucci}{Vanderbilt University}
\journaleditor{Ganesh Iyeri}{University of California, Berkeley}
\journaleditor{Anirban Mukhopadhyayi}{HKUST}
\journaleditor{Sharon Ngi}{Nanyang Technological University}
\journaleditor{Gerrit van Bruggeni}{Erasmus University}
\journaleditor{Miguel Villas Boasi}{University of California, Berkeley}
\journaleditor{Hema Yoganarasimhani}{University of Washington}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MKT-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MKTcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MKTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Marketing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MKT}
\journalurl        {http://www.nowpublishers.com/MKT}
\journalissnprint  {1555-0753}
\journalissnonline {1555-0761}
\journaldoi        {10.1561/17}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Marketing publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{B2B Marketing}
\item{Bayesian Models}
\item{Behavioral Decision Making}
\item{Branding and Brand Equity}
\item{Channel Management}
\item{Choice Modeling}
\item{Comparative Market Structure}
\item{Competitive Marketing Strategy}
\item{Conjoint Analysis}
\item{Customer Equity}
\item{Customer Relationship Management}
\item{Game Theoretic Models}
\item{Group Choice and Negotiation}
\item{Discrete Choice Models}
\item{Individual Decision Making}
\item{Marketing Decisions Models}
\item{Market Forecasting}
\item{Marketing Information Systems}
\item{Market Response Models}
\item{Market Segmentation}
\item{Market Share Analysis}
\item{Multi-channel Marketing}
\item{New Product Diffusion}
\item{Pricing Models}
\item{Product Development}
\item{Product Innovation}
\item{Sales Forecasting}
\item{Sales Force Management}
\item{Sales Promotion}
\item{Services Marketing}
\item{Stochastic Model}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Marketing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MKT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Brands: An Integrated Marketing, Finance, and Societal Perspective}\\
Bobby J. Calder\\
ISBN: 978-1-68083-746-9\\
\\
\noindent \textit{Machine Learning in Marketing: Overview, Learning Strategies, Applications, and Future Developments}\\
Vinicius Andrade Brei\\
ISBN: 978-1-68083-720-9\\
\\
\noindent \textit{Crowdfunding Platforms: Ecosystem and Evolution}\\
Yee Heng Tan and Srinivas K. Reddy\\
ISBN: 978-1-68083-698-1\\
\\
\noindent \textit{A Practical Approach to Sales Compensation: What Do We Know Now? What Should We Know in the Future?}\\
Doug J. Chung, Byungyeon Kim and Niladri B. Syam\\
ISBN: 978-1-68083-684-4\\


==> journaldata/NET-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Anthony Ephremides}{University of Maryland\\United States}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fran\c{c}ois Baccelli}{University of Texas, Austin}
\journaleditor{Victor Bahl}{Microsoft Research}
\journaleditor{Helmut B\"{o}lcskei}{ETH Zurich}
\journaleditor{J.J. Garcia-Luna Aceves}{UC Santa Cruz}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Roch Guerin}{Washington University in Saint Louis}
\journaleditor{Bruce Hajek}{UIUC}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Frank Kelly}{University of Cambridge}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Steven Low}{Caltech}
\journaleditor{Eytan Modiano}{MIT}
\columnbreak
\journaleditor{Keith Ross}{Polytechnic Institute of NYU}
\journaleditor{Henning Schulzrinne}{Columbia University}
\journaleditor{Mani Srivastava}{UCLA}
\journaleditor{Leandros Tassiulas}{Yale University}
\journaleditor{Lang Tong}{Cornell University}
\journaleditor{Ozan Tonguz}{Carnegie Mellon University}
\journaleditor{Don Towsley}{University of Massachusetts, Amherst}
\journaleditor{Nitin Vaidya}{UIUC}
\journaleditor{Pravin Varaiya}{UC Berkeley}
\journaleditor{Roy Yates}{Rutgers University}
\journaleditor{Raymond Yeung}{Chinese University of Hong Kong}
\end{multicols*}
\end{editorialboard} 

==> journaldata/NET-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{NETcolor}{cerise}   %new color names can be defined before use
\journalcolor      {NETcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Networking}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {NET}
\journalurl        {http://www.nowpublishers.com/NET}
\journalissnprint  {1554-057X}
\journalissnonline {1554-0588}
\journaldoi        {10.1561/13}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Networking publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Modeling and Analysis of:}
	\begin{itemize}
	\item{Ad Hoc Wireless Networks}
	\item{Sensor Networks}
	\item{Optical Networks}
	\item{Local Area Networks}
	\item{Satellite and Hybrid Networks}
	\item{Cellular Networks}
	\item{Internet and Web Services}
	\end{itemize}
\item{Protocols and Cross-Layer Design}
\item{Network Coding}
\item{Energy-Efficiency Incentives/Pricing/Utility-based}
\item{Games (co-operative or not)}
\item{Security}
\item{Scalability}
\item{Topology}
\item{Control/Graph-theoretic models}
\item{Dynamics and Asymptotic Behavior of Networks}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Networking, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/NET-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Age of Information: A New Concept, Metric, and Tool}\\
Antzela Kosta, Nikolaos Pappas and Vangelis Angelakis\\
ISBN: 978-1-68083-360-7\\
\\
\noindent \textit{Network and Protocol Architectures for Future Satellite Systems}\\
Tomaso de Cola, Alberto Ginesi, Giovanni Giambene,\\ George C. Polyzos, Vasilios A. Siris, Nikos Fotiou and Yiannis Thomas\\
ISBN: 978-1-68083-334-8\\
\\
\noindent \textit{Duality of the Max-Plus and Min-Plus Network Calculus}\\
Jorg Liebeherr\\
ISBN: 978-1-68083-294-5\\
\\
\noindent \textit{Opportunistic Routing in Wireless Networks}\\
Tara Javidi and Eric Van Buhler\\
ISBN: 978-1-68083-150-4

==> journaldata/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> journaldata/OPT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Garud Iyengar}{Columbia University, USA}
%\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dimitris Bertsimas}{Massachusetts Institute of Technology}
\journaleditor{John R. Birge}{The University of Chicago}
\journaleditor{Robert E. Bixby}{Rice University}
\journaleditor{Emmanuel Candes}{Stanford University}
\journaleditor{David Donoho}{Stanford University}
\journaleditor{Laurent El Ghaoui}{University of California, Berkeley}
\journaleditor{Donald Goldfarb}{Columbia University}
\journaleditor{Michael I. Jordan}{University of California, Berkeley}
\journaleditor{Zhi-Quan (Tom) Luo}{University of Minnesota, Twin Cites}
\journaleditor{George L. Nemhauser}{Georgia Institute of Technology}
\journaleditor{Arkadi Nemirovski}{Georgia Institute of Technology}
\columnbreak
\journaleditor{Yurii Nesterov}{HSE University}
\journaleditor{Jorge Nocedal}{Northwestern University}
\journaleditor{Pablo A. Parrilo}{Massachusetts Institute of Technology}
\journaleditor{Boris T. Polyak}{Institute for Control Science, Moscow}
\journaleditor{Tam\'as Terlaky}{Lehigh University}
\journaleditor{Michael J. Todd}{Cornell University}
\journaleditor{Kim-Chuan Toh}{National University of Singapore}
\journaleditor{John N. Tsitsiklis}{Massachusetts Institute of Technology}
\journaleditor{Lieven Vandenberghe}{University of California, Los Angeles}
\journaleditor{Robert J. Vanderbei}{Princeton University}
\journaleditor{Stephen J. Wright}{University of Wisconsin}
\end{multicols*}
\end{editorialboard} 

==> journaldata/OPT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{OPTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {OPTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Optimization}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {OPT}
\journalurl        {http://www.nowpublishers.com/OPT}
\journalissnprint  {2167-3888}
\journalissnonline {2167-3918}
\journaldoi        {10.1561/24}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Optimization publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{algorithm design, analysis, and implementation (especially, on modern computing platforms}
\item{models and modeling systems, new optimization formulations for practical problems}
\item{applications of optimization in machine learning, statistics, and data analysis, signal and image processing, computational economics and finance, engineering design, scheduling and resource allocation, and other areas}
\end{itemize}
 %\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Optimization, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/OPT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Atomic Decomposition via Polar Alignment: The Geometry of Structured Optimization}\\
Zhenan Fan, Halyun Jeong, Yifan Sun and Michael P. Friedlander\\
ISBN: 978-1-68083-742-1\\
\\
\noindent \textit{Optimization Methods for Financial Index Tracking: From Theory to Practice}\\
Konstantinos Benidis, Yiyong Feng and Daniel P. Palomar\\
ISBN: 978-1-68083-464-2\\
\\
\noindent \textit{The Many Faces of Degeneracy in Conic Optimization}\\
Dmitriy Drusvyatskiy and Henry Wolkowicz\\
ISBN: 978-1-68083-390-4\\

==> journaldata/PGL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Rupak Majumdari}{Max Planck Institute for Software Systems}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and UC Santa Cruz}
\journaleditor{Anindya Banerjee}{IMDEA Software Instituet}
\journaleditor{Patrick Cousot}{ENS, Paris and NYU}
\journaleditor{Oege De Moor}{University of Oxford}
\journaleditor{Matthias Felleisen}{Northeastern University}
\journaleditor{John Field}{Google}
\journaleditor{Cormac Flanagan}{UC Santa Cruz}
\journaleditor{Philippa Gardner}{Imperial College}
\journaleditor{Andrew Gordon}{Microsoft Research and University of Edinburgh}
\journaleditor{Dan Grossman}{University of Washington}
\journaleditor{Robert Harper}{CMU}
\journaleditor{Tim Harris}{Amazon}
\journaleditor{Fritz Henglein}{University of Copenhagen}
\journaleditor{Rupak Majumdar}{MPI and UCLA}
\journaleditor{Kenneth McMillan}{Microsoft Research}
\journaleditor{J. Eliot B. Moss}{University of Massachusetts, Amherst}
\journaleditor{Andrew C. Myers}{Cornell University}
\journaleditor{Hanne Riis Nielson}{Technical University of Denmark}
\journaleditor{Peter O'Hearni}{University College London}
\journaleditor{Benjamin C. Pierce}{University of Pennsylvania}
\journaleditor{Andrew Pittsi}{University of Cambridge}
\journaleditor{Ganesan Ramalingami}{Microsoft Research}
\journaleditor{Mooly Sagiv}{Tel Aviv University}
\journaleditor{Davide Sangiorgi}{University of Bologna}
\journaleditor{David Schmidt}{Kansas State University}
\journaleditor{Peter Sewell}{University of Cambridge}
\journaleditor{Scott Stoller}{Stony Brook University}
\journaleditor{Peter Stuckey}{University of Melbourne}
\journaleditor{Jan Vitek}{Northeastern University}
\journaleditor{Philip Wadler}{University of Edinburgh}
\journaleditor{David Walker}{Princeton University}
\journaleditor{Stephanie Weiric}{University of Pennsylvania}
\end{multicols*}
\end{editorialboard} 

==> journaldata/PGL-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{PGLcolor}{brickred}   %new color names can be defined before use
\journalcolor      {PGLcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Programming Languages}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {PGL}
\journalurl        {http://www.nowpublishers.com/PGL}
\journalissnprint  {2325-1107}
\journalissnonline {2325-1131}
\journaldoi        {10.1561/25}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Programming Languages publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Abstract Interpretation}
\item{Compilation and Interpretation Techniques}
\item{Domain Specific Languages}
\item{Formal Semantics, including Lambda Calculi, Process Calculi, and Process Algebra}
\item{Language Paradigms}
    \item{Mechanical Proof Checking}
    \item{Memory Management}
    \item{Partial Evaluation}
    \item{Program Logic}
    \item{Programming Language Implementation}
    \item{Programming Language Security}
    \item{Programming Languages for Concurrency}
    \item{Programming Languages for Parallelism}
    \item{Program Synthesis}
    \item{Program Transformations and Optimizations}
    \item{Program Verification}
    \item{Runtime Techniques for Programming Languages}
    \item{Software Model Checking}
    \item{Static and Dynamic Program Analysis}
    \item{Type Theory and Type Systems}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Programming Languages, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/PGL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Shape Analysis}\\
Bor-Yuh Evan Chang, Cezara Drăgoi, Roman Manevich, Noam Rinetzky and Xavier Rival\\
ISBN: 978-1-68083-732-2\\
\\
\noindent \textit{Progress of Concurrent Objects}\\
Hongjin Liang and Xinyu Feng\\
ISBN: 978-1-68083-672-1\\
\\
\noindent \textit{QED at Large: A Survey of Engineering of Formally Verified \\Software}\\
Talia Ringer, Karl Palmskog, Ilya Sergey, Milos Gligoric and \\Zachary Tatlock\\
ISBN: 978-1-68083-594-6\\
\\
\noindent \textit{Reconciling Abstraction with High Performance: A MetaOCaml \\approach}\\
Oleg Kiselyov\\
ISBN: 978-1-68083-436-9

==> journaldata/ROB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}
\journalchiefeditor{Julie Shah}{Massachusetts Institute of Technology}

\subsection{Honorary Editors}
\journaleditor{Henrik Christensen}{University of California, San Diego}
\journaleditor{Roland Siegwart}{ETH Zurich}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Minoru Asada}{Osaka University}
\journaleditor{Antonio Bicchi}{University of Pisa}
\journaleditor{Aude Billard}{EPFL}
\journaleditor{Cynthia Breazeal}{Massachusetts Institute of Technology}
\journaleditor{Oliver Brock}{TU Berlin}
\journaleditor{Wolfram Burgard}{University of Freiburg}
\journaleditor{Udo Frese}{University of Bremen}
\journaleditor{Ken Goldberg}{University of California, Berkeley}
\journaleditor{Hiroshi Ishiguro}{Osaka University}
\journaleditor{Makoto Kaneko}{Osaka University}
\journaleditor{Danica Kragic}{KTH Stockholm}
\journaleditor{Vijay Kumar}{University of Pennsylvania}
\journaleditor{Simon Lacroix}{LAAS}
\journaleditor{Christian Laugier}{INRIA}
\journaleditor{Steve LaValle}{University of Illinois at Urbana-Champaign}
\journaleditor{Yoshihiko Nakamura}{The University of Tokyo}
\journaleditor{Brad Nelson}{ETH Zurich}
\journaleditor{Paul Newman}{University of Oxford}
\journaleditor{Daniela Rus}{Massachusetts Institute of Technology}
\journaleditor{Giulio Sandini}{University of Genova}
\journaleditor{Sebastian Thrun}{Stanford University}
\journaleditor{Manuela Veloso}{Carnegie Mellon University}
\journaleditor{Markus Vincze}{Vienna University}
\journaleditor{Alex Zelinsky}{DSTG}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ROB-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{ROBcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {ROBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Robotics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ROB}
\journalurl        {http://www.nowpublishers.com/ROB}
\journalissnprint  {1935-8253}
\journalissnonline {1935-8261}
\journaldoi        {10.1561/23}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Robotics publishes
 survey and tutorial articles in the following topics:
\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Mathematical modelling}
\item{Kinematics}
\item{Dynamics}
\item{Estimation Methods}
\item{Robot Control}
\item{Planning}
\item{Artificial Intelligence in Robotics}
\item{Software Systems and Architectures}
\item{Mechanisms and Actuators}
\item{Sensors and Estimation}
\item{Planning and Control}
\item{Human-Robot Interaction}
\item{Industrial Robotics}
\item{Service Robotics }
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Robotics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ROB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{A Roadmap for US Robotics – From Internet to Robotics 2020 Edition}\\
Henrik Christensen, Nancy Amato, Holly Yanco, Maja Mataric, Howie Choset, Ann Drobnis, Ken Goldberg, Jessy Grizzle, Gregory Hager, John Hollerbach, Seth Hutchinson, Venkat Krovi, Daniel Lee, Bill Smart, Jeff Trinkle and Gaurav Sukhatme\\
ISBN: 978-1-68083-858-9\\
\\
\noindent \textit{The State of Industrial Robotics: Emerging Technologies, Challenges, and Key Research Directions}\\
Lindsay Sanneman, Christopher Fourie and Julie A. Shah\\
ISBN: 978-1-68083-800-8\\
\\
\noindent \textit{Semantics for Robotic Mapping, Perception and Interaction: A Survey}\\
Sourav Garg, Niko Sünderhauf, Feras Dayoub, Douglas Morrison, Akansel Cosgun, Gustavo Carneiro, Qi Wu, Tat-Jun Chin, Ian Reid, Stephen Gould, Peter Corke and Michael Milford\\
ISBN: 978-1-68083-768-1\\


==> journaldata/SEC-editorialboard.tex <==
%SEC-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Anupam Datta}{Carnegie Mellon University, USA}
\journalchiefeditor{Jeannette Wing}{Columbia University, USA}


\subsection{Editors}
\begin{multicols}{2}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and University of California, Santa Cruz}
\journaleditor{Michael Backes}{Saarland University}
\journaleditor{Dan Boneh}{Stanford University, USA}
\journaleditor{V\'eronique Cortier}{LORIA, CNRS, France}
\journaleditor{Lorrie Cranor}{Carnegie Mellon University}
\journaleditor{C\'edric Fournet}{Microsoft Research}
\journaleditor{Virgil Gligor}{Carnegie Mellon University}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Deirdre Mulligan}{University of California, Berkeley}
\journaleditor{Andrew Myers}{Cornell University}
\journaleditor{Helen Nissenbaum}{New York University}
\journaleditor{Michael Reiter}{University of North Carolina}
\journaleditor{Shankar Sastry}{University of California, Berkeley}
\journaleditor{Dawn Song}{University of California, Berkeley}
\journaleditor{Daniel Weitzner}{Massachusetts Institute of Technology}
\end{multicols}
\end{editorialboard} 


==> journaldata/SEC-journaldata.tex <==
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}
\colorlet{SECcolor}{bananayellow}   %new color names can be defined before use
\journalcolor      {SECcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Privacy and Security}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SEC}
\journalurl        {http://nowpublishers.com/SEC}
\journalissnprint  {2474-1558}
\journalissnonline {2474-1566}
\journaldoi        {10.1561/33}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Privacy and Security publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Access control}
\item{Accountability}
\item{Anonymity}
\item{Application security}
\item{Artifical intelligence methods in security and privacy}
\item{Authentication}
\item{Big data analytics and privacy}
\item{Cloud security}
\item{Cyber-physical systems security and privacy}
\item{Distributed systems security and privacy}
\item{Embedded systems security and privacy}
\item{Forensics}
\item{Hardware security}
\item{Human factors in security and privacy}
\item{Information flow}
\item{Intrusion detection}
\item{Malware}
\item{Metrics}
\item{Mobile security and privacy}
\item{Language-based security and privacy}
\item{Network security}
\item{Privacy-preserving systems}
\item{Protocol security}
\item{Security and privacy policies}
\item{Security architectures}
\item{System security}
\item{Web security and privacy}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Privacy and Security, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SEC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Contextual Integrity through the Lens of Computer Science}\\
Sebastian Benthall, Seda Gurses and Helen Nissenbaum\\
ISBN: 978-1-68083-384-3\\
\\
\noindent \textit{Methods for Location Privacy: A comparative overview}\\
Kostantinos Chatzikokolakis, Ehab ElSalamouny, Catuscia Palamidessi and Pazii Anna\\
ISBN: 978-1-68083-366-9\\
\\
\noindent \textit{Principles and Implementation Techniques of Software-Based Fault Isolation}\\
Gang Tan\\
ISBN: 978-1-68083-344-7\\
\\
\noindent \textit{Modeling and Verifying Security Protocols with the Applied Pi\\ Calculus and ProVerif}\\
Bruno Blanchet\\
ISBN: 978-1-68083-206-8

==> journaldata/SIG-editorialboard.tex <==
%SIG-Editorialboard.

\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Yonina Eldar}{Weizmann Institute\\Israel}



\subsection{Editors}
\begin{multicols}{3}\raggedcolumns
\journaleditor{Pao-Chi Chang}{National Central University}
\journaleditor{Pamela Cosman}{University of California, San Diego}
\journaleditor{Michelle Effros}{California Institute of Technology}
\journaleditor{Yariv Ephraim}{George Mason University}
\journaleditor{Alfonso Farina}{Selex ES}
\journaleditor{Sadaoki Furui}{Tokyo Institute of Technology}
\journaleditor{Georgios Giannakis}{University of Minnesota}
\journaleditor{Vivek Goyal}{Boston University}
\journaleditor{Sinan Gunturk}{Courant Institute}
\journaleditor{Christine Guillemot}{INRIA}
\journaleditor{Robert W. Heath, Jr.}{The University of Texas at Austin}
\journaleditor{Sheila Hemami}{Northeastern University}
\journaleditor{Lina Karam}{Arizona State University}
\journaleditor{Nick Kingsbury}{University of Cambridge}
\journaleditor{Alex Kot}{Nanyang Technical University}
\journaleditor{Jelena Kovacevic}{New York University}
\journaleditor{Geert Leus}{TU Delft}
\journaleditor{Jia Li}{Pennsylvania State University}
\journaleditor{Henrique Malvar}{Microsoft Research}
\journaleditor{B.S. Manjunath}{University of California, Santa Barbara}
\journaleditor{Urbashi Mitra}{University of Southern California}
\journaleditor{Bj\"{o}rn Ottersten}{KTH Stockholm}
\journaleditor{Vincent Poor}{Princeton University}
\journaleditor{Anna Scaglione}{University of California, Davis}
\journaleditor{Mihaela van der Shaar}{University of California, Los Angeles}
\journaleditor{Nicholas D. Sidiropoulos}{Technical University of Crete}
\journaleditor{Michael Unser}{EPFL}
\journaleditor{P.P. Vaidyanathan}{California Institute of Technology}
\journaleditor{Ami Wiesel}{The Hebrew University of Jerusalem}
\journaleditor{Min Wu}{University of Maryland}
\journaleditor{Josiane Zerubia}{INRIA}
\end{multicols}
\end{editorialboard} 


==> journaldata/SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SIG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Recent Advances in Clock Synchronization for Packet-Switched Networks}\\
Anantha K. Karthik and Rick S. Blum\\
ISBN: 978-1-68083-726-1\\
\\
\noindent \textit{Biomedical Image Reconstruction: From the Foundations to Deep Neural Networks}\\
Michael T. McCann and Michael Unser\\
ISBN: 978-1-68083-650-9\\
\\
\noindent \textit{Compressed Sensing with Applications in Wireless Networks}\\
Markus Leinonen, Marian Codreanu and Georgios B. Giannakis\\
ISBN: 978-1-68083-646-2\\

==> journaldata/STP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/STP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Panos J. Antsaklis}{University of Notre Dame\\United States}
\journalchiefeditor{Alessandro Astolfi}{Imperial College London, United Kingdom\\ University of Rome ''Tor Vergata'', Italy}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{John Baillieul}{Boston University}
\journaleditor{Peter Caines}{McGill University}
\journaleditor{Christos Cassandras}{Boston University}
\journaleditor{Denis Dochain}{UC Louvain}
\journaleditor{Magnus Egerstedt}{Georgia Institute of Technology}
\journaleditor{Karl Henrik Johansson}{KTH Stockholm}
\journaleditor{Miroslav Krstic}{University of California, San Diego}
\journaleditor{Jan Maciejowski}{University of Cambridge}
\columnbreak
\journaleditor{Dragan Nesic}{The University of Melbourne}
\journaleditor{Marios Polycarpou}{University of Cyprus}
\journaleditor{J\"{o}rg Raisch}{Technical University Berlin}
\journaleditor{Arjan van der Schaft}{University of Groningen}
\journaleditor{M. Elena Valcher}{University of Padova}
\journaleditor{Richard Vinter}{Imperial College London}
\journaleditor{George Weiss}{Tel Aviv University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/SYS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet {SYScolor}{cobalt} %new color names can be defined before use
\journalcolor      {SYScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Systems and Control}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SYS}
\journalurl        {http://www.nowpublishers.com/SYS}
\journalissnprint  {2325-6818}
\journalissnonline {2325-6826}
\journaldoi        {10.1561/26}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Systems and Control publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Control of:}
	\begin{itemize}
	\item{Hybrid and Discrete Event Systems}
	\item{Nonlinear Systems}
	\item{Network Systems}
	\item{Stochastic Systems}
	\item{Multi-agent Systems}
	\item{Distributed Parameter Systems}
	\item{Delay Systems}
	\end{itemize}
	\columnbreak
\item{Filtering, Estimation, Identification}
\item{Optimal Control}
\item{Systems Theory}
\item{Control Applications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Systems and Control, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Learning-Based Control: A Tutorial and Some Recent Results}\\
Zhong-Ping Jiang, Tao Bian and Weinan Gao\\
ISBN: 978-1-68083-752-0\\
\\
\noindent \textit{Synchronous Reinforcement Learning-Based Control for Cognitive Autonomy}\\
Kyriakos G. Vamvoudakis and Nick-Marios T. Kokolakis\\
ISBN: 978-1-68083-744-5\\
\\
\noindent \textit{Achieving Ecological Resilience Through Regime Shift Management}\\
M. D. Lemmon\\
ISBN: 978-1-68083-716-2\\
\\
\noindent \textit{Distributed Optimization for Smart Cyber-Physical Networks}\\
Giuseppe Notarstefano, Ivano Notarnicola and Andrea Camisa\\
ISBN: 978-1-68083-618-9\\
\\
\noindent \textit{Resilient Control in Cyber-Physical Systems: Countering Uncertainty, Constraints, and Adversarial Behavior}\\
Sean Weerakkody, Omur Ozel, Yilin Mo and Bruno Sinopoli\\
ISBN: 978-1-68083-586-1


==> journaldata/TCS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Salil Vadhan}{Harvard University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Bernard Chazelle}{Princeton University}
\journaleditor{Oded Goldreich}{Weizmann Institute}
\journaleditor{Shafi Goldwasser}{Massachusetts Institute of Technology and Weizmann Institute}
\journaleditor{Sanjeev Khanna}{University of Pennsylvania}
\journaleditor{Jon Kleinberg}{Cornell University}
\journaleditor{L\'aszl\'o Lov\'asz}{Eötvös Lor\'and University}
\journaleditor{Christos Papadimitriou}{University of California, Berkeley}
\journaleditor{Peter Shor}{Massachusetts Institute of Technology}
\journaleditor{Eva Tardos}{Cornell University}
\journaleditor{Salil Vadhan}{Cornell University}
\journaleditor{Avi Wigderson}{AIS, Princeton University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TCS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{TCScolor}{cobalt}   %new color names can be defined before use
\journalcolor      {TCScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TCS}
\journalurl        {http://www.nowpublishers.com/TCS}
\journalissnprint  {1551-305X}
\journalissnonline {1551-3068}
\journaldoi        {10.1561/04}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Algorithmic game theory}
    \item{Computational algebra}
    \item{Computational aspects of combinatorics and graph theory}
    \item{Computational aspects of communication}
    \item{Computational biology}
    \item{Computational complexity}
    \item{Computational geometry}
    \item{Computational learning}
    \item{Computational Models and Complexity}
    \item{Computational Number Theory}
    \item{Cryptography and information security}
    \item{Data structures}
    \item{Database theory}
    \item{Design and analysis of algorithms}
    \item{Distributed computing}
    \item{Information retrieval}
    \item{Operations Research}
    \item{Parallel algorithms}
    \item{Quantum Computation}
    \item{Randomness in Computation}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TCS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Higher-order Fourier Analysis and Applications}\\
Hamed Hatami, Pooya Hatami and Shachar Lovett\\
ISBN: 978-1-68083-592-2\\
\\
\noindent \textit{On Doubly-Efficient Interactive Proof Systems}\\
Oded Goldreich \\
ISBN: 978-1-68083-424-6\\
\\
\noindent \textit{Coding for Interactive Communication: A Survey}\\
Ran Gelles\\
ISBN: 978-1-68083-346-1\\

==> journaldata/TOM-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Panos Kouvelis}{Washington University St. Louis\\USA}

\subsection{Editors}
\journaleditor{Charles Corbett}{UCLA, USA}
\journaleditor{Uday Karmarkar}{UCLA, USA}

\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Onur Bayabatli}{Singapore Management University, Singapore}
\journaleditor{Jan Fransoo}{Tilburg University, The Netherlands} 
\journaleditor{Chuck Munson}{Washington State University, USA} 
\journaleditor{Nicholas Petruzzi}{Pennsylvania State University, USA}
\journaleditor{Guillaume Roels}{INSEAD, France}
\journaleditor{Nicola Secomandi}{Carnegie-Mellon University, USA} 
\journaleditor{Zuo-Jun Max Shen}{University of California, Berkeley, USA} 
\journaleditor{Sherri Xiaole Wu}{Fudan University, China} 
\journaleditor{Y. Karen Zheng}{MIT, USA} 
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TOM-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{TOMcolor}{cerise}   %new color names can be defined before use
\journalcolor      {TOMcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Technology, Information and Operations Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TOM}
\journalurl        {http://www.nowpublishers.com/TOM}
\journalissnprint  {1571-9545}
\journalissnonline {1571-9553}
\journaldoi        {10.1561/02}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Technology, Information and Operations Management publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{B2B Commerce}
\item{Business Process Engineering and Design}
\item{Business Process Outsourcing}
\item{Capacity Planning}
\item{Competitive Operations}
\item{Contracting in Supply Chains}
\item{E-Commerce and E-Business Models}
\item{Electronic markets, auctions and exchanges}
\item{Enterprise Management Systems}
\item{Facility Location}
\item{Information Chain Structure and Competition}
\item{International Operations}
\item{Marketing/Manufacturing Interfaces}
\item{Multi-location inventory theory}
\item{New Product \& Service Design}
\item{Queuing Networks}
\item{Reverse Logistics}
\item{Service Logistics and Product Support}
\item{Supply Chain Management}
\item{Technology Management and Strategy}
\item{Technology, Information and Operations in:}
	\begin{itemize}
	\item{Automotive Industries}
	\item{Electronics manufacturing}
	\item{Financial Services}
	\item{Health Care}
	\item{Media and Entertainment}
	\item{Process Industries}
	\item{Retailing}
	\item{Telecommunications}
	\end{itemize}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Technology, Information and Operations Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TOM-seriespage.tex <==
\vspace{12pt}
\noindent \textit{AI and Business Models: The Good, The Bad and The Ugly}\\
Vania Sena and Manuela Nocker
\\ISBN: 978-1-68083-794-0
\\
\\
\noindent \textit{The Business of Electric Vehicles: A Platform Perspective}\\
Jonas Boehm, Hemant K. Bhargava and Geoffrey G. Parker
\\ISBN: 978-1-68083-762-9
\\
\\
\noindent \textit{Advances in Supply Chain Finance and FinTech Innovations Overview}\\
Panos Kouvelis, Ling Dong and Danko Turcic
\\ISBN: 978-1-68083-722-3

==> journaldata/WEB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}%\raggedcolumns
\journalchiefeditor{Wendy Hall}{University of Southampton, UK}
\journalchiefeditor{Noshir R. Contractor}{Northwestern University, USA}
\journalchiefeditor{Kieron O'Hara}{University of Southampton, UK}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Tim Berners-Lee}{Massachusetts Institute of Technology}
\journaleditor{Noshir Contractor}{Northwestern University}
\journaleditor{Lorrie Crano}{Carnegie Mellon University}
\journaleditor{Dieter Fensel}{University of Innsbruck}
\journaleditor{Carole Goble}{University of Manchester}
\journaleditor{Pat Hayes}{IHMC}
\journaleditor{James Hendler}{Rensselaer Polytechnic Institute}
\journaleditor{Arun Iyengar}{IBM Research}
%\columnbreak
\journaleditor{Craig Knoblock}{University of Southern California}
\journaleditor{Ora Lassila}{Pegasystems}
\journaleditor{Sun Maosong}{Tsinghua University}
\journaleditor{Cathy Marshall}{Microsoft}
\journaleditor{Peter Monge}{University of Southern California}
\journaleditor{Ben Shneiderman}{University of Maryland}
\journaleditor{Danny Weitzner}{Massachusetts Institute of Technology}
\journaleditor{Yorick Wilks}{University of Sheffield}
\end{multicols*}
\end{editorialboard} 

==> journaldata/WEB-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{WEBcolor}{brickred}   %new color names can be defined before use
\journalcolor      {WEBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Web Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {WEB}
\journalurl        {http://www.nowpublishers.com/WEB}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Web Science publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Agents and the Semantic Web}
    \item{Collective Intelligence}
    \item{Content Management}
    \item{Databases on the Web}
    \item{Data Mining}
    \item{Democracy and the Web}
    \item{Dependability}
    \item{Economics of information and the Web}
    \item{E-Crime}
    \item{E-Government}
    \item{Emergent behaviour}
    \item{Ethics}
    \item{Hypertext/Hypermedia}
    \item{Identity}
    \item{Languages on the Web}
    \item{Memories for Life}
    \item{Mobile/Pervasive}
    \item{Network Infrastructures}
    \item{Performance}
    \item{Privacy}
    \item{Scalability}
    \item{Security}
    \item{Semantic Web}
    \item{Social Networking}
    \item{Standards}
    \item{The Law and the Web}
    \item{The Web as an Educational Tool}
    \item{The Web in the Developing World}
    \item{Trust and Provenance}
    \item{Universal Usability}
    \item{User Interfaces}
    \item{Virtual Reality}
    \item{Web Art}
    \item{Web Governance}
    \item{Search}
    \item{Web Services}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Web Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/WEB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{An Introduction to Hybrid Human-Machine Information Systems}\\
Gianluca Demartini, Djellel Eddine Difallah, Ujwal Gadiraju and\\ Michele Catasta\\
ISBN: 978-1-68083-374-4\\
\\
\noindent \textit{Minds Online: The Interface between Web Science, Cognitive Science and the Philosophy of Mind}\\
Paul Smart, Robert Clowes and Richard Heersmink\\
ISBN: 978-1-68083-322-5\\
\\
\noindent \textit{Collective Attention on the Web}\\
Christian Bauckhage and Kristian Kersting\\
ISBN: 978-1-68083-204-4

==> methods_table.tex <==
\begin{tabular}{llllllllllllllllllllllllll}
\toprule
{} &                                               Name &         FCN & Skip Connections & Boundary Awareness & Multi-scale Feature Maps & Dilated Convolutions & Dynamic Parameters &        RNNs &        LSTM & Deformable Convolution &   Attention &          EM & Graphical representation & 3D segmentation &         GAN & Semi-supervision & Reinforcement Learning & Contour-based & Region Proposals &   One-stage & Meta-learning & Query-based &                                            Summary &                        Benchmarks and Performances &                  Notes \\
\midrule
0  &                                                FCN &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  End-to-end dense learning with fully convoluti... &  PASCAL VOC (62.2), NYUDv2 (34.0), SIFT Flow (3... &                        \\
1  &                                              U-Net &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &                                   Skip connections &                 PhC-U373 (92.03), DIC-HeLa (77.56) &                        \\
2  &                                             SegNet &  \checkmark &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &                                    Pooling indices &                                   SUN-RGBD (31.84) &                        \\
3  &                                                SDS &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Multiscale Combinatorial Grouping (MCN) algori... &                                  PASCAL VOC (52.6) &                        \\
4  &                                                SDN &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  SDN unit - shallow deconvolutional network wit... &    PASCAL VOC (86.6), CamVid (71.8), GATECH (55.9) &                        \\
5  &                                            LSD-Net &  \checkmark &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &               Boundary refinement and RGB-D fusion &                                NYU-Depth v2 (45.9) &                        \\
6  &                                                FPN &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Feature pyramids with top-down and bottom-up p... &                              MS COCO val (AR=48.1) &                        \\
7  &                                             PSPNet &  \checkmark &       \checkmark &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Pyramid Pooling Module that takes global infor... &               PASCAL VOC (85.4), Cityscapes (80.2) &                        \\
8  &                                              DMNet &  \checkmark &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Dynamic Convolutional Module that generates co... &  PASCAL VOC (84.4), ADE20K (45.50), PASCAL-Cont... &                        \\
9  &                                             APCNet &  \checkmark &                  &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Adaptive Context Module that estimate Global-g... &  PASCAL VOC (84.2), ADE20K (45.38), PASCAL-Cont... &                        \\
10 &                                                CCN &  \checkmark &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Selectively aggregation of appropriate scale f... &  Pascal Context (51.6), SUN-RGBD (47.1), COCO S... &                        \\
11 &                                               MSCI &  \checkmark &                  &                    &               \checkmark &                      &                    &             &  \checkmark &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Contextual information exchange through bidire... &  PASCAL VOC (88.0), NYUDv2 (49.0), PASCAL-Conte... &                        \\
12 &                                           ParseNet &  \checkmark &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Global Pooling and simple global feature map i... &  PASCAL VOC (69.8), SIFT Flow (40.4), PASCAL-Co... &                        \\
13 &                                          RefineNet &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Residual Convolution Units for end-to-end trai... &  PASCAL VOC (83.4), ADE20K (40.7), PASCAL-Conte... &                        \\
14 &                                              DANet &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Dual-attention modules for incoporating contex... &  Cityscapes (81.5), PASCAL VOC (82.6), PASCAL-C... &                        \\
15 &                                             PSANet &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Distribute and Collect attention branches for ... &  ADE20K (43.77), PASCAL VOC (85.7), Cityscapes ... &                        \\
16 &                                             GT-OCR &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Aggregation of object region representations b... &  Cityscapes (84.5), LIP (56.65), PASCAL-Context... &                        \\
17 &                                               FaPN &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &             \checkmark &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Feature alignment between top-down and bottom ... &  ADE20K(56.7), Cityscapes (80.0),  COCO-Stuff (... &                        \\
18 &                                          DeepLab3+ &             &                  &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Segmentation quality improvement with atrous c... &                                  PASCAL VOC (89.0) &                        \\
19 &                                         Dilation10 &             &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Aggretation of contextual information through ... &                                  PASCAL VOC (75.3) &                        \\
20 &                                    ResNet-DUC-HDC  &             &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Solve "Gridding" issue from dilated convolutio... &                                  PASCAL VOC (83.1) &                        \\
21 &                                          DenseASPP &             &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Dense multi-scale feature map generation with ... &                                  Cityscapes (80.6) &                        \\
22 &                                               GALD &             &       \checkmark &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Improves small pattern segmentation with Globa... &          Cityscapes (83.3), MS-COCO (Mask AP=37.8) &                        \\
23 &                                               MRFM &             &                  &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Adaptive selection of receptive field and edge... &               PASCAL VOC (88.4), Cityscapes (83.0) &                        \\
24 &                                          SegFormer &             &                  &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Hierarchical Transformer encoder and all-MLP d... &  Cityscapes (84.0), ADE20K(50.3), COCO-Stuff (4... &                        \\
25 &                                             ExFuse &             &                  &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  More effective multi-scale feature fusion with... &                                  PASCAL VOC (87.9) &                        \\
26 &                                              SANet &  \checkmark &                  &                    &               \checkmark &           \checkmark &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &      Class-wise mask generation for pixel grouping &           PASCAL VOC (86.1), PASCAL-Context (54.4) &                        \\
27 &                                               Swin &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Efficient computation of hierarchical feature ... &              ADE20K (53.5), MS-COCO (Mask AP=51.1) &                        \\
28 &                                            EMA-Net &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &  \checkmark &                          &                 &             &                  &                        &               &                  &             &               &             &  Formulation of attention into Expectation-Maxi... &  PASCAL VOC (88.2), PASCAL-Context (53.1), COCO... &                        \\
29 &                                                DFN &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Application of different weights to different ... &               PASCAL VOC (86.2), Cityscapes (80.3) &                        \\
30 &                                              CCNet &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Impvorves efficiency of attention mechanism wi... &                  ADE20K (45.22), Cityscapes (81.4) &                        \\
31 &                Hierarchical Multi-scale Attention  &             &                  &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Hierarchical attention-based approach that lea... &           Cityscapes test (85.1), Mapillary (61.1) &                        \\
32 &                                         MaskFormer &             &                  &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Solves semantic and instance segmentation in u... &  ADE20K (55.6), Cityscapes (78.5), COCO-Stuff (... &                        \\
33 &                                            CRF-RNN &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Integrates CRF modeling with CNN by formulatin... &                                  PASCAL VOC (74.7) &                        \\
34 &                                          Piecewise &             &                  &                    &               \checkmark &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Formulates CNN-based general pairwise potentia... &  PASCAL VOC (78.0), NYUDv2 (40.6), SIFT-flow (4... &                        \\
35 &                                                DPN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Solves Markov Random Fields with a single CNN ... &                                  PASCAL VOC (77.5) &                        \\
36 &                                               GCRF &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Unification of Mean Field algorithm with CNN u... &                                  PASCAL VOC (73.2) &                        \\
37 &                                   Domain Transform &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Boundary learning with domain transfer edge-pr... &                                  PASCAL VOC (71.8) &                        \\
38 &                                              GSCNN &             &       \checkmark &         \checkmark &               \checkmark &           \checkmark &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &   Boundary detection improvement with shape stream &                             Cityscapes test (82.8) &                        \\
39 &                                             EncNet &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Context Encoding Module that captures the sema... &  PASCAL-Context (51.7), PASCAL VOC (85.9), ADE2... &                        \\
40 &                                              ReSeg &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Incorporation of contextual information with R... &  CamVid (58.8), Weizmann Horses (91.6), Oxford ... &                        \\
41 &                                            DAG-RNN &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Leveraging long-range contextual information w... &  SIFT Flow (global pixel acc=85.3), CamVid (glo... &                        \\
42 &                                            2D LSTM &             &                  &                    &                          &                      &                    &             &  \checkmark &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Capturing global and local dependencies with 2... &             SIFT Flow (70.11), Stanford BG (78.56) &                        \\
43 &                                            LSTM-CF &             &                  &                    &                          &                      &                    &             &  \checkmark &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Capturing and fusion of contextual information... &                     SUN-RGBD (48.1), NYUDv2 (49.7) &                        \\
44 &                                         Graph LSTM &             &                  &                    &                          &                      &                    &             &  \checkmark &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &               &             &  Modeling natural visual pattern flows with gra... &                         PASCAL-Person-Part (60.35) &                        \\
45 &  Segmenting Images based on natural language ex... &  \checkmark &                  &                    &                          &                      &                    &  \checkmark &  \checkmark &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  End-to-end trainable recurrent convolutional n... &                                    ReferIt (48.03) &                        \\
46 &         Convolutional GAN with weakly-labeled data &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &  \checkmark &       \checkmark &                        &               &                  &             &               &             &         GAN-based CNN leveraging three input types &  all labeled + unlabeled PASCAL VOC (65.8), ful... &                        \\
47 &  Semi-supervised semantic segmentation using an... &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &  \checkmark &       \checkmark &                        &               &                  &             &               &             &  Leveraging unlabeled images to enhance the seg... &  1/2 of PASCAL VOC (73.8), 1/2 of Cityscapes (6... &                        \\
48 &                                              SegAN &  \checkmark &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &             \checkmark &               &                  &             &               &             &  Segmentor and a critic network trained in an a... &                  BRATS 2015 test (Dice score=85.0) &                        \\
49 &                                              V-Net &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Loss function based on Dice coefficient for ta... &                     PROMISE2012 (Dice score=82.39) &                        \\
50 &                                             DA-RNN &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Injection of Semantic labels into 3D scenes wi... &        Synthetic ShapeNet Scene dataset (acc=85.9) &                        \\
51 &                                             3D-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &                   3D point cloud data segmentation &  Large Lidar point cloud dataset of the urban a... &                        \\
52 &                                      3DCNN-DQN-RNN &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &      \checkmark &             &                  &             \checkmark &               &                  &             &               &             &  Combining CNN, RNN, and Deep Q-Network for 3D ... &  Stanford 3D semantic parsing (acc=70.76), SUNC... &                        \\
53 &                                           PointNet &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Raw point clouds segmentation with feature tra... &                               ShapeNet part (83.7) &                        \\
54 &                                 Clockwork Convnets &             &                  &                    &                          &                      &         \checkmark &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Clockwork convnets driven by fixed or adaptive... &  Youtube-Objects (70.0), NYUD (28.9), and Citys... &                        \\
55 &                                End2End Voxel2Voxel &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  End-to-end trainable 3D convolutional architec... &                                      GATECH (76.0) &                        \\
56 &                                              RSNet &             &                  &                    &                          &                      &                    &  \checkmark &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Extraction of feature dependencies with slice ... &  S3DIS (51.93),  ScanNet (39.35), ShapeNet (acc... &                        \\
57 &                                                SPG &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &               \checkmark &      \checkmark &             &                  &                        &               &                  &             &               &             &  Novel 3D point cloud representation capturing ... &                   S3DIS (62.1),  Semantic3D (76.2) &                        \\
58 &                                         RandLA-Net &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Random sampling of point clouds and local feat... &            Semantic3D (77.4), SemanticKITTI (53.9) &                        \\
59 &                                            SCF-Net &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Spatial Contextual Feature learning from large... &                   S3DIS (71.6),  Semantic3D (77.6) &                        \\
60 &                                           BAAF-Net &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Local context augmentation with bilateral bloc... &  S3DIS (72.2),  Semantic3D (76.2), SemanticKITT... &                        \\
61 &                                  Point Transformer &             &       \checkmark &                    &                          &                      &                    &             &             &                        &  \checkmark &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &      Vector self-attention based transformer layer &        S3DIS (73.5), ShapeNetPart (ins. mIoU=86.6) &                        \\
62 &                                         Cylinder3D &             &       \checkmark &                    &                          &                      &         \checkmark &             &             &                        &             &             &                          &      \checkmark &             &                  &                        &               &                  &             &               &             &  Cylindrical partition of point clouds and asym... &             SemanticKITTI (67.8), nuScenes (76.1)  &                        \\
63 &      Dense U-Net-based active contour segmentation &             &       \checkmark &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Loss function combining contour length and reg... &  ACDC 2017 Challenge (Hausdorff Dist. is 33.8%,... &                        \\
64 &  Unsupervised Microvascular Image Segmentation ... &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Novel pooling layer mimicking curvature morpho... &                   VesselNN (76.0), DeepVess (83.8) &                        \\
65 &                    Trainable Deep Active Contours  &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Integration of Active Contour Models and CNNs ... &                 Vaihingen (84.0), Bing huts (65.0) &                        \\
66 &                                           DeepMask &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &         Region proposals and object classification &    MS COCO (AR= 36.6), PASCAL VOC 2007 (AR = 43.3) &  Proposal accuracy: AR \\
67 &                                          SharpMask &             &                  &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Augmenting feedforward nets for object segment... &                                 MS COCO (AR= 39.3) &                        \\
68 &                                       MultiPathNet &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Capturing multi-scale contexts with foveal str... &                             MS COCO (Mask AP=25.0) &                        \\
69 &                                         Mask R-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Extends Faster R-CNN by adding a branch for pr... &  Cityscapes (Mask AP=36.4), MS COCO (ResNeXt-10... &                        \\
70 &                                 Mask Scoring R-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  MaskIoU head trained with simple regression fo... &                             MS COCO (Mask AP=39.6) &                        \\
71 &                                              PANet &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Bottom-up path augmentation; adaptive feature ... &  MS COCO (Mask AP=42.0), Cityscapes (Mask AP=41.4) &                        \\
72 &                                               MNCs &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Three-stage network consisting of instance dif... &  PASCAL VOC (Mask AP(IOU=0.5)=63.5), MS COCO (M... &                        \\
73 &                                        MaskX R-CNN &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Weight transfer function that maps a category’... &                             MS COCO (Mask AP=29.5) &                        \\
74 &                                            MaskLab &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Three branches consisting of box detection, se... &                             MS COCO (Mask AP=43.0) &                        \\
75 &                                                OMN &             &       \checkmark &         \checkmark &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  inference of object segment representation bas... &  PASCAL VOC (MASK AP(IOU=0.5)=65.69), Cityscape... &                        \\
76 &                                               FCOS &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Center-ness loss measuring how “centered” is t... &                             MS COCO (Mask AP=44.7) &                        \\
77 &                                         ExtremeNet &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Extreme points used approximate an instance se... &                             MS COCO (Mask AP=34.6) &                        \\
78 &                                           ESE-Seg  &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Using inner center radius shape signature to p... &                             MS COCO (Mask AP=21.6) &                        \\
79 &                                          PolarMask &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Formulating segmentation as  a regression prob... &                             MS COCO (Mask AP=32.9) &                        \\
80 &                                         FourierNet &             &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &  \checkmark &               &             &  Obtaining contour points with Inverse Fast Fou... &                             MS COCO (Mask AP=30.6) &                        \\
81 &                                             MEInst &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Mask representation with compact fixed-dimensi... &                             MS COCO (Mask AP=38.2) &                        \\
82 &                                         TensorMask &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Representation of image content (e.g., masks) ... &                             MS COCO (Mask AP=37.3) &                        \\
83 &                                             YOLACT &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Real-time instance segmentation through linear... &                             MS COCO (Mask AP=31.2) &                        \\
84 &                                          BlendMask &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Blender module incorporating rich instance-lev... &                             MS COCO (Mask AP=41.3) &                        \\
85 &                                         CenterMask &             &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Predicting segmentation mask inside detected b... &                             MS COCO (Mask AP=41.8) &                        \\
86 &                                               SOLO &  \checkmark &       \checkmark &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Transforms instance segmentation into two pixe... &                             MS COCO (Mask AP=37.8) &                        \\
87 &                                             SOLOv2 &  \checkmark &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Decomposing mask learning to feature learning ... &                             MS COCO (Mask AP=41.7) &                        \\
88 &                                           CondInst &             &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &  \checkmark &               &             &  Dynamically generated convolutional filters co... &                             MS COCO (Mask AP=40.1) &                        \\
89 &                           Deep Watershed Transform &             &       \checkmark &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &    \checkmark &                  &             &               &             &  Extraction of object instance segments with en... &                          Cityscapes (Mask AP=19.4) &                        \\
90 &                               Deep Metric Learning &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Clustering pixel embeddings for instance segme... &                PASCAL VOC (MASK AP(IOU=0.5)=62.21) &                        \\
91 &                                 Cascade Mask R-CNN &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &             &  Progressively improves boudning box quaality w... &                 MS COCO (2017 val)  (Mask AP=42.3) &                        \\
92 &                     Soft Teacher and Box Jittering &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &       \checkmark &             \checkmark &               &                  &             &               &             &  Semi-supervised training with both labeled and... &                             MS COCO (Mask AP=53.0) &                        \\
93 &                                               SOTR &             &       \checkmark &                    &               \checkmark &                      &         \checkmark &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &             &  Twin attention mechanism with sparse represent... &                             MS COCO (Mask AP=42.1) &                        \\
94 &                                              DCNAS &             &                  &                    &                          &                      &                    &             &             &                        &             &             &               \checkmark &                 &             &                  &                        &               &                  &             &    \checkmark &             &  Direct search of optimal network structure for... &  Cityscapes test (84.3), PASCAL VOC (86.9), ADE... &                        \\
95 &                                                DPC &             &                  &                    &               \checkmark &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &                  &             &    \checkmark &             &  Recursive search space for optimal network str... &  Cityscapes test (82.7), PASCAL VOC (87.9), PAS... &                        \\
96 &                                               DETR &             &                  &                    &                          &                      &         \checkmark &             &             &                        &  \checkmark &             &                          &                 &             &                  &                        &               &                  &             &               &  \checkmark &  Set-based global loss that forces unique predi... &                      MS COCO (Panoptic Quality=46) &                        \\
97 &                                          QueryInst &             &                  &                    &                          &                      &                    &             &             &                        &             &             &                          &                 &             &                  &                        &               &       \checkmark &             &               &  \checkmark &         Parallel supervision on dynamic mask heads &  MS COCO (Mask AP=42.8), Cityscapes (Mask AP=34... &                        \\
\bottomrule
\end{tabular}


==> new_datasets_tables.tex <==
\begin{tabular}{lllllll}
\toprule
Dataset Name & Object Detection & Semantic Segmentation & Instance Segmentation & Panoptic Segmentation & 3D segmentation & Video segmentation \\
\midrule
  Cityscapes &                  &             checkmark &             checkmark &             checkmark &                 &          checkmark \\
    ShapeNet &                  &             checkmark &                       &                       &       checkmark &                    \\
       S3DIS &                  &             checkmark &                       &                       &       checkmark &                    \\
       NYUv2 &                  &             checkmark &             checkmark &                       &                 &                    \\
     ScanNet &                  &             checkmark &                       &             checkmark &       checkmark &                    \\
       DAVIS &                  &                       &                       &                       &                 &          checkmark \\
      ADE20K &                  &             checkmark &                       &                       &                 &                    \\
   Sun RGB-D &        checkmark &             checkmark &                       &                       &                 &                    \\
  Semantic3D &                  &             checkmark &                       &                       &                 &                    \\
  PASCAL VOC &        checkmark &             checkmark &                       &                       &                 &                    \\
      CamVid &                  &             checkmark &                       &                       &                 &          checkmark \\
         LIP &                  &             checkmark &                       &                       &                 &                    \\
        COCO &        checkmark &             checkmark &             checkmark &             checkmark &                 &                    \\
       KITTI &        checkmark &             checkmark &                       &             checkmark &                 &                    \\
 YouTube-VOS &                  &                       &                       &                       &                 &          checkmark \\
    nuScenes &        checkmark &             checkmark &             checkmark &                       &       checkmark &                    \\
    nuImages &        checkmark &             checkmark &             checkmark &                       &                 &                    \\
        LVIS &        checkmark &                       &             checkmark &                       &                 &                    \\
     PartNet &                  &                       &                       &                       &       checkmark &                    \\
       DRIVE &                  &             checkmark &                       &                       &                 &                    \\
   PROMISE12 &                  &             checkmark &                       &                       &                 &                    \\
\bottomrule
\end{tabular}
\begin{tabular}{lllllll}
\toprule
Dataset Name &                                   Others (Specify) &                                \# of object classes &                                               Size &   Scene &                                              Notes &                                              Links \\
\midrule
  Cityscapes & Image-to-image Translation, Real-Time Semantic ... &                                                 30 & 5000 fine annotated images, 20000 coarse annota... &  street &                                                    &                                                    \\
    ShapeNet &                                  3D Reconstruction &                                               3135 &                  over 300M models, 220k classified & variety & ShapeNet Parts subset contains 31,693 meshes ca... &                                                    \\
       S3DIS &                                                    &                                                 12 &          6 large-scale indoor areas with 271 rooms &  indoor & 3D Instance Segmentation and 3D Semantic Segmen... &                                                    \\
       NYUv2 & 3D Object Detection, Scene Segmentation, Monocu... &                                                 26 & 1449 densely labeled pairs of aligned RGB and d... &  indoor &                                                    &                                                    \\
     ScanNet & Scene Segmentation, 3D Object Detection, Depth ... &                                                 20 & 1513 annotated scans of labeled voxels with an ... &  indoor &                                       2D \& 3D data &                                                    \\
       DAVIS & Interactive Segmentation, Video Denoising, Vide... &                                                    & 50 video sequences with 3455 densely annotated ... & variety &                                                    &                                                    \\
      ADE20K & Image-to-Image Translation, Scene Recognition, ... &                                                150 & 20K scene-centric images exhaustively annotated... & variety & Scene Parsing Benchmark (SceneParse150) is a sm... &                                                    \\
   Sun RGB-D & 3D Object Detection, Monocular 3D Obeject Detec... &                                                700 & 10335 real RGB-D images of room scenes. Each RG... &  indoor &                                                    &                                                    \\
  Semantic3D &                                                    &                                                  8 & over 3 billion points, 15 training and 15 test ... & outdoor &                                                    &                                                    \\
  PASCAL VOC & Weakly-supervised instance segmentation, Weakly... &                                                 20 & 1,464 images for training, 1,449 images for val... & variety &                                                    &                                                    \\
      CamVid &                    Real-Time Semantic Segmentation &                                                 32 &                                         701 frames &  street &                                                    &                                                    \\
         LIP &                                                    &                                                 19 & 50,000 images with elaborated pixel-wise annota... &  people &                                                    &                                                    \\
        COCO & Real-Time Object Detection, Pose Estimation, Ke... & object detection: 80, keypoints detection: 17, ... &                                        328K images & variety &                                                    &                                                    \\
       KITTI & 3D Object Detection, Vehicle Pose Estimation, M... &                                                    & 180 GB sensor streams with images, OXTS, and Ve... &  street & Not all sequences are annotated, i.e. only the ... & http://www.cvlibs.net/publications/Geiger2013IJ... \\
 YouTube-VOS & Visual Object Tracking, One-shot visual object ... &                                               7800 & 4,453 videos, 340+ minutes, labeled with dense ... &         &                                                    &                                                    \\
    nuScenes & 3D Object Detection, 3D Multi-Object Tracking, ... &                                                 10 &                    28130 samples from 1,000 scenes &  street &                                                    &                                                    \\
    nuImages &                                                    &                                                 10 &                            93,000 annotated images &  street &                                                    &                                                    \\
        LVIS &                                                    &                                                1k+ &                                        164k images & variety &                    Has a long tail of rare objects &               https://arxiv.org/pdf/1908.03195.pdf \\
     PartNet &                                                    &                                                 24 &       573,585 part instances over 26,671 3D models &         & annotated with fine-grained, instance-level, an... &                   https://partnet.cs.stanford.edu/ \\
       DRIVE &                         Medical Image Segmentation &                                                    &                                          40 images & medical &                                                    &                                                    \\
   PROMISE12 &                         Medical Image Segmentation &                                                    &                                  50 training cases & medical &                                                    &                                                    \\
\bottomrule
\end{tabular}

